Practical and Matching Gradient Variance Bounds for Black-Box Variational Bayesian Inference

Understanding the gradient variance of black-box variational inference (BBVI) is a crucial step for establishing its convergence and developing algorithmic improvements. However, existing studies have yet to show that the gradient variance of BBVI satisfies the conditions used to study the convergence of stochastic gradient descent (SGD), the workhorse of BBVI. In this work, we show that BBVI satisfies a matching bound corresponding to the $ABC$ condition used in the SGD literature when applied to smooth and quadratically-growing log-likelihoods. Our results generalize to nonlinear covariance parameterizations widely used in the practice of BBVI. Furthermore, we show that the variance of the mean-field parameterization has provably superior dimensional dependence.

==> figures/group_airfoil_linearchol_generalbound.tex <==

  \nextgroupplot[
      %% legend style={
      %%   legend image post style = {scale=0.5},
      %%   legend columns          = -1,
      %%   column sep              = 1em,
      %%   %at                     ={(0.5,1.5)},
      %%   anchor                  = north,
      %%   legend cell align       = left,
      %%   line width              = 0.8pt,
      %%   draw                    = none,
      %%   legend to name          = grouplegend
      %% },
      %
      tuftelike, 
      axis line style = thick,
      every tick/.style={black,thick},
      %axis lines = left,
      %grids=both,
      ymode  = log,
      xmin   = 1,
      xmax   = 500,
      xtick  = {1, 100, 200, 300, 400, 500},
      ytick  = {1e+3, 1e+5, 1e+7, 1e+9, 1e+11},
      %
      ymin   = 1e+3,
      ymax   = 1e+11,
      %
      xlabel = {Iteration},
      %ylabel = {\(\mathbb{E}\norm{\rvvg}^2_2\)},
      height = 5cm,
      width  = 4.7cm,
      axis on top,
    ]
    \addplot[name path=gvar, color1, mark=none, thick]
      table [x=t, y=gvar] {data/simulation/airfoil_linearchol_generalbound.csv}
      %node[above=3pt,pos=0.8] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
      coordinate [pos=0.95] (gvarcoord);
    %\addlegendentry{\scriptsize\( \mathbb{E}\norm{ \rvvg }_2^2 \)}

    \addplot[name path=opt, color3, mark=none, thick] %
      table [x=t, y=opt] {data/simulation/airfoil_linearchol_generalbound.csv} %
      %node[above=3pt,pos=0.8] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)}
      coordinate [pos=0.95] (optcoord);
    %\addlegendentry{\scriptsize\(2 A \left(\mathbb{E}_{q_{\vlambda}} f_{\text{KL}} - f^*_{\text{KL}} \right)\)}

    \addplot[name path=ABC, color2, mark=none, thick]
      table [x=t, y=ABC] {data/simulation/airfoil_linearchol_generalbound.csv}
      coordinate [pos=0.05] (ABCcoord1) coordinate [pos=0.95] (ABCcoord2);
    %\addlegendentry{\scriptsize\(2 A \left(F\left(\vlambda\right) - F^*\right) + B \norm{\nabla F}_2^2 + C\)}

    \addplot[name path=axis, domain=0:490, fill=none, no markers, draw=none] {1e+3}
      coordinate [pos=0.05] (axiscoord);

    \addplot[name path=C, fill=none, gray, mark=none]
      table [x=t, y=C] {data/simulation/airfoil_linearchol_generalbound.csv}
      coordinate [pos=0.05] (Ccoord);

    \addplot[thick, color=color3, fill=color3, fill opacity=0.2] fill between[of=ABC and opt];
    \addplot[thick, color=color2, fill=color2, fill opacity=0.2] fill between[of=ABC and   C];

    \addplot[thick, color=color1, fill=color1, fill opacity=0.2] fill between[of=opt and gvar];
    \addplot[thick, color=gray,   fill=gray,   fill opacity=0.2] fill between[of=C   and axis];

    \draw[thick,color=color3,latex-latex] (ABCcoord2) -- (optcoord)
      node[midway,xshift=-20pt] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)};

    \draw[thick,color=gray,latex-] (Ccoord) -- (axiscoord)
      node[midway,xshift=5pt] {\scriptsize\(C\) };


==> figures/group_airfoil_softplusmf_generalbound.tex <==

  \nextgroupplot[
      %% legend style={
      %%   legend image post style = {scale=0.5},
      %%   legend columns          = -1,
      %%   column sep              = 1em,
      %%   %at                     ={(0.5,1.5)},
      %%   anchor                  = north,
      %%   legend cell align       = left,
      %%   line width              = 0.8pt,
      %%   draw                    = none,
      %%   legend to name          = grouplegend
      %% },
      %
      tuftelike, 
      axis line style = thick,
      every tick/.style={black,thick},
      %axis lines = left,
      %grids=both,
      ymode  = log,
      xmin   = 1,
      xmax   = 4000,
      xtick  = {1, 2000, 4000},
      ytick  = {1e+3, 1e+5, 1e+7, 1e+9, 1e+11},
      %
      ymin   = 1e+3,
      ymax   = 1e+11,
      %
      xlabel = {Iteration},
      %ylabel = {\(\mathbb{E}\norm{\rvvg}^2_2\)},
      height = 5cm,
      width  = 4.7cm,
      axis on top,
    ]
    \addplot[name path=gvar, color1, mark=none, thick]
      table [x=t, y=gvar] {data/simulation/airfoil_softplusmf_generalbound.csv}
      %node[above=3pt,pos=0.8] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
      coordinate [pos=0.95] (gvarcoord);
    %\addlegendentry{\scriptsize\( \mathbb{E}\norm{ \rvvg }_2^2 \)}

    \addplot[name path=opt, color3, mark=none, thick] %
      table [x=t, y=opt] {data/simulation/airfoil_softplusmf_generalbound.csv} %
      %node[above=3pt,pos=0.8] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)}
      coordinate [pos=0.95] (optcoord);
    %\addlegendentry{\scriptsize\(2 A \left(\mathbb{E}_{q_{\vlambda}} f_{\text{KL}} - f^*_{\text{KL}} \right)\)}

    \addplot[name path=ABC, color2, mark=none, thick]
      table [x=t, y=ABC] {data/simulation/airfoil_softplusmf_generalbound.csv}
      coordinate [pos=0.05] (ABCcoord1) coordinate [pos=0.95] (ABCcoord2);
    %\addlegendentry{\scriptsize\(2 A \left(F\left(\vlambda\right) - F^*\right) + B \norm{\nabla F}_2^2 + C\)}

    \addplot[name path=axis, domain=0:3990, fill=none, no markers, draw=none] {1e+3}
      coordinate [pos=0.05] (axiscoord);

    \addplot[name path=C, fill=none, gray, mark=none]
      table [x=t, y=C] {data/simulation/airfoil_softplusmf_generalbound.csv}
      coordinate [pos=0.05] (Ccoord);

    \addplot[thick, color=color3, fill=color3, fill opacity=0.2] fill between[of=ABC and opt];
    \addplot[thick, color=color2, fill=color2, fill opacity=0.2] fill between[of=ABC and   C];

    \addplot[thick, color=color1, fill=color1, fill opacity=0.2] fill between[of=opt and gvar];
    \addplot[thick, color=gray,   fill=gray,   fill opacity=0.2] fill between[of=C   and axis];

    \draw[thick,color=color3,draw=none,latex-latex] (ABCcoord2) -- (optcoord)
      node[midway,xshift=-20pt] {}
      coordinate [pos=0.5] (DKLcoord);

    \draw[thick,color=gray,latex-] (Ccoord) -- (axiscoord)
      node[pos=0.8,xshift=5pt] {\scriptsize\(C\) };

    \node[%
      pin={%
        [%
          pin distance=0.2cm,%
          pin edge={color3},%
          text=color3%
        ]110:{\scriptsize\(\DKL{q_{\vlambda}}{p}\)}},%
      inner sep=0pt,%
    ] at (DKLcoord) {};


==> figures/group_airfoil_squareroot_generalbound.tex <==

  \nextgroupplot[
      %% legend style={
      %%   legend image post style = {scale=0.5},
      %%   legend columns          = -1,
      %%   column sep              = 1em,
      %%   %at                     ={(0.5,1.5)},
      %%   anchor                  = north,
      %%   legend cell align       = left,
      %%   line width              = 0.8pt,
      %%   draw                    = none,
      %%   legend to name          = grouplegend
      %% },
      %
      tuftelike, 
      axis line style = thick,
      every tick/.style={black,thick},
      %axis lines = left,
      %grids=both,
      ymode  = log,
      xmin   = 1,
      xmax   = 4000,
      xtick  = {1, 2000, 4000},
      ytick  = {1e+3, 1e+5, 1e+7, 1e+9, 1e+11},
      %
      ymin   = 1e+3,
      ymax   = 1e+11,
      %
      xlabel = {Iteration},
      %ylabel = {\(\mathbb{E}\norm{\rvvg}^2_2\)},
      height = 5cm,
      width  = 4.7cm,
      axis on top,
    ]
    \addplot[name path=gvar, color1, mark=none, thick]
      table [x=t, y=gvar] {data/simulation/airfoil_squareroot_generalbound.csv}
      %node[above=3pt,pos=0.8] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
      coordinate [pos=0.95] (gvarcoord);
    %% \addlegendentry{\scriptsize\( \mathbb{E}\norm{ \rvvg }_2^2 \)}

    \addplot[name path=opt, color3, mark=none, thick] %
      table [x=t, y=opt] {data/simulation/airfoil_squareroot_generalbound.csv} %
      %node[above=3pt,pos=0.8] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)}
      coordinate [pos=0.95] (optcoord);
    %\addlegendentry{\scriptsize\(2 A \left(\mathbb{E}_{q_{\vlambda}} f_{\text{KL}} - f^*_{\text{KL}} \right)\)}

    \addplot[name path=ABC, color2, mark=none, thick]
      table [x=t, y=ABC] {data/simulation/airfoil_squareroot_generalbound.csv}
      coordinate [pos=0.05] (ABCcoord1) coordinate [pos=0.95] (ABCcoord2);
    %% \addlegendentry{\scriptsize\(2 A \left(F\left(\vlambda\right) - F^*\right) + B \norm{\nabla F}_2^2 + C\)}

    \addplot[name path=axis, domain=0:3990, fill=none, no markers, draw=none] {1e+3}
      coordinate [pos=0.05] (axiscoord);

    \addplot[name path=C, fill=none, gray, mark=none]
      table [x=t, y=C] {data/simulation/airfoil_squareroot_generalbound.csv}
      coordinate [pos=0.05] (Ccoord);

    \addplot[thick, color=color3, fill=color3, fill opacity=0.2] fill between[of=ABC and opt];
    \addplot[thick, color=color2, fill=color2, fill opacity=0.2] fill between[of=ABC and   C];

    \addplot[thick, color=color1, fill=color1, fill opacity=0.2] fill between[of=opt and gvar];
    \addplot[thick, color=gray,   fill=gray,   fill opacity=0.2] fill between[of=C   and axis];

    \draw[thick,color=color3,draw=none,latex-latex] (ABCcoord2) -- (optcoord)
      node[midway,xshift=-20pt] {}
      coordinate [pos=0.5] (DKLcoord);

    \draw[thick,color=gray,latex-] (Ccoord) -- (axiscoord)
      node[pos=0.8,xshift=5pt] {\scriptsize\(C\) };

    \node[%
      pin={%
        [%
          pin distance=0.3cm,%
          pin edge={color3},%
          text=color3%
        ]100:{\scriptsize\(\DKL{q_{\vlambda}}{p}\)}},%
      inner sep=0pt,%
    ] at (DKLcoord) {};


==> figures/group_fertility_linearchol_generalbound.tex <==

  \nextgroupplot[
      legend style={
        legend image post style = {scale=0.5},
        legend columns          = -1,
        column sep              = 1em,
        %at                     ={(0.5,1.5)},
        anchor                  = north,
        legend cell align       = left,
        line width              = 0.8pt,
        draw                    = none,
        legend to name          = grouplegend
      },
      %
      tuftelike, 
      axis line style = thick,
      every tick/.style={black,thick},
      %axis lines = left,
      %grids=both,
      ymode  = log,
      xmin   = 1,
      xmax   = 500,
      xtick  = {1, 100, 200, 300, 400, 500},
      ytick  = {1e+2, 1e+4, 1e+6, 1e+8},
      %
      ymin   = 1e+2,
      ymax   = 1e+8,
      %
      xlabel = {Iteration},
      %ylabel = {\(\mathbb{E}\norm{\rvvg}^2_2\)},
      height = 5cm,
      width  = 4.7cm,
      axis on top,
    ]
    \addplot[name path=gvar, color1, mark=none, thick]
      table [x=t, y=gvar] {data/simulation/fertility_linearchol_generalbound.csv}
      %node[above=3pt,pos=0.8] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
      coordinate [pos=0.95] (gvarcoord);
    \addlegendentry{\scriptsize\( \mathbb{E}\norm{ \rvvg }_2^2 \)}

    \addplot[name path=ABC, color2, mark=none, thick]
      table [x=t, y=ABC] {data/simulation/fertility_linearchol_generalbound.csv}
      coordinate [pos=0.05] (ABCcoord1) coordinate [pos=0.95] (ABCcoord2);
    \addlegendentry{\scriptsize\(2 A \left(F\left(\vlambda\right) - F^*\right) + B \norm{\nabla F}_2^2 + C\)}

    \addplot[name path=opt, color3, mark=none, thick] %
      table [x=t, y=opt] {data/simulation/fertility_linearchol_generalbound.csv} %
      %node[above=3pt,pos=0.8] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)}
      coordinate [pos=0.95] (optcoord);
    %\addlegendentry{\scriptsize\(2 A \left(\mathbb{E}_{q_{\vlambda}} f_{\text{KL}} - f^*_{\text{KL}} \right)\)}

    \addplot[name path=axis, domain=0:490, fill=none, no markers, draw=none] {1e+2}
      coordinate [pos=0.05] (axiscoord);

    \addplot[name path=C, fill=none, gray, mark=none]
      table [x=t, y=C] {data/simulation/fertility_linearchol_generalbound.csv}
      coordinate [pos=0.05] (Ccoord);

    \addplot[thick, color=color3, fill=color3, fill opacity=0.2] fill between[of=ABC and opt];
    \addplot[thick, color=color2, fill=color2, fill opacity=0.2] fill between[of=ABC and   C];

    \addplot[thick, color=color1, fill=color1, fill opacity=0.2] fill between[of=opt and gvar];
    \addplot[thick, color=gray,   fill=gray,   fill opacity=0.2] fill between[of=C   and axis];

    \draw[thick,color=color3,latex-latex] (ABCcoord2) -- (optcoord)
      node[midway,xshift=-20pt] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)};

    \draw[thick,color=gray,latex-] (Ccoord) -- (axiscoord)
      node[midway,xshift=5pt] {\scriptsize\(C\) };


==> figures/group_fertility_softpluschol_generalbound.tex <==

  \nextgroupplot[
      legend style={
        legend image post style = {scale=0.5},
        legend columns          = -1,
        column sep              = 1em,
        %at                     ={(0.5,1.5)},
        anchor                  = north,
        legend cell align       = left,
        line width              = 0.8pt,
        draw                    = none,
        legend to name          = grouplegend
      },
      %
      tuftelike, 
      axis line style = thick,
      every tick/.style={black,thick},
      %axis lines = left,
      %grids=both,
      ymode  = log,
      xmin   = 1,
      xmax   = 4000,
      xtick  = {1, 1000, 2000, 3000, 4000},
      ytick  = {1e+2, 1e+4, 1e+6, 1e+8},
      %
      ymin   = 1e+2,
      ymax   = 1e+8,
      %
      xlabel = {Iteration},
      %ylabel = {\(\mathbb{E}\norm{\rvvg}^2_2\)},
      height = 4.5cm,
      width  = 5cm,
      axis on top,
    ]
    \addplot[name path=gvar, color1, mark=none, thick]
      table [x=t, y=gvar] {data/simulation/fertility_softpluschol_generalbound.csv}
      %node[above=3pt,pos=0.8] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
      coordinate [pos=0.95] (gvarcoord);
    \addlegendentry{\scriptsize\( \mathbb{E}\norm{ \rvvg }_2^2 \)}

    \addplot[name path=ABC, color2, mark=none, thick]
      table [x=t, y=ABC] {data/simulation/fertility_softpluschol_generalbound.csv}
      coordinate [pos=0.05] (ABCcoord1) coordinate [pos=0.95] (ABCcoord2);
    \addlegendentry{\scriptsize\(2 A \left(F\left(\vlambda\right) - F^*\right) + B \norm{\nabla F}_2^2 + C\)}

    \addplot[name path=opt, color3, mark=none, thick] %
      table [x=t, y=opt] {data/simulation/fertility_softpluschol_generalbound.csv} %
      %node[above=3pt,pos=0.8] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)}
      coordinate [pos=0.95] (optcoord);
    %\addlegendentry{\scriptsize\(2 A \left(\mathbb{E}_{q_{\vlambda}} f_{\text{KL}} - f^*_{\text{KL}} \right)\)}

    \addplot[name path=axis, domain=0:3990, fill=none, no markers, draw=none] {1e+2}
      coordinate [pos=0.05] (axiscoord);

    \addplot[name path=C, fill=none, gray, mark=none]
      table [x=t, y=C] {data/simulation/fertility_softpluschol_generalbound.csv}
      coordinate [pos=0.05] (Ccoord);

    \addplot[thick, color=color3, fill=color3, fill opacity=0.2] fill between[of=ABC and opt];
    \addplot[thick, color=color2, fill=color2, fill opacity=0.2] fill between[of=ABC and   C];

    \addplot[thick, color=color1, fill=color1, fill opacity=0.2] fill between[of=opt and gvar];
    \addplot[thick, color=gray,   fill=gray,   fill opacity=0.2] fill between[of=C   and axis];

    \draw[thick,color=color3,latex-latex] (ABCcoord2) -- (optcoord)
      node[midway,xshift=-20pt] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)};

    \draw[thick,color=gray,latex-] (Ccoord) -- (axiscoord)
      node[pos=0.8,xshift=5pt] {\scriptsize\(C\) };


==> figures/group_fertility_softplusmf_generalbound.tex <==

  \nextgroupplot[
      legend style={
        legend image post style = {scale=0.5},
        legend columns          = -1,
        column sep              = 1em,
        %at                     ={(0.5,1.5)},
        anchor                  = north,
        legend cell align       = left,
        line width              = 0.8pt,
        draw                    = none,
        legend to name          = grouplegend
      },
      %
      tuftelike, 
      axis line style = thick,
      every tick/.style={black,thick},
      %axis lines = left,
      %grids=both,
      ymode  = log,
      xmin   = 1,
      xmax   = 4000,
      xtick  = {1, 2000, 4000},
      ytick  = {1e+2, 1e+4, 1e+6, 1e+8},
      %
      ymin   = 1e+2,
      ymax   = 1e+8,
      %
      xlabel = {Iteration},
      %ylabel = {\(\mathbb{E}\norm{\rvvg}^2_2\)},
      height = 5cm,
      width  = 4.7cm,
      axis on top,
    ]
    \addplot[name path=gvar, color1, mark=none, thick]
      table [x=t, y=gvar] {data/simulation/fertility_softplusmf_generalbound.csv}
      %node[above=3pt,pos=0.8] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
      coordinate [pos=0.95] (gvarcoord);
    \addlegendentry{\scriptsize\( \mathbb{E}\norm{ \rvvg }_2^2 \)}

    \addplot[name path=ABC, color2, mark=none, thick]
      table [x=t, y=ABC] {data/simulation/fertility_softplusmf_generalbound.csv}
      coordinate [pos=0.05] (ABCcoord1) coordinate [pos=0.95] (ABCcoord2);
    \addlegendentry{\scriptsize\(2 A \left(F\left(\vlambda\right) - F^*\right) + B \norm{\nabla F}_2^2 + C\)}

    \addplot[name path=opt, color3, mark=none, thick] %
      table [x=t, y=opt] {data/simulation/fertility_softplusmf_generalbound.csv} %
      %node[above=3pt,pos=0.8] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)}
      coordinate [pos=0.95] (optcoord);
    %\addlegendentry{\scriptsize\(2 A \left(\mathbb{E}_{q_{\vlambda}} f_{\text{KL}} - f^*_{\text{KL}} \right)\)}

    \addplot[name path=axis, domain=0:3990, fill=none, no markers, draw=none] {1e+2}
      coordinate [pos=0.05] (axiscoord);

    \addplot[name path=C, fill=none, gray, mark=none]
      table [x=t, y=C] {data/simulation/fertility_softplusmf_generalbound.csv}
      coordinate [pos=0.05] (Ccoord);

    \addplot[thick, color=color3, fill=color3, fill opacity=0.2] fill between[of=ABC and opt];
    \addplot[thick, color=color2, fill=color2, fill opacity=0.2] fill between[of=ABC and   C];

    \addplot[thick, color=color1, fill=color1, fill opacity=0.2] fill between[of=opt and gvar];
    \addplot[thick, color=gray,   fill=gray,   fill opacity=0.2] fill between[of=C   and axis];

    \draw[thick,color=color3,latex-latex] (ABCcoord2) -- (optcoord)
      node[midway,xshift=-20pt] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)};

    \draw[thick,color=gray,latex-] (Ccoord) -- (axiscoord)
      node[pos=0.8,xshift=5pt] {\scriptsize\(C\) };


==> figures/group_fertility_squareroot_generalbound.tex <==

  \nextgroupplot[
      legend style={
        legend image post style = {scale=0.5},
        legend columns          = -1,
        column sep              = 1em,
        %at                     ={(0.5,1.5)},
        anchor                  = center,
        legend cell align       = left,
        line width              = 0.8pt,
        draw                    = none,
        legend to name          = grouplegend
      },
      %
      tuftelike, 
      axis line style = thick,
      every tick/.style={black,thick},
      %axis lines = left,
      %grids=both,
      ymode  = log,
      xmin   = 1,
      xmax   = 4000,
      xtick  = {1, 2000, 4000},
      ytick  = {1e+2, 1e+4, 1e+6, 1e+8},
      %
      ymin   = 1e+2,
      ymax   = 1e+8,
      %
      xlabel = {Iteration},
      %ylabel = {\(\mathbb{E}\norm{\rvvg}^2_2\)},
      height = 5cm,
      width  = 4.7cm,
      axis on top,
    ]
    \addplot[name path=gvar, color1, mark=none, thick]
      table [x=t, y=gvar] {data/simulation/fertility_squareroot_generalbound.csv}
      %node[above=3pt,pos=0.8] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
      coordinate [pos=0.95] (gvarcoord);
    \addlegendentry{\scriptsize\( \mathbb{E}\norm{ \rvvg }_2^2 \)}

    \addplot[name path=ABC, color2, mark=none, thick]
      table [x=t, y=ABC] {data/simulation/fertility_squareroot_generalbound.csv}
      coordinate [pos=0.05] (ABCcoord1) coordinate [pos=0.95] (ABCcoord2);
    \addlegendentry{\scriptsize\(2 A \left(F\left(\vlambda\right) - F^*\right) + B \norm{\nabla F}_2^2 + C\)}

    \addplot[name path=opt, color3, mark=none, thick] %
      table [x=t, y=opt] {data/simulation/fertility_squareroot_generalbound.csv} %
      %node[above=3pt,pos=0.8] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)}
      coordinate [pos=0.95] (optcoord);
    %\addlegendentry{\scriptsize\(2 A \left(\mathbb{E}_{q_{\vlambda}} f_{\text{KL}} - f^*_{\text{KL}} \right)\)}

    \addplot[name path=axis, domain=0:3990, fill=none, no markers, draw=none] {1e+2}
      coordinate [pos=0.05] (axiscoord);

    \addplot[name path=C, fill=none, gray, mark=none]
      table [x=t, y=C] {data/simulation/fertility_squareroot_generalbound.csv}
      coordinate [pos=0.05] (Ccoord);

    \addplot[thick, color=color3, fill=color3, fill opacity=0.2] fill between[of=ABC and opt];
    \addplot[thick, color=color2, fill=color2, fill opacity=0.2] fill between[of=ABC and   C];

    \addplot[thick, color=color1, fill=color1, fill opacity=0.2] fill between[of=opt and gvar];
    \addplot[thick, color=gray,   fill=gray,   fill opacity=0.2] fill between[of=C   and axis];

    \draw[thick,color=color3,latex-latex] (ABCcoord2) -- (optcoord)
      node[midway,xshift=-20pt] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)};

    \draw[thick,color=gray,latex-] (Ccoord) -- (axiscoord)
      node[pos=0.7,xshift=5pt] {\scriptsize\(C\) };


==> figures/group_pendulum_linearchol_generalbound.tex <==

  \nextgroupplot[
      %% legend style={
      %%   legend image post style = {scale=0.5},
      %%   legend columns          = -1,
      %%   column sep              = 1em,
      %%   %at                     ={(0.5,1.5)},
      %%   anchor                  = north,
      %%   legend cell align       = left,
      %%   line width              = 0.8pt,
      %%   draw                    = none,
      %%   legend to name          = grouplegend
      %% },
      %
      tuftelike, 
      axis line style = thick,
      every tick/.style={black,thick},
      %axis lines = left,
      %grids=both,
      ymode  = log,
      xmin   = 1,
      xmax   = 500,
      xtick  = {1, 100, 200, 300, 400, 500},
      ytick  = {1e+3, 1e+5, 1e+7, 1e+9, 1e+11},
      %
      ymin   = 1e+3,
      ymax   = 1e+11,
      %
      xlabel = {Iteration},
      %ylabel = {\(\mathbb{E}\norm{\rvvg}^2_2\)},
      height = 5cm,
      width  = 4.7cm,
      axis on top,
    ]
    \addplot[name path=gvar, color1, mark=none, thick]
      table [x=t, y=gvar] {data/simulation/pendulum_linearchol_generalbound.csv}
      %node[above=3pt,pos=0.8] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
      coordinate [pos=0.95] (gvarcoord);
    %\addlegendentry{\scriptsize\( \mathbb{E}\norm{ \rvvg }_2^2 \)}

    \addplot[name path=opt, color3, mark=none, thick] %
      table [x=t, y=opt] {data/simulation/pendulum_linearchol_generalbound.csv} %
      %node[above=3pt,pos=0.8] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)}
      coordinate [pos=0.95] (optcoord);
    %\addlegendentry{\scriptsize\(2 A \left(\mathbb{E}_{q_{\vlambda}} f_{\text{KL}} - f^*_{\text{KL}} \right)\)}

    \addplot[name path=ABC, color2, mark=none, thick]
      table [x=t, y=ABC] {data/simulation/pendulum_linearchol_generalbound.csv}
      coordinate [pos=0.05] (ABCcoord1) coordinate [pos=0.95] (ABCcoord2);
    %\addlegendentry{\scriptsize\(2 A \left(F\left(\vlambda\right) - F^*\right) + B \norm{\nabla F}_2^2 + C\)}

    \addplot[name path=axis, domain=0:490, fill=none, no markers, draw=none] {1e+3}
      coordinate [pos=0.05] (axiscoord);

    \addplot[name path=C, fill=none, gray, mark=none]
      table [x=t, y=C] {data/simulation/pendulum_linearchol_generalbound.csv}
      coordinate [pos=0.05] (Ccoord);

    \addplot[thick, color=color3, fill=color3, fill opacity=0.2] fill between[of=ABC and opt];
    \addplot[thick, color=color2, fill=color2, fill opacity=0.2] fill between[of=ABC and   C];

    \addplot[thick, color=color1, fill=color1, fill opacity=0.2] fill between[of=opt and gvar];
    \addplot[thick, color=gray,   fill=gray,   fill opacity=0.2] fill between[of=C   and axis];

    \draw[thick,color=color3,latex-latex] (ABCcoord2) -- (optcoord)
      node[midway,xshift=-20pt] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)};

    \draw[thick,color=gray,latex-] (Ccoord) -- (axiscoord)
      node[midway,xshift=5pt] {\scriptsize\(C\) };


==> figures/group_pendulum_softpluschol_generalbound.tex <==

  \nextgroupplot[
      %% legend style={
      %%   legend image post style = {scale=0.5},
      %%   legend columns          = -1,
      %%   column sep              = 1em,
      %%   %at                     ={(0.5,1.5)},
      %%   anchor                  = north,
      %%   legend cell align       = left,
      %%   line width              = 0.8pt,
      %%   draw                    = none,
      %%   legend to name          = grouplegend
      %% },
      %
      tuftelike, 
      axis line style = thick,
      every tick/.style={black,thick},
      %axis lines = left,
      %grids=both,
      ymode  = log,
      xmin   = 1,
      xmax   = 4000,
      xtick  = {1, 1000, 2000, 3000, 4000},
      ytick  = {1e+3, 1e+5, 1e+7, 1e+9, 1e+11},
      %
      ymin   = 1e+3,
      ymax   = 1e+11,
      %
      xlabel = {Iteration},
      %ylabel = {\(\mathbb{E}\norm{\rvvg}^2_2\)},
      height = 4.5cm,
      width  = 5cm,
      axis on top,
    ]
    \addplot[name path=gvar, color1, mark=none, thick]
      table [x=t, y=gvar] {data/simulation/pendulum_softpluschol_generalbound.csv}
      %node[above=3pt,pos=0.8] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
      coordinate [pos=0.95] (gvarcoord);
    %\addlegendentry{\scriptsize\( \mathbb{E}\norm{ \rvvg }_2^2 \)}

    \addplot[name path=opt, color3, mark=none, thick] %
      table [x=t, y=opt] {data/simulation/pendulum_softpluschol_generalbound.csv} %
      %node[above=3pt,pos=0.8] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)}
      coordinate [pos=0.95] (optcoord);
    %\addlegendentry{\scriptsize\(2 A \left(\mathbb{E}_{q_{\vlambda}} f_{\text{KL}} - f^*_{\text{KL}} \right)\)}

    \addplot[name path=ABC, color2, mark=none, thick]
      table [x=t, y=ABC] {data/simulation/pendulum_softpluschol_generalbound.csv}
      coordinate [pos=0.05] (ABCcoord1) coordinate [pos=0.95] (ABCcoord2);
    %\addlegendentry{\scriptsize\(2 A \left(F\left(\vlambda\right) - F^*\right) + B \norm{\nabla F}_2^2 + C\)}

    \addplot[name path=axis, domain=0:3990, fill=none, no markers, draw=none] {1e+3}
      coordinate [pos=0.05] (axiscoord);

    \addplot[name path=C, fill=none, gray, mark=none]
      table [x=t, y=C] {data/simulation/pendulum_softpluschol_generalbound.csv}
      coordinate [pos=0.05] (Ccoord);

    \addplot[thick, color=color3, fill=color3, fill opacity=0.2] fill between[of=ABC and opt];
    \addplot[thick, color=color2, fill=color2, fill opacity=0.2] fill between[of=ABC and   C];

    \addplot[thick, color=color1, fill=color1, fill opacity=0.2] fill between[of=opt and gvar];
    \addplot[thick, color=gray,   fill=gray,   fill opacity=0.2] fill between[of=C   and axis];

    \draw[thick,color=color3,draw=none,latex-latex] (ABCcoord2) -- (optcoord)
      node[midway,xshift=-20pt] {}
      coordinate [pos=0.5] (DKLcoord);

    \draw[thick,color=gray,latex-] (Ccoord) -- (axiscoord)
      node[pos=0.8,xshift=5pt] {\scriptsize\(C\) };

    \node[%
      pin={%
        [%
          pin distance=0.2cm,%
          pin edge={color3},%
          text=color3%
        ]110:{\scriptsize\(\DKL{q_{\vlambda}}{p}\)}},%
      inner sep=0pt,%
    ] at (DKLcoord) {};


==> figures/group_pendulum_softplusmf_generalbound.tex <==

  \nextgroupplot[
      %% legend style={
      %%   legend image post style = {scale=0.5},
      %%   legend columns          = -1,
      %%   column sep              = 1em,
      %%   %at                     ={(0.5,1.5)},
      %%   anchor                  = north,
      %%   legend cell align       = left,
      %%   line width              = 0.8pt,
      %%   draw                    = none,
      %%   legend to name          = grouplegend
      %% },
      %
      tuftelike, 
      axis line style = thick,
      every tick/.style={black,thick},
      %axis lines = left,
      %grids=both,
      ymode  = log,
      xmin   = 1,
      xmax   = 4000,
      xtick  = {1, 2000, 4000},
      ytick  = {1e+3, 1e+5, 1e+7, 1e+9, 1e+11},
      %
      ymin   = 1e+3,
      ymax   = 1e+11,
      %
      xlabel = {Iteration},
      %ylabel = {\(\mathbb{E}\norm{\rvvg}^2_2\)},
      height = 5cm,
      width  = 4.7cm,
      axis on top,
    ]
    \addplot[name path=gvar, color1, mark=none, thick]
      table [x=t, y=gvar] {data/simulation/pendulum_softplusmf_generalbound.csv}
      %node[above=3pt,pos=0.8] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
      coordinate [pos=0.95] (gvarcoord);
    %\addlegendentry{\scriptsize\( \mathbb{E}\norm{ \rvvg }_2^2 \)}

    \addplot[name path=opt, color3, mark=none, thick] %
      table [x=t, y=opt] {data/simulation/pendulum_softplusmf_generalbound.csv} %
      %node[above=3pt,pos=0.8] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)}
      coordinate [pos=0.95] (optcoord);
    %\addlegendentry{\scriptsize\(2 A \left(\mathbb{E}_{q_{\vlambda}} f_{\text{KL}} - f^*_{\text{KL}} \right)\)}

    \addplot[name path=ABC, color2, mark=none, thick]
      table [x=t, y=ABC] {data/simulation/pendulum_softplusmf_generalbound.csv}
      coordinate [pos=0.05] (ABCcoord1) coordinate [pos=0.95] (ABCcoord2);
    %\addlegendentry{\scriptsize\(2 A \left(F\left(\vlambda\right) - F^*\right) + B \norm{\nabla F}_2^2 + C\)}

    \addplot[name path=axis, domain=0:3990, fill=none, no markers, draw=none] {1e+3}
      coordinate [pos=0.05] (axiscoord);

    \addplot[name path=C, fill=none, gray, mark=none]
      table [x=t, y=C] {data/simulation/pendulum_softplusmf_generalbound.csv}
      coordinate [pos=0.05] (Ccoord);

    \addplot[thick, color=color3, fill=color3, fill opacity=0.2] fill between[of=ABC and opt];
    \addplot[thick, color=color2, fill=color2, fill opacity=0.2] fill between[of=ABC and   C];

    \addplot[thick, color=color1, fill=color1, fill opacity=0.2] fill between[of=opt and gvar];
    \addplot[thick, color=gray,   fill=gray,   fill opacity=0.2] fill between[of=C   and axis];

    \draw[thick,color=color3,draw=none,latex-latex] (ABCcoord2) -- (optcoord)
      node[midway,xshift=-20pt] {}
      coordinate [pos=0.5] (DKLcoord);

    \draw[thick,color=gray,latex-] (Ccoord) -- (axiscoord)
      node[pos=0.8,xshift=5pt] {\scriptsize\(C\) };

    \node[%
      pin={%
        [%
          pin distance=0.2cm,%
          pin edge={color3},%
          text=color3%
        ]110:{\scriptsize\(\DKL{q_{\vlambda}}{p}\)}},%
      inner sep=0pt,%
    ] at (DKLcoord) {};


==> figures/group_pendulum_squareroot_generalbound.tex <==

  \nextgroupplot[
      %% legend style={
      %%   legend image post style = {scale=0.5},
      %%   legend columns          = -1,
      %%   column sep              = 1em,
      %%   %at                     ={(0.5,1.5)},
      %%   anchor                  = north,
      %%   legend cell align       = left,
      %%   line width              = 0.8pt,
      %%   draw                    = none,
      %%   legend to name          = grouplegend
      %% },
      %
      tuftelike, 
      axis line style = thick,
      every tick/.style={black,thick},
      %axis lines = left,
      %grids=both,
      ymode  = log,
      xmin   = 1,
      %xmax   = 500,
      xtick  = {1, 1000, 2000},
      ytick  = {1e+3, 1e+5, 1e+7, 1e+9, 1e+11},
      %
      ymin   = 1e+3,
      ymax   = 1e+11,
      %
      xlabel = {Iteration},
      %ylabel = {\(\mathbb{E}\norm{\rvvg}^2_2\)},
      height = 5cm,
      width  = 4.7cm,
      axis on top,
    ]
    \addplot[name path=gvar, color1, mark=none, thick]
      table [x=t, y=gvar] {data/simulation/pendulum_squareroot_generalbound.csv}
      %node[above=3pt,pos=0.8] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
      coordinate [pos=0.95] (gvarcoord);
    %% \addlegendentry{\scriptsize\( \mathbb{E}\norm{ \rvvg }_2^2 \)}

    \addplot[name path=ABC, color2, mark=none, thick]
      table [x=t, y=ABC] {data/simulation/pendulum_squareroot_generalbound.csv}
      coordinate [pos=0.05] (ABCcoord1) coordinate [pos=0.95] (ABCcoord2);
    %% \addlegendentry{\scriptsize\(2 A \left(F\left(\vlambda\right) - F^*\right) + B \norm{\nabla F}_2^2 + C\)}

    \addplot[name path=opt, color3, mark=none, thick] %
      table [x=t, y=opt] {data/simulation/pendulum_squareroot_generalbound.csv} %
      %node[above=3pt,pos=0.8] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)}
      coordinate [pos=0.95] (optcoord);
    %\addlegendentry{\scriptsize\(2 A \left(\mathbb{E}_{q_{\vlambda}} f_{\text{KL}} - f^*_{\text{KL}} \right)\)}

    \addplot[name path=axis, domain=0:1990, fill=none, no markers, draw=none] {1e+3}
      coordinate [pos=0.05] (axiscoord);

    \addplot[name path=C, fill=none, gray, mark=none]
      table [x=t, y=C] {data/simulation/pendulum_squareroot_generalbound.csv}
      coordinate [pos=0.05] (Ccoord);

    \addplot[thick, color=color3, fill=color3, fill opacity=0.2] fill between[of=ABC and opt];
    \addplot[thick, color=color2, fill=color2, fill opacity=0.2] fill between[of=ABC and   C];

    \addplot[thick, color=color1, fill=color1, fill opacity=0.2] fill between[of=opt and gvar];
    \addplot[thick, color=gray,   fill=gray,   fill opacity=0.2] fill between[of=C   and axis];

    \draw[thick,color=color3,draw=none,latex-latex] (ABCcoord2) -- (optcoord)
      node[midway,xshift=-20pt] {}
      coordinate [pos=0.5] (DKLcoord);

    \draw[thick,color=gray,latex-] (Ccoord) -- (axiscoord)
      node[pos=0.8,xshift=5pt] {\scriptsize\(C\) };

    \node[%
      pin={%
        [%
          pin distance=0.3cm,%
          pin edge={color3},%
          text=color3%
        ]100:{\scriptsize\(\DKL{q_{\vlambda}}{p}\)}},%
      inner sep=0pt,%
    ] at (DKLcoord) {};


==> figures/group_quadratic_linearchol_boundedentropy.tex <==

% Tikz examples & demos
% https://holatex.app/examples.html?package=tikz

  \nextgroupplot[
      %
      tuftelike, 
      axis line style = thick,
      every tick/.style={black,thick},
      %axis lines = left,
      %grids=both,
      ymode  = log,
      xmin   = 1,
      xmax   = 500,
      xtick  = {1, 100, 200, 300, 400, 500},
      ytick  = {1e+4, 1e+5, 1e+6, 1e+7, 1e+8, 1e+9},
      %
      ymin   = 1e+4,
      ymax   = 1e+9,
      %
      xlabel = {Iteration},
      %ylabel = {\(\mathbb{E}\norm{\rvvg}^2_2\)},
      height = 4.5cm,
      width  = 4.7cm,
      axis on top,
    ]
    \addplot[name path=gvar, color1, mark=none, thick]
      table [x=t, y=gvar] {data/simulation/quadratic_linearchol_boundedentropybound.csv}
      %node[above=3pt,pos=0.8] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
      coordinate [pos=0.95] (gvarcoord);
    %\addlegendentry{\scriptsize\( \mathbb{E}\norm{ \rvvg }_2^2 \)}

    \addplot[name path=opt, color3, mark=none, thick] %
      table [x=t, y=opt] {data/simulation/quadratic_linearchol_boundedentropybound.csv} %
      %node[above=3pt,pos=0.8] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)}
      coordinate [pos=0.95] (optcoord);
    %\addlegendentry{\scriptsize\(2 A \left(\mathbb{E}_{q_{\vlambda}} f_{\mathrm{H}} - f^*_{\mathrm{H}}\right)\)}

    \addplot[name path=ABC, color2, mark=none, thick]
      table [x=t, y=ABC] {data/simulation/quadratic_linearchol_boundedentropybound.csv}
      coordinate [pos=0.05] (ABCcoord1) coordinate [pos=0.95] (ABCcoord2);
    %\addlegendentry{\scriptsize\(2 A \left(F\left(\vlambda\right) - F^*\right) + B \norm{\nabla F}_2^2 + C\)}

    \addplot[name path=axis, domain=0:490, fill=none, no markers, draw=none] {1e+4}
      coordinate [pos=0.05] (axiscoord);

    %\addplot[name path=ABC, color2, mark=none]
    %  table [x=t, y=ABC] {figures/quadratic_linearchol_boundedentropybound.csv}
    %  ;

    \addplot[name path=C, fill=none, gray, mark=none]
      table [x=t, y=C] {data/simulation/quadratic_linearchol_boundedentropybound.csv}
      coordinate [pos=0.05] (Ccoord);

    \addplot[thick, color=color3, fill=color3, fill opacity=0.2] fill between[of=ABC and opt];
    \addplot[thick, color=color2, fill=color2, fill opacity=0.2] fill between[of=ABC and   C];

    \addplot[thick, color=color1, fill=color1, fill opacity=0.2] fill between[of=opt and gvar];
    \addplot[thick, color=gray,   fill=gray,   fill opacity=0.2] fill between[of=C   and axis];

    \draw[thick,color=color3, latex-latex] (ABCcoord2) -- (optcoord)
      node[midway,xshift=-25pt] {\scriptsize\(h\left(\vlambda\right) - h^*\)}
      coordinate [pos=0.5] (dklarrow_coord);

    %\draw[thick,color=color1] (gvarcoord) -- (optcoord)
    %  %node[midway,xshift=-25pt] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
    %  coordinate [pos=0.5] (muL_coord);

    \draw[thick,color=gray,latex-] (Ccoord) -- (axiscoord)
      node[midway,xshift=5pt] {\scriptsize\(C\) };

    %% \node[%
    %%   pin={%
    %%     [%
    %%       pin distance=1cm,%
    %%       pin edge={color3},%
    %%       text=color3%
    %%     ]100:{\scriptsize\( h\left(\vlambda\right) - h^*\)}%
    %%   },%
    %%   inner sep=0pt,
    %% ] at (dklarrow_coord) {};

    %% \node[%
    %%   pin={%
    %%     [%
    %%       pin distance=1cm,%
    %%       pin edge={color1},%
    %%       text=color1%
    %%     ]130:{\scriptsize\(\mu_{\mathrm{H}}, L_{\mathrm{H}}\) bound}},%
    %%   inner sep=0pt,%
    %% ] at (muL_coord) {};


    %\draw[thick,color=color2,latex-latex] (ABCcoord1) -- (Ccoord)
    %  node[midway,xshift=25pt] {\scriptsize\(2 A \left( F\left(\lambda\right) - F^* \right)\) };
  %$\end{axis}


==> figures/group_quadratic_linearchol_generalbound.tex <==

% Tikz examples & demos
% https://holatex.app/examples.html?package=tikz

  \nextgroupplot[
      legend style={
        legend image post style = {scale=0.5},
        legend columns          = -1,
        column sep              = 1em,
        %at                     ={(0.5,1.5)},
        anchor                  = north,
        legend cell align       = left,
        line width              = 0.8pt,
        draw                    = none,
        legend to name          = grouplegend
      },
      %
      tuftelike, 
      axis line style = thick,
      every tick/.style={black,thick},
      %axis lines = left,
      %grids=both,
      ymode  = log,
      xmin   = 1,
      xmax   = 500,
      xtick  = {1, 100, 200, 300, 400, 500},
      ytick  = {1e+4, 1e+5, 1e+6, 1e+7, 1e+8, 1e+9},
      %
      ymin   = 1e+4,
      ymax   = 1e+9,
      %
      xlabel = {Iteration},
      %ylabel = {\(\mathbb{E}\norm{\rvvg}^2_2\)},
      height = 4.5cm,
      width  = 4.7cm,
      axis on top,
    ]
    \addplot[name path=gvar, color1, mark=none, thick]
      table [x=t, y=gvar] {data/simulation/quadratic_linearchol_generalbound.csv}
      %node[above=3pt,pos=0.8] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
      coordinate [pos=0.95] (gvarcoord);
    \addlegendentry{\scriptsize\( \mathbb{E}\norm{ \rvvg }_2^2 \)}

    \addplot[name path=ABC, color2, mark=none, thick]
      table [x=t, y=ABC] {data/simulation/quadratic_linearchol_generalbound.csv}
      coordinate [pos=0.05] (ABCcoord1) coordinate [pos=0.95] (ABCcoord2);
    \addlegendentry{\scriptsize\(2 A \left(F\left(\vlambda\right) - F^*\right) + B \norm{\nabla F}_2^2 + C\)}

    \addplot[name path=opt, color3, mark=none, thick] %
      table [x=t, y=opt] {data/simulation/quadratic_linearchol_generalbound.csv} %
      %node[above=3pt,pos=0.8] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)}
      coordinate [pos=0.95] (optcoord);
    %\addlegendentry{\scriptsize\(2 A \left(\mathbb{E}_{q_{\vlambda}} f_{\text{KL}} - f^*_{\text{KL}} \right)\)}

    \addplot[name path=axis, domain=0:490, fill=none, no markers, draw=none] {1e+4}
      coordinate [pos=0.05] (axiscoord);

    %\addplot[name path=ABC, color2, mark=none]
    %  table [x=t, y=ABC] {data/simulation/quadratic_linearchol_generalbound.csv}
    %  ;

    \addplot[name path=C, fill=none, gray, mark=none]
      table [x=t, y=C] {data/simulation/quadratic_linearchol_generalbound.csv}
      coordinate [pos=0.05] (Ccoord);

    \addplot[thick, color=color3, fill=color3, fill opacity=0.2] fill between[of=ABC and opt];
    \addplot[thick, color=color2, fill=color2, fill opacity=0.2] fill between[of=ABC and   C];

    \addplot[thick, color=color1, fill=color1, fill opacity=0.2] fill between[of=opt and gvar];
    \addplot[thick, color=gray,   fill=gray,   fill opacity=0.2] fill between[of=C   and axis];

    \draw[thick,color=color3,latex-latex] (ABCcoord2) -- (optcoord)
      node[midway,xshift=-20pt] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)};

    %\draw[thick,color=color1] (gvarcoord) -- (optcoord)
      %node[midway,xshift=-32pt] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}, \Delta \vz^*\) bound}
    %  coordinate [pos=0.5] (muL_coord);

    \draw[thick,color=gray,latex-] (Ccoord) -- (axiscoord)
      node[midway,xshift=5pt] {\scriptsize\(C\) };

    %\draw[thick,color=color2,latex-latex] (ABCcoord1) -- (Ccoord)
    %  node[midway,xshift=25pt] {\scriptsize\(2 A \left( F\left(\lambda\right) - F^* \right)\) };

%%     \node[%
%%       pin={%
%%         [%
%%           pin distance=0.45cm,%
%%           pin edge={color1},%
%%           text=color1%
%%         ]263:{\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}, \Delta \vz^* \) bound}},%
%%       inner sep=0pt,%
%%     ] at (muL_coord) {};

%%     \node[%
%%       pin={%
%%         [%
%%           pin distance=1.8cm,%
%%           pin edge={color1},%
%%           text=color1%
%%         ]92:{\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}},%
%%       inner sep=0pt,%
%%     ] at (muL_coord) {};



==> figures/group_quadratic_linearmf_boundedentropy.tex <==

% Tikz examples & demos
% https://holatex.app/examples.html?package=tikz

  \nextgroupplot[
      legend style={
        legend image post style={scale=0.5},
        at={(0.5,1.5)},
        anchor=north,
        legend cell align=left,
        line width=0.8pt,
        %draw=none % Unterdrücke Box
      },
      %
      tuftelike, 
      axis line style = thick,
      every tick/.style={black,thick},
      %axis lines = left,
      %grids=both,
      ymode  = log,
      xmin   = 1,
      xmax   = 500,
      xtick  = {1, 100, 200, 300, 400, 500},
      %
      ymin   = 1e+4,
      ymax   = 1e+8,
      %
      xlabel = {Iteration},
      %ylabel = {\(\mathbb{E}\norm{\rvvg}^2_2\)},
      height = 5cm,
      width  = 6cm,
      axis on top,
    ]
    \addplot[name path=gvar, color1, mark=none, thick]
      table [x=t, y=gvar] {data/simulation/quadratic_linearmf_boundedentropybound.csv}
      %node[above=3pt,pos=0.8] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
      coordinate [pos=0.95] (gvarcoord);
    \addlegendentry{\scriptsize\( \mathbb{E}\norm{ \rvvg }_2^2 \)}

    \addplot[name path=opt, color3, mark=none, thick] %
      table [x=t, y=opt] {data/simulation/quadratic_linearmf_boundedentropybound.csv} %
      %node[above=3pt,pos=0.8] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)}
      coordinate [pos=0.95] (optcoord);
    \addlegendentry{\scriptsize\(2 A \left(\mathbb{E}_{q_{\vlambda}} f_{\mathrm{H}} - f^*_{\mathrm{H}}\right)\)}

    \addplot[name path=ABC, color2, mark=none, thick]
      table [x=t, y=ABC] {data/simulation/quadratic_linearmf_boundedentropybound.csv}
      coordinate [pos=0.05] (ABCcoord1) coordinate [pos=0.95] (ABCcoord2);
    \addlegendentry{\scriptsize\(2 A \left(F\left(\vlambda\right) - F^*\right) + B \norm{\nabla F}_2^2 + C\)}

    \addplot[name path=axis, domain=0:490, fill=none, no markers, draw=none] {1e+1}
      coordinate [pos=0.05] (axiscoord);

    %\addplot[name path=ABC, color2, mark=none]
    %  table [x=t, y=ABC] {figures/quadratic_linearchol_boundedentropybound.csv}
    %  ;

    \addplot[name path=C, fill=none, draw=none, gray, mark=none]
      table [x=t, y=C] {data/simulation/quadratic_linearmf_boundedentropybound.csv}
      coordinate [pos=0.05] (Ccoord);

    \addplot[thick, color=color3, fill=color3, fill opacity=0.2] fill between[of=ABC and opt];
    \addplot[thick, color=color2, fill=color2, fill opacity=0.2] fill between[of=ABC and   C];

    \addplot[thick, color=color1, fill=color1, fill opacity=0.2] fill between[of=opt and gvar];
    \addplot[thick, color=gray,   fill=gray,   fill opacity=0.2] fill between[of=C   and axis];

    \draw[thick,color=color3,{Latex[scale=0.5]}-{Latex[scale=0.5]}] (ABCcoord2) -- (optcoord)
      %node[midway,xshift=-25pt] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)}
      coordinate [pos=0.5] (dklarrow_coord);

    \draw[thick,color=color1,{Latex[scale=0.5]}-{Latex[scale=0.5]}] (gvarcoord) -- (optcoord)
      %node[midway,xshift=-25pt] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
      coordinate [pos=0.5] (muL_coord);

    \draw[thick,color=gray,latex-latex] (Ccoord) -- (axiscoord)
      node[midway,xshift=5pt] {\scriptsize\(C\) };

    \node[%
      pin={%
        [%
          pin distance=1cm,%
          pin edge={color3},%
          text=color3%
        ]100:{\scriptsize\( h\left(\vlambda\right) - h^*\)}%
      },%
      inner sep=0pt,
    ] at (dklarrow_coord) {};

    \node[%
      pin={%
        [%
          pin distance=1cm,%
          pin edge={color1},%
          text=color1%
        ]130:{\scriptsize\(\mu_{\mathrm{H}}, L_{\mathrm{H}}\) bound}},%
      inner sep=0pt,%
    ] at (muL_coord) {};


    %\draw[thick,color=color2,latex-latex] (ABCcoord1) -- (Ccoord)
    %  node[midway,xshift=25pt] {\scriptsize\(2 A \left( F\left(\lambda\right) - F^* \right)\) };
  %$\end{axis}


==> figures/group_quadratic_linearmf_generalbound.tex <==

% Tikz examples & demos
% https://holatex.app/examples.html?package=tikz

  \nextgroupplot[
      legend style={
        legend image post style={scale=0.5},
        at={(0.5,1.5)},
        anchor=north,
        legend cell align=left,
        line width=0.8pt,
        %draw=none % Unterdrücke Box
      },
      %
      tuftelike, 
      axis line style = thick,
      every tick/.style={black,thick},
      %axis lines = left,
      %grids=both,
      ymode  = log,
      xmin   = 1,
      xmax   = 500,
      xtick  = {1, 100, 200, 300, 400, 500},
      ytick  = {1e+3, 1e+4, 1e+5, 1e+6, 1e+7},
      %
      ymin   = 1e+3,
      ymax   = 1e+7,
      %
      xlabel = {Iteration},
      %ylabel = {\(\mathbb{E}\norm{\rvvg}^2_2\)},
      height = 5cm,
      width  = 6cm,
      axis on top,
    ]
    \addplot[name path=gvar, color1, mark=none, thick]
      table [x=t, y=gvar] {data/simulation/quadratic_linearmf_generalbound.csv}
      %node[above=3pt,pos=0.8] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
      coordinate [pos=0.95] (gvarcoord);
    \addlegendentry{\scriptsize\( \mathbb{E}\norm{ \rvvg }_2^2 \)}

    \addplot[name path=opt, color3, mark=none, thick] %
      table [x=t, y=opt] {data/simulation/quadratic_linearmf_generalbound.csv} %
      %node[above=3pt,pos=0.8] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)}
      coordinate [pos=0.95] (optcoord);
    \addlegendentry{\scriptsize\(2 A \left(\mathbb{E}_{q_{\vlambda}} f_{\text{KL}} - f^*_{\text{KL}} \right)\)}

    \addplot[name path=ABC, color2, mark=none, thick]
      table [x=t, y=ABC] {data/simulation/quadratic_linearmf_generalbound.csv}
      coordinate [pos=0.05] (ABCcoord1) coordinate [pos=0.95] (ABCcoord2);
    \addlegendentry{\scriptsize\(2 A \left(F\left(\vlambda\right) - F^*\right) + B \norm{\nabla F}_2^2 + C\)}

    \addplot[name path=axis, domain=0:490, fill=none, no markers, draw=none] {1e+3}
      coordinate [pos=0.05] (axiscoord);

    %\addplot[name path=ABC, color2, mark=none]
    %  table [x=t, y=ABC] {data/simulation/quadratic_linearchol_generalbound.csv}
    %  ;

    \addplot[name path=C, fill=none, draw=none, gray, mark=none]
      table [x=t, y=C] {data/simulation/quadratic_linearmf_generalbound.csv}
      coordinate [pos=0.05] (Ccoord);

    \addplot[thick, color=color3, fill=color3, fill opacity=0.2] fill between[of=ABC and opt];
    \addplot[thick, color=color2, fill=color2, fill opacity=0.2] fill between[of=ABC and   C];

    \addplot[thick, color=color1, fill=color1, fill opacity=0.2] fill between[of=opt and gvar];
    \addplot[thick, color=gray,   fill=gray,   fill opacity=0.2] fill between[of=C   and axis];

    \draw[thick,color=color3,latex-latex] (ABCcoord2) -- (optcoord)
      node[midway,xshift=-20pt] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)};

    \draw[thick,color=color1,{Latex[scale=0.5]}-{Latex[scale=0.5]}] (gvarcoord) -- (optcoord)
      node[midway,xshift=-32pt] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}, \Delta \vz^*\) bound}
      coordinate [pos=0.5] (muL_coord);

    \draw[thick,color=gray,latex-] (Ccoord) -- (axiscoord)
      node[midway,xshift=5pt] {\scriptsize\(C\) };

    %\draw[thick,color=color2,latex-latex] (ABCcoord1) -- (Ccoord)
    %  node[midway,xshift=25pt] {\scriptsize\(2 A \left( F\left(\lambda\right) - F^* \right)\) };

%%     \node[%
%%       pin={%
%%         [%
%%           pin distance=0.45cm,%
%%           pin edge={color1},%
%%           text=color1%
%%         ]263:{\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}, \Delta \vz^* \) bound}},%
%%       inner sep=0pt,%
%%     ] at (muL_coord) {};

%%     \node[%
%%       pin={%
%%         [%
%%           pin distance=1.8cm,%
%%           pin edge={color1},%
%%           text=color1%
%%         ]92:{\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}},%
%%       inner sep=0pt,%
%%     ] at (muL_coord) {};



==> figures/group_quadratic_softpluschol_boundedentropy.tex <==

% Tikz examples & demos
% https://holatex.app/examples.html?package=tikz

  \nextgroupplot[
      %% legend style={
      %%   legend image post style={scale=0.5},
      %%   at={(0.5,1.5)},
      %%   anchor=north,
      %%   legend cell align=left,
      %%   line width=0.8pt,
      %%   %draw=none % Unterdrücke Box
      %% },
      %
      tuftelike, 
      axis line style = thick,
      every tick/.style={black,thick},
      %axis lines = left,
      %grids=both,
      ymode  = log,
      xmin   = 1,
      xmax   = 1000,
      xtick  = {1, 200, 400, 600, 800, 1000},
      ytick  = {1e+4, 1e+5, 1e+6, 1e+7, 1e+8},
      %
      xlabel style={yshift=-0.8ex},
      %
      ymin   = 1e+4,
      ymax   = 1e+8,
      %
      xlabel = {Iteration},
      %ylabel = {\(\mathbb{E}\norm{\rvvg}^2_2\)},
      tick label style={font=\small},  
      height = 4cm,
      width  = 4.7cm,
      axis on top,
    ]
    \addplot[name path=gvar, color1, mark=none, thick]
      table [x=t, y=gvar] {data/simulation/quadratic_softpluschol_boundedentropybound.csv}
      %node[above=3pt,pos=0.8] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
      coordinate [pos=0.95] (gvarcoord);
    %% \addlegendentry{\scriptsize\( \mathbb{E}\norm{ \rvvg }_2^2 \)}

    \addplot[name path=opt, color3, mark=none, thick] %
      table [x=t, y=opt] {data/simulation/quadratic_softpluschol_boundedentropybound.csv} %
      %node[above=3pt,pos=0.8] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)}
      coordinate [pos=0.95] (optcoord);
    %% \addlegendentry{\scriptsize\(2 A \left(\mathbb{E}_{q_{\vlambda}} f_{\mathrm{H}} - f^*_{\mathrm{H}}\right)\)}

    \addplot[name path=ABC, color2, mark=none, thick]
      table [x=t, y=ABC] {data/simulation/quadratic_softpluschol_boundedentropybound.csv}
      coordinate [pos=0.05] (ABCcoord1) coordinate [pos=0.95] (ABCcoord2);
    %% \addlegendentry{\scriptsize\(2 A \left(F\left(\vlambda\right) - F^*\right) + B \norm{\nabla F}_2^2 + C\)}

    \addplot[name path=axis, domain=0:990, fill=none, no markers, draw=none] {1e+4}
      coordinate [pos=0.05] (axiscoord);

    %\addplot[name path=ABC, color2, mark=none]
    %  table [x=t, y=ABC] {data/simulation/quadratic_softpluschol_boundedentropybound.csv}
    %  ;

    \addplot[name path=C, fill=none, gray, mark=none]
      table [x=t, y=C] {data/simulation/quadratic_softpluschol_boundedentropybound.csv}
      coordinate [pos=0.05] (Ccoord);

    \addplot[thick, color=color3, fill=color3, fill opacity=0.2] fill between[of=ABC and opt];
    \addplot[thick, color=color2, fill=color2, fill opacity=0.2] fill between[of=ABC and   C];

    \addplot[thick, color=color1, fill=color1, fill opacity=0.2] fill between[of=opt and gvar];
    \addplot[thick, color=gray,   fill=gray,   fill opacity=0.2] fill between[of=C   and axis];

    \draw[thick,color=color3,{Latex[scale=0.5]}-{Latex[scale=0.5]}] (ABCcoord2) -- (optcoord)
      node[midway,xshift=-18pt] {\scriptsize\(h\left(\vlambda\right) - h^*\)}
      coordinate [pos=0.5] (dklarrow_coord);

    %\draw[thick,color=color1,{Latex[scale=0.5]}-{Latex[scale=0.5]}] (gvarcoord) -- (optcoord)
      %node[midway,xshift=-25pt] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
    %  coordinate [pos=0.5] (muL_coord);

    \draw[thick,color=gray,latex-] (Ccoord) -- (axiscoord)
      node[midway,xshift=5pt] {\scriptsize\(C\) };

    %% \node[%
    %%   pin={%
    %%     [%
    %%       pin distance=1cm,%
    %%       pin edge={color3},%
    %%       text=color3%
    %%     ]100:{\scriptsize\( h\left(\vlambda\right) - h^* \)}%
    %%   },%
    %%   inner sep=0pt,
    %% ] at (dklarrow_coord) {};

    %% \node[%
    %%   pin={%
    %%     [%
    %%       pin distance=1cm,%
    %%       pin edge={color1},%
    %%       text=color1%
    %%     ]130:{\scriptsize\(\mu_{\mathrm{H}}, L_{\mathrm{H}}\) bound}},%
    %%   inner sep=0pt,%
    %% ] at (muL_coord) {};


    %\draw[thick,color=color2,latex-latex] (ABCcoord1) -- (Ccoord)
    %  node[midway,xshift=25pt] {\scriptsize\(2 A \left( F\left(\lambda\right) - F^* \right)\) };


==> figures/group_quadratic_softpluschol_generalbound.tex <==

% Tikz examples & demos
% https://holatex.app/examples.html?package=tikz

  \nextgroupplot[
      legend style={
        legend image post style = {scale=0.5},
        legend columns          = -1,
        column sep              = 1em,
        %at                     ={(0.5,1.5)},
        anchor                  = north,
        legend cell align       = left,
        line width              = 0.8pt,
        draw                    = none,
        legend to name          = grouplegend
      },
      %
      tuftelike, 
      %
      xlabel style={yshift=-0.8ex},
      %
      axis line style = thick,
      every tick/.style={black,thick},
      %axis lines = left,
      %grids=both,
      ymode  = log,
      xmin   = 1,
      xmax   = 1000,
      xtick  = {1, 200, 400, 600, 800, 1000},
      ytick  = {1e+4, 1e+5, 1e+6, 1e+7, 1e+8},
      %
      ymin   = 1e+4,
      ymax   = 1e+8,
      %
      xlabel = {Iteration},
      %ylabel = {\(\mathbb{E}\norm{\rvvg}^2_2\)},
      tick label style={font=\small},  
      height = 4cm,
      width  = 4.7cm,
      axis on top,
    ]
    \addplot[name path=gvar, color1, mark=none, thick]
      table [x=t, y=gvar] {data/simulation/quadratic_softpluschol_generalbound.csv}
      %node[above=3pt,pos=0.8] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
      coordinate [pos=0.95] (gvarcoord);
    \addlegendentry{\scriptsize Gradient Variance\;\; \( \mathbb{E}\norm{ \rvvg }_2^2 \)}

    \addplot[name path=ABC, color2, mark=none, thick]
      table [x=t, y=ABC] {data/simulation/quadratic_softpluschol_generalbound.csv}
      coordinate [pos=0.05] (ABCcoord1) coordinate [pos=0.95] (ABCcoord2);
    \addlegendentry{\scriptsize Upper Bound\;\; \(2 A \left(F\left(\vlambda\right) - F^*\right) + B \norm{\nabla F}_2^2 + C\)}

    %\addplot[color4, draw=none, mark=none, thick] {x};
    %\addlegendentry{\scriptsize\(2 A \left(\mathbb{E}_{q_{\vlambda}} f_{\mathrm{KL}} - f^*_{\mathrm{KL}} \right) + B \norm{\nabla F}_2^2 + C_{\Delta \zeta} {\lVert \bar{\zeta}_{\mathrm{KL}} - \bar{\zeta}_{\mathrm{H}} \rVert}^2_2 \)}

    \addplot[name path=opt, color3, mark=none, thick] %
      table [x=t, y=opt] {data/simulation/quadratic_softpluschol_generalbound.csv} %
      %node[above=3pt,pos=0.8] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)}
      coordinate [pos=0.95] (optcoord);
    %\addlegendentry{\scriptsize\(2 A \left(\mathbb{E}_{q_{\vlambda}} f_{\mathrm{H}} - f^*_{\mathrm{H}} \right) + B \norm{\nabla F}_2^2\)}

    \addplot[name path=axis, domain=0:990, fill=none, no markers, draw=none] {1e+4}
      coordinate [pos=0.05] (axiscoord);

    %\addplot[name path=ABC, color2, mark=none]
    %  table [x=t, y=ABC] {data/simulation/quadratic_softpluschol_generalbound.csv}
    %  ;

    \addplot[name path=C, fill=none, gray, mark=none]
      table [x=t, y=C] {data/simulation/quadratic_softpluschol_generalbound.csv}
      coordinate [pos=0.05] (Ccoord);

    \addplot[thick, color=color3, fill=color3, fill opacity=0.2] fill between[of=ABC and opt];
    \addplot[thick, color=color2, fill=color2, fill opacity=0.2] fill between[of=ABC and   C];

    \addplot[thick, color=color1, fill=color1, fill opacity=0.2] fill between[of=opt and gvar];
    \addplot[thick, color=gray,   fill=gray,   fill opacity=0.2] fill between[of=C   and axis];

    \draw[thick,color=color3,{Latex[scale=0.5]}-{Latex[scale=0.5]}] (ABCcoord2) -- (optcoord)
      node[midway,xshift=-18pt] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)};

    %\draw[thick,color=color1,latex-latex] (gvarcoord) -- (optcoord)
    %  %node[midway,xshift=-32pt] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}, \Delta \vz^*\) bound}
    %  coordinate [pos=0.5] (muL_coord);

    \draw[thick,color=gray,latex-] (Ccoord) -- (axiscoord)
      node[midway,xshift=5pt] {\scriptsize\(C\) };

%%     \node[%
%%       pin={%
%%         [%
%%           pin distance=0.3cm,%
%%           pin edge={color1},%
%%           text=color1%
%%         ]265:{\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}, \Delta \vz^*, \phi \) bound}},%
%%       inner sep=0pt,%
%%     ] at (muL_coord) {};

    %\draw[thick,color=color2,latex-latex] (ABCcoord1) -- (Ccoord)
    %  node[midway,xshift=25pt] {\scriptsize\(2 A \left( F\left(\lambda\right) - F^* \right)\) };


==> figures/group_quadratic_softplusmf_boundedentropy.tex <==

% Tikz examples & demos
% https://holatex.app/examples.html?package=tikz

  \nextgroupplot[
      %% legend style={
      %%   legend image post style={scale=0.5},
      %%   at={(0.5,1.5)},
      %%   anchor=north,
      %%   legend cell align=left,
      %%   line width=0.8pt,
      %%   %draw=none % Unterdrücke Box
      %% },
      %
      tuftelike, 
      axis line style = thick,
      every tick/.style={black,thick},
      %axis lines = left,
      %grids=both,
      ymode  = log,
      xmin   = 1,
      xmax   = 1000,
      xtick  = {1, 200, 400, 600, 800, 1000},
      ytick  = {1e+3, 1e+4, 1e+5, 1e+6, 1e+7, 1e+8},
      %
      xlabel style={yshift=-0.8ex},
      %
      ymin   = 1e+3,
      ymax   = 1e+8,
      %
      xlabel = {Iteration},
      %ylabel = {\(\mathbb{E}\norm{\rvvg}^2_2\)},
      tick label style={font=\small},  
      height = 4cm,
      width  = 4.7cm,
      axis on top,
    ]
    \addplot[name path=gvar, color1, mark=none, thick]
      table [x=t, y=gvar] {data/simulation/quadratic_softplusmf_boundedentropybound.csv}
      %node[above=3pt,pos=0.8] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
      coordinate [pos=0.95] (gvarcoord);
    %\addlegendentry{\scriptsize\( \mathbb{E}\norm{ \rvvg }_2^2 \)}

    \addplot[name path=opt, color3, mark=none, thick] %
      table [x=t, y=opt] {data/simulation/quadratic_softplusmf_boundedentropybound.csv} %
      %node[above=3pt,pos=0.8] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)}
      coordinate [pos=0.95] (optcoord);
    %\addlegendentry{\scriptsize\(2 A \left(\mathbb{E}_{q_{\vlambda}} f_{\mathrm{H}} - f^*_{\mathrm{H}}\right)\)}

    \addplot[name path=ABC, color2, mark=none, thick]
      table [x=t, y=ABC] {data/simulation/quadratic_softplusmf_boundedentropybound.csv}
      coordinate [pos=0.05] (ABCcoord1) coordinate [pos=0.95] (ABCcoord2);
    %\addlegendentry{\scriptsize\(2 A \left(F\left(\vlambda\right) - F^*\right) + B \norm{\nabla F}_2^2 + C\)}

    \addplot[name path=axis, domain=0:990, fill=none, no markers, draw=none] {1e+3}
      coordinate [pos=0.05] (axiscoord);

    %\addplot[name path=ABC, color2, mark=none]
    %  table [x=t, y=ABC] {data/simulation/quadratic_softpluschol_boundedentropybound.csv}
    %  ;

    \addplot[name path=C, fill=none, gray, mark=none]
      table [x=t, y=C] {data/simulation/quadratic_softplusmf_boundedentropybound.csv}
      coordinate [pos=0.05] (Ccoord);

    \addplot[thick, color=color3, fill=color3, fill opacity=0.2] fill between[of=ABC and opt];
    \addplot[thick, color=color2, fill=color2, fill opacity=0.2] fill between[of=ABC and   C];

    \addplot[thick, color=color1, fill=color1, fill opacity=0.2] fill between[of=opt and gvar];
    \addplot[thick, color=gray,   fill=gray,   fill opacity=0.2] fill between[of=C   and axis];

    \draw[thick,color=color3,{Latex[scale=0.5]}-{Latex[scale=0.5]}] (ABCcoord2) -- (optcoord)
      node[midway,xshift=-18pt] {\scriptsize\(h\left(\vlambda\right) - h^*\)}
      coordinate [pos=0.5] (dklarrow_coord);

    %\draw[thick,color=color1,{Latex[scale=0.5]}-{Latex[scale=0.5]}] (gvarcoord) -- (optcoord)
      %node[midway,xshift=-25pt] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
    %  coordinate [pos=0.5] (muL_coord);

    \draw[thick,color=gray,latex-] (Ccoord) -- (axiscoord)
      node[midway,xshift=5pt] {\scriptsize\(C\) };

    %% \node[%
    %%   pin={%
    %%     [%
    %%       pin distance=1cm,%
    %%       pin edge={color3},%
    %%       text=color3%
    %%     ]100:{\scriptsize\( h\left(\vlambda\right) - h^* \)}%
    %%   },%
    %%   inner sep=0pt,
    %% ] at (dklarrow_coord) {};

    %% \node[%
    %%   pin={%
    %%     [%
    %%       pin distance=1cm,%
    %%       pin edge={color1},%
    %%       text=color1%
    %%     ]130:{\scriptsize\(\mu_{\mathrm{H}}, L_{\mathrm{H}}\) bound}},%
    %%   inner sep=0pt,%
    %% ] at (muL_coord) {};


    %\draw[thick,color=color2,latex-latex] (ABCcoord1) -- (Ccoord)
    %  node[midway,xshift=25pt] {\scriptsize\(2 A \left( F\left(\lambda\right) - F^* \right)\) };


==> figures/group_quadratic_softplusmf_generalbound.tex <==

% Tikz examples & demos
% https://holatex.app/examples.html?package=tikz

  \nextgroupplot[
      %% legend style={
      %%   legend image post style={scale=0.5},
      %%   at={(0.5,1.5)},
      %%   anchor=north,
      %%   legend cell align=left,
      %%   line width=0.8pt,
      %%   %draw=none % Unterdrücke Box
      %% },
      %
      tuftelike, 
      axis line style = thick,
      every tick/.style={black,thick},
      %axis lines = left,
      %grids=both,
      ymode  = log,
      xmin   = 1,
      xmax   = 1000,
      xtick  = {1, 200, 400, 600, 800, 1000},
      ytick  = {1e+3, 1e+4, 1e+5, 1e+6, 1e+7, 1e+8},
      %
      xlabel style={yshift=-0.8ex},
      %
      ymin   = 1e+3,
      ymax   = 1e+8,
      %
      xlabel = {Iteration},
      %ylabel = {\(\mathbb{E}\norm{\rvvg}^2_2\)},
      tick label style={font=\small},  
      height = 4cm,
      width  = 4.7cm,
      axis on top,
    ]
    \addplot[name path=gvar, color1, mark=none, thick]
      table [x=t, y=gvar] {data/simulation/quadratic_softplusmf_generalbound.csv}
      %node[above=3pt,pos=0.8] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
      coordinate [pos=0.95] (gvarcoord);
    %% \addlegendentry{\scriptsize\( \mathbb{E}\norm{ \rvvg }_2^2 \)}

    \addplot[name path=opt, color3, mark=none, thick] %
      table [x=t, y=opt] {data/simulation/quadratic_softplusmf_generalbound.csv} %
      %node[above=3pt,pos=0.8] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)}
      coordinate [pos=0.95] (optcoord);
    %% \addlegendentry{\scriptsize\(2 A \left(\mathbb{E}_{q_{\vlambda}} f_{\text{KL}} - f^*_{\text{KL}} \right)\)}

    \addplot[name path=ABC, color2, mark=none, thick]
      table [x=t, y=ABC] {data/simulation/quadratic_softplusmf_generalbound.csv}
      coordinate [pos=0.05] (ABCcoord1) coordinate [pos=0.95] (ABCcoord2);
    %% \addlegendentry{\scriptsize\(2 A \left(F\left(\vlambda\right) - F^*\right) + B \norm{\nabla F}_2^2 + C\)}

    \addplot[name path=axis, domain=0:990, fill=none, no markers, draw=none] {1e+3}
      coordinate [pos=0.05] (axiscoord);

    %\addplot[name path=ABC, color2, mark=none]
    %  table [x=t, y=ABC] {data/simulation/quadratic_softpluschol_generalbound.csv}
    %  ;

    \addplot[name path=C, fill=none, gray, mark=none]
      table [x=t, y=C] {data/simulation/quadratic_softplusmf_generalbound.csv}
      coordinate [pos=0.05] (Ccoord);

    \addplot[thick, color=color3, fill=color3, fill opacity=0.2] fill between[of=ABC and opt];
    \addplot[thick, color=color2, fill=color2, fill opacity=0.2] fill between[of=ABC and   C];

    \addplot[thick, color=color1, fill=color1, fill opacity=0.2] fill between[of=opt and gvar];
    \addplot[thick, color=gray,   fill=gray,   fill opacity=0.2] fill between[of=C   and axis];

    \draw[thick,color=color3,{Latex[scale=0.5]}-{Latex[scale=0.5]}] (ABCcoord2) -- (optcoord)
      node[midway,xshift=-20pt] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)};

    %\draw[thick,color=color1,latex-latex] (gvarcoord) -- (optcoord)
      %node[midway,xshift=-32pt] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}, \Delta \vz^*\) bound}
    %  coordinate [pos=0.5] (muL_coord);

    \draw[thick,color=gray,latex-] (Ccoord) -- (axiscoord)
      node[midway,xshift=5pt] {\scriptsize\(C\) };

    %% \node[%
    %%   pin={%
    %%     [%
    %%       pin distance=0.3cm,%
    %%       pin edge={color1},%
    %%       text=color1%
    %%     ]265:{\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}, \Delta \vz^*, \phi \) bound}},%
    %%   inner sep=0pt,%
    %% ] at (muL_coord) {};

    %\draw[thick,color=color2,latex-latex] (ABCcoord1) -- (Ccoord)
    %  node[midway,xshift=25pt] {\scriptsize\(2 A \left( F\left(\lambda\right) - F^* \right)\) };


==> figures/group_quadratic_squareroot_generalbound.tex <==

% Tikz examples & demos
% https://holatex.app/examples.html?package=tikz

  \nextgroupplot[
      %
      tuftelike, 
      axis line style = thick,
      every tick/.style={black,thick},
      %axis lines = left,
      %grids=both,
      ymode  = log,
      xmin   = 1,
      xmax   = 500,
      xtick  = {1, 100, 200, 300, 400, 500},
      ytick  = {1e+4, 1e+5, 1e+6, 1e+7, 1e+8, 1e+9},
      %
      ymin   = 1e+4,
      ymax   = 1e+9,
      %
      xlabel = {Iteration},
      %ylabel = {\(\mathbb{E}\norm{\rvvg}^2_2\)},
      height = 4.5cm,
      width  = 4.7cm,
      axis on top,
    ]
    \addplot[name path=gvar, color1, mark=none, thick]
      table [x=t, y=gvar] {data/simulation/quadratic_squareroot_generalbound.csv}
      %node[above=3pt,pos=0.8] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
      coordinate [pos=0.95] (gvarcoord);
    %\addlegendentry{\scriptsize\( \mathbb{E}\norm{ \rvvg }_2^2 \)}

    \addplot[name path=opt, color3, mark=none, thick] %
      table [x=t, y=opt] {data/simulation/quadratic_squareroot_generalbound.csv} %
      %node[above=3pt,pos=0.8] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)}
      coordinate [pos=0.95] (optcoord);
    %\addlegendentry{\scriptsize\(2 A \left(\mathbb{E}_{q_{\vlambda}} f_{\text{KL}} - f^*_{\text{KL}}\right)\)}

    \addplot[name path=ABC, color2, mark=none, thick]
      table [x=t, y=ABC] {data/simulation/quadratic_squareroot_generalbound.csv}
      coordinate [pos=0.05] (ABCcoord1) coordinate [pos=0.95] (ABCcoord2);
    %\addlegendentry{\scriptsize\(2 A \left(F\left(\vlambda\right) - F^*\right) + B \norm{\nabla F}_2^2 + C\)}

    \addplot[name path=axis, domain=0:490, fill=none, no markers, draw=none] {1e+4}
      coordinate [pos=0.05] (axiscoord);

    %\addplot[name path=ABC, color2, mark=none]
    %  table [x=t, y=ABC] {data/simulation/quadratic_squareroot_generalbound.csv}
    %  ;

    \addplot[name path=C, fill=none, gray, mark=none]
      table [x=t, y=C] {data/simulation/quadratic_squareroot_generalbound.csv}
      coordinate [pos=0.05] (Ccoord);

    \addplot[thick, color=color3, fill=color3, fill opacity=0.2] fill between[of=ABC and opt];
    \addplot[thick, color=color2, fill=color2, fill opacity=0.2] fill between[of=ABC and   C];

    \addplot[thick, color=color1, fill=color1, fill opacity=0.2] fill between[of=opt and gvar];
    \addplot[thick, color=gray,   fill=gray,   fill opacity=0.2] fill between[of=C   and axis];

    \draw[thick,color=color3,latex-latex] (ABCcoord2) -- (optcoord)
      node[midway,xshift=-20pt] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)};

    %\draw[thick,color=color1] (gvarcoord) -- (optcoord)
      %node[midway,xshift=-32pt] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}, \Delta \vz^*\) bound}
    %  coordinate [pos=0.5] (muL_coord);

    \draw[thick,color=gray,latex-] (Ccoord) -- (axiscoord)
      node[midway,xshift=5pt] {\scriptsize\(C\) };

    %% \node[%
    %%   pin={%
    %%     [%
    %%       pin distance=0.2cm,%
    %%       pin edge={color1},%
    %%       text=color1%
    %%     ]263:{\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}, \Delta \vz^* \) bound}},%
    %%   inner sep=0pt,%
    %% ] at (muL_coord) {};

    %\draw[thick,color=color2,latex-latex] (ABCcoord1) -- (Ccoord)
    %  node[midway,xshift=25pt] {\scriptsize\(2 A \left( F\left(\lambda\right) - F^* \right)\) };


==> figures/group_wine_linearchol_generalbound.tex <==

  \nextgroupplot[
      %% legend style={
      %%   legend image post style = {scale=0.5},
      %%   legend columns          = -1,
      %%   column sep              = 1em,
      %%   %at                     ={(0.5,1.5)},
      %%   anchor                  = north,
      %%   legend cell align       = left,
      %%   line width              = 0.8pt,
      %%   draw                    = none,
      %%   legend to name          = grouplegend
      %% },
      %
      tuftelike, 
      axis line style = thick,
      every tick/.style={black,thick},
      %axis lines = left,
      %grids=both,
      ymode  = log,
      xmin   = 1,
      xmax   = 500,
      xtick  = {1, 100, 200, 300, 400, 500},
      ytick  = {1e+3, 1e+6, 1e+9, 1e+12},
      %
      ymin   = 1e+3,
      ymax   = 1e+12,
      %
      xlabel = {Iteration},
      %ylabel = {\(\mathbb{E}\norm{\rvvg}^2_2\)},
      height = 5cm,
      width  = 4.7cm,
      axis on top,
    ]
    \addplot[name path=gvar, color1, mark=none, thick]
      table [x=t, y=gvar] {data/simulation/wine_linearchol_generalbound.csv}
      %node[above=3pt,pos=0.8] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
      coordinate [pos=0.95] (gvarcoord);
    %\addlegendentry{\scriptsize\( \mathbb{E}\norm{ \rvvg }_2^2 \)}

    \addplot[name path=opt, color3, mark=none, thick] %
      table [x=t, y=opt] {data/simulation/wine_linearchol_generalbound.csv} %
      %node[above=3pt,pos=0.8] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)}
      coordinate [pos=0.95] (optcoord);
    %\addlegendentry{\scriptsize\(2 A \left(\mathbb{E}_{q_{\vlambda}} f_{\text{KL}} - f^*_{\text{KL}} \right)\)}

    \addplot[name path=ABC, color2, mark=none, thick]
      table [x=t, y=ABC] {data/simulation/wine_linearchol_generalbound.csv}
      coordinate [pos=0.05] (ABCcoord1) coordinate [pos=0.95] (ABCcoord2);
    %\addlegendentry{\scriptsize\(2 A \left(F\left(\vlambda\right) - F^*\right) + B \norm{\nabla F}_2^2 + C\)}

    \addplot[name path=axis, domain=0:490, fill=none, no markers, draw=none] {1e+3}
      coordinate [pos=0.05] (axiscoord);

    \addplot[name path=C, fill=none, gray, mark=none]
      table [x=t, y=C] {data/simulation/wine_linearchol_generalbound.csv}
      coordinate [pos=0.05] (Ccoord);

    \addplot[thick, color=color3, fill=color3, fill opacity=0.2] fill between[of=ABC and opt];
    \addplot[thick, color=color2, fill=color2, fill opacity=0.2] fill between[of=ABC and   C];

    \addplot[thick, color=color1, fill=color1, fill opacity=0.2] fill between[of=opt and gvar];
    \addplot[thick, color=gray,   fill=gray,   fill opacity=0.2] fill between[of=C   and axis];

    \draw[thick,color=color3,latex-latex] (ABCcoord2) -- (optcoord)
      node[midway,xshift=-20pt] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)};

    \draw[thick,color=gray,latex-] (Ccoord) -- (axiscoord)
      node[midway,xshift=5pt] {\scriptsize\(C\) };


==> figures/group_wine_softpluschol_generalbound.tex <==

  \nextgroupplot[
      %% legend style={
      %%   legend image post style = {scale=0.5},
      %%   legend columns          = -1,
      %%   column sep              = 1em,
      %%   %at                     ={(0.5,1.5)},
      %%   anchor                  = north,
      %%   legend cell align       = left,
      %%   line width              = 0.8pt,
      %%   draw                    = none,
      %%   legend to name          = grouplegend
      %% },
      %
      tuftelike, 
      axis line style = thick,
      every tick/.style={black,thick},
      %axis lines = left,
      %grids=both,
      ymode  = log,
      xmin   = 1,
      xmax   = 4000,
      xtick  = {1, 1000, 2000, 3000, 4000},
      ytick  = {1e+4, 1e+6, 1e+8, 1e+10, 1e+12},
      %
      ymin   = 1e+4,
      ymax   = 1e+12,
      %
      xlabel = {Iteration},
      %ylabel = {\(\mathbb{E}\norm{\rvvg}^2_2\)},
      height = 4.5cm,
      width  = 5cm,
      axis on top,
    ]
    \addplot[name path=gvar, color1, mark=none, thick]
      table [x=t, y=gvar] {data/simulation/wine_softpluschol_generalbound.csv}
      %node[above=3pt,pos=0.8] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
      coordinate [pos=0.95] (gvarcoord);
    %\addlegendentry{\scriptsize\( \mathbb{E}\norm{ \rvvg }_2^2 \)}

    \addplot[name path=opt, color3, mark=none, thick] %
      table [x=t, y=opt] {data/simulation/wine_softpluschol_generalbound.csv} %
      %node[above=3pt,pos=0.8] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)}
      coordinate [pos=0.95] (optcoord);
    %\addlegendentry{\scriptsize\(2 A \left(\mathbb{E}_{q_{\vlambda}} f_{\text{KL}} - f^*_{\text{KL}} \right)\)}

    \addplot[name path=ABC, color2, mark=none, thick]
      table [x=t, y=ABC] {data/simulation/wine_softpluschol_generalbound.csv}
      coordinate [pos=0.05] (ABCcoord1) coordinate [pos=0.95] (ABCcoord2);
    %\addlegendentry{\scriptsize\(2 A \left(F\left(\vlambda\right) - F^*\right) + B \norm{\nabla F}_2^2 + C\)}

    \addplot[name path=axis, domain=0:3990, fill=none, no markers, draw=none] {1e+4}
      coordinate [pos=0.05] (axiscoord);

    \addplot[name path=C, fill=none, gray, mark=none]
      table [x=t, y=C] {data/simulation/wine_softpluschol_generalbound.csv}
      coordinate [pos=0.05] (Ccoord);

    \addplot[thick, color=color3, fill=color3, fill opacity=0.2] fill between[of=ABC and opt];
    \addplot[thick, color=color2, fill=color2, fill opacity=0.2] fill between[of=ABC and   C];

    \addplot[thick, color=color1, fill=color1, fill opacity=0.2] fill between[of=opt and gvar];
    \addplot[thick, color=gray,   fill=gray,   fill opacity=0.2] fill between[of=C   and axis];

    \draw[thick,color=color3,draw=none,latex-latex] (ABCcoord2) -- (optcoord)
      node[midway,xshift=-20pt] {}
      coordinate [pos=0.5] (DKLcoord);

    \draw[thick,color=gray,latex-] (Ccoord) -- (axiscoord)
      node[pos=0.8,xshift=5pt] {\scriptsize\(C\) };

    \node[%
      pin={%
        [%
          pin distance=0.2cm,%
          pin edge={color3},%
          text=color3%
        ]110:{\scriptsize\(\DKL{q_{\vlambda}}{p}\)}},%
      inner sep=0pt,%
    ] at (DKLcoord) {};


==> figures/group_wine_softplusmf_generalbound.tex <==

  \nextgroupplot[
      %% legend style={
      %%   legend image post style = {scale=0.5},
      %%   legend columns          = -1,
      %%   column sep              = 1em,
      %%   %at                     ={(0.5,1.5)},
      %%   anchor                  = north,
      %%   legend cell align       = left,
      %%   line width              = 0.8pt,
      %%   draw                    = none,
      %%   legend to name          = grouplegend
      %% },
      %
      tuftelike, 
      axis line style = thick,
      every tick/.style={black,thick},
      %axis lines = left,
      %grids=both,
      ymode  = log,
      xmin   = 1,
      xmax   = 4000,
      xtick  = {1, 2000, 4000},
      ytick  = {1e+3, 1e+6, 1e+9, 1e+12},
      %
      ymin   = 1e+3,
      ymax   = 1e+12,
      %
      xlabel = {Iteration},
      %ylabel = {\(\mathbb{E}\norm{\rvvg}^2_2\)},
      height = 5cm,
      width  = 4.7cm,
      axis on top,
    ]
    \addplot[name path=gvar, color1, mark=none, thick]
      table [x=t, y=gvar] {data/simulation/wine_softplusmf_generalbound.csv}
      %node[above=3pt,pos=0.8] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
      coordinate [pos=0.95] (gvarcoord);
    %\addlegendentry{\scriptsize\( \mathbb{E}\norm{ \rvvg }_2^2 \)}

    \addplot[name path=opt, color3, mark=none, thick] %
      table [x=t, y=opt] {data/simulation/wine_softplusmf_generalbound.csv} %
      %node[above=3pt,pos=0.8] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)}
      coordinate [pos=0.95] (optcoord);
    %\addlegendentry{\scriptsize\(2 A \left(\mathbb{E}_{q_{\vlambda}} f_{\text{KL}} - f^*_{\text{KL}} \right)\)}

    \addplot[name path=ABC, color2, mark=none, thick]
      table [x=t, y=ABC] {data/simulation/wine_softplusmf_generalbound.csv}
      coordinate [pos=0.05] (ABCcoord1) coordinate [pos=0.95] (ABCcoord2);
    %\addlegendentry{\scriptsize\(2 A \left(F\left(\vlambda\right) - F^*\right) + B \norm{\nabla F}_2^2 + C\)}

    \addplot[name path=axis, domain=0:3990, fill=none, no markers, draw=none] {1e+3}
      coordinate [pos=0.05] (axiscoord);

    \addplot[name path=C, fill=none, gray, mark=none]
      table [x=t, y=C] {data/simulation/wine_softplusmf_generalbound.csv}
      coordinate [pos=0.05] (Ccoord);

    \addplot[thick, color=color3, fill=color3, fill opacity=0.2] fill between[of=ABC and opt];
    \addplot[thick, color=color2, fill=color2, fill opacity=0.2] fill between[of=ABC and   C];

    \addplot[thick, color=color1, fill=color1, fill opacity=0.2] fill between[of=opt and gvar];
    \addplot[thick, color=gray,   fill=gray,   fill opacity=0.2] fill between[of=C   and axis];

    \draw[thick,color=color3,draw=none,latex-latex] (ABCcoord2) -- (optcoord)
      node[midway,xshift=-20pt] {}
      coordinate [pos=0.5] (DKLcoord);

    \draw[thick,color=gray,latex-] (Ccoord) -- (axiscoord)
      node[pos=0.8,xshift=5pt] {\scriptsize\(C\) };

    \node[%
      pin={%
        [%
          pin distance=0.2cm,%
          pin edge={color3},%
          text=color3%
        ]110:{\scriptsize\(\DKL{q_{\vlambda}}{p}\)}},%
      inner sep=0pt,%
    ] at (DKLcoord) {};


==> figures/group_wine_squareroot_generalbound.tex <==

  \nextgroupplot[
      %% legend style={
      %%   legend image post style = {scale=0.5},
      %%   legend columns          = -1,
      %%   column sep              = 1em,
      %%   %at                     ={(0.5,1.5)},
      %%   anchor                  = north,
      %%   legend cell align       = left,
      %%   line width              = 0.8pt,
      %%   draw                    = none,
      %%   legend to name          = grouplegend
      %% },
      %
      tuftelike, 
      axis line style = thick,
      every tick/.style={black,thick},
      %axis lines = left,
      %grids=both,
      ymode  = log,
      xmin   = 1,
      xmax   = 4000,
      xtick  = {1, 2000, 4000},
      ytick  = {1e+3, 1e+5, 1e+7, 1e+9, 1e+11},
      %
      ymin   = 1e+3,
      ymax   = 1e+11,
      %
      xlabel = {Iteration},
      %ylabel = {\(\mathbb{E}\norm{\rvvg}^2_2\)},
      height = 5cm,
      width  = 4.7cm,
      axis on top,
    ]
    \addplot[name path=gvar, color1, mark=none, thick]
      table [x=t, y=gvar] {data/simulation/wine_squareroot_generalbound.csv}
      %node[above=3pt,pos=0.8] {\scriptsize\(\mu_{\mathrm{KL}}, L_{\mathrm{H}}\) bound}
      coordinate [pos=0.95] (gvarcoord);
    %% \addlegendentry{\scriptsize\( \mathbb{E}\norm{ \rvvg }_2^2 \)}

    \addplot[name path=opt, color3, mark=none, thick] %
      table [x=t, y=opt] {data/simulation/wine_squareroot_generalbound.csv} %
      %node[above=3pt,pos=0.8] {\scriptsize\(\DKL{q_{\vlambda}}{p}\)}
      coordinate [pos=0.95] (optcoord);
    %\addlegendentry{\scriptsize\(2 A \left(\mathbb{E}_{q_{\vlambda}} f_{\text{KL}} - f^*_{\text{KL}} \right)\)}

    \addplot[name path=ABC, color2, mark=none, thick]
      table [x=t, y=ABC] {data/simulation/wine_squareroot_generalbound.csv}
      coordinate [pos=0.05] (ABCcoord1) coordinate [pos=0.95] (ABCcoord2);
    %% \addlegendentry{\scriptsize\(2 A \left(F\left(\vlambda\right) - F^*\right) + B \norm{\nabla F}_2^2 + C\)}

    \addplot[name path=axis, domain=0:3990, fill=none, no markers, draw=none] {1e+3}
      coordinate [pos=0.05] (axiscoord);

    \addplot[name path=C, fill=none, gray, mark=none]
      table [x=t, y=C] {data/simulation/wine_squareroot_generalbound.csv}
      coordinate [pos=0.05] (Ccoord);

    \addplot[thick, color=color3, fill=color3, fill opacity=0.2] fill between[of=ABC and opt];
    \addplot[thick, color=color2, fill=color2, fill opacity=0.2] fill between[of=ABC and   C];

    \addplot[thick, color=color1, fill=color1, fill opacity=0.2] fill between[of=opt and gvar];
    \addplot[thick, color=gray,   fill=gray,   fill opacity=0.2] fill between[of=C   and axis];

    \draw[thick,color=color3,draw=none,latex-latex] (ABCcoord2) -- (optcoord)
      node[midway,xshift=-20pt] {}
      coordinate [pos=0.5] (DKLcoord);

    \draw[thick,color=gray,latex-] (Ccoord) -- (axiscoord)
      node[pos=0.8,xshift=5pt] {\scriptsize\(C\) };

    \node[%
      pin={%
        [%
          pin distance=0.3cm,%
          pin edge={color3},%
          text=color3%
        ]100:{\scriptsize\(\DKL{q_{\vlambda}}{p}\)}},%
      inner sep=0pt,%
    ] at (DKLcoord) {};


==> main-figure0-pratendcommon.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatev}\label{thm:prAtEndv}{(\citealt [Lemma 9]{domke_provable_2019})}\label {thm:u_identities} Let \(\rvvu = \left (\rvu _1, \rvu _2, \ldots , \rvu _d\right )\) be a \(d\)-dimensional vector-valued random variable with zero-mean independently and identically distributed components. Then, \begin {alignat*}{2} &\mathbb {E}\rvvu \rvvu ^{\top } &&= \left ( \mathbb {E} \rvu _i^2 \right ) \mI \\ &\mathbb {E}\norm {\rvvu }_2^2 &&= d \, \mathbb {E} \rvu _i^2 \\ &\mathbb {E} \rvvu \left ( 1 + \norm {\rvvu }_2^2 \right ) &&= \left ( \mathbb {E} \rvu _i^3 \right ) \mathbf {1} \\ &\mathbb {E} \rvvu \rvvu ^{\top } \rvvu \rvvu ^{\top } &&= \left ( \left (d - 1\right ) \, {\left ( \mathbb {E} \rvu _i^2 \right )}^2 + \mathbb {E}\rvu _i^4 \right ) \mI . \end {alignat*}\end{restatable}

\begin{restatable}[]{lemma}{prAtEndRestatevi}\label{thm:prAtEndvi}{(\citealt [Lemma 1]{domke_provable_2019})}\label {thm:variational_gradient_norm_identity} Let \(\vt _{\vlambda }: \mathbb {R}^d \mapsto \mathbb {R}^d\) be defined as in \cref {def:reparam} with parameters \(\vlambda = \left (\vm , \mC \right )\). Also, let \(f : \mathbb {R}^d \mapsto \mathbb {R} \) be some differentiable function. Then, \begin {alignat*}{2} \norm {\nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) }_2^2 = \mathbb {E}\norm {\nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) }_2^2 \left (1 + \norm {\vu }_2^2\right ). \end {alignat*}\end{restatable}

\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}{(\citealt [Lemma 1]{domke_provable_2019})}\label {thm:reparam_u_identity} Let \(\vt _{\vlambda }: \mathbb {R}^d \mapsto \mathbb {R}^d\) be defined as in \cref {def:reparam} with parameters \(\vz = \left (\vm , \mC \right )\). Also, let \(\vz \in \mathbb {R}^d\) be some vector and \(\rvvu = \left (\rvu _1, \ldots , \rvu _d \right )\) be a vector-valued random variable sampled as \(\rvvu \sim \varphi \), where \(\varphi \) is defined as in \cref {assumption:symmetric_standard} with kurtosis \(\kappa = \mathbb {E}\rvu _i^4\). Then, \begin {alignat*}{2} &\mathbb {E} \norm {\,\vt _{\vlambda }\left (\rvvu \right ) - \vz \,}_2^2 \left (1 + \norm {\rvvu }_2^2\right ) \\ &\;= \left (d+1\right ) \norm {\vm - \vz }_2^2 + \left (d + \kappa \right ) \norm {\mC }^2_{\mathrm {F}}. \end {alignat*}\end{restatable}


==> main-figure0-pratendlowerboundlemma.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatexiii}\label{thm:prAtEndxiii}Let \(\vt _{\vlambda }: \mathbb {R}^d \mapsto \mathbb {R}^d\) be defined as in \cref {def:reparam} with parameters \(\vlambda = \left (\vm , \mC \right )\) such that \(\vm \in \mathbb {R}^d\) and \(\mC \in \mathbb {R}^{d \times d}\). Also, let \(\rvvu \sim \varphi \), where \(\varphi \) is defined as in \cref {assumption:symmetric_standard}. Then, \begin {alignat*}{2} \mathbb {E}\vt _{\vlambda }\left (\rvvu \right ) \left (1 + \norm {\rvvu }_2^2\right ) = \left (d + 1\right ) \vm . \end {alignat*}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxiii}Since \(\rvu _i\) follows a symmetric and standardized distribution, \(\mathbb {E}\rvu _i^3 = 0, \mathbb {E} \rvu _i^2 = 1\). Then, \begin {alignat*}{2} \mathbb {E}\vt _{\vlambda }\left (\rvvu \right ) \left (1 + \norm {\rvvu }_2^2\right ) &= \mathbb {E} \left (\mC \rvvu + \vm \right ) \left (1 + \norm {\rvvu }_2^2\right ) \\ &= \mC \, \mathbb {E} \rvvu \left (1 + \norm {\rvvu }_2^2\right ) + \vm \left (1 + \mathbb {E} \norm {\rvvu }_2^2\right ), \shortintertext {applying \cref {thm:u_identities},} &= \left ( \mathbb {E}\rvu _i^3 \right ) \mC \mathbf {1} + \vm \left (1 + d \, \mathbb {E} \rvu _i^2\right ), \shortintertext {and by~\cref {assumption:symmetric_standard},} &= \left (d + 1\right ) \vm . \end {alignat*}\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexiv}\label{thm:prAtEndxiv}\label {thm:general_quad_reparam} Let \(\vt _{\vlambda }: \mathbb {R}^d \mapsto \mathbb {R}^d\) be defined as in \cref {def:reparam} with parameters \(\vlambda = \left (\vm , \mC \right )\) such that \(\vm \in \mathbb {R}^d\) and \(\mC \in \mathbb {R}^{d \times d}\). Also, let \(\mSigma \in \mathbb {R}^{d \times d}\) be some matrix, \(\vmu \in \mathbb {R}^d\) be some vector, and \(\rvvu \sim \varphi \) be a vector-valued random variable, where \(\varphi \) is defined as in \cref {assumption:symmetric_standard}. Then, \begin {align*} &\mathbb {E} \, {\left ( \vt _{\vlambda }\left (\rvvu \right ) - \vmu \right )}^{\top } \mSigma \left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu \right ) \\ &\;= {\left (\vm - \vmu \right )}^{\top } \mSigma \left (\vm - \vmu \right ) + \mathrm {tr}\left ({\mSigma }^{-1} \mC \mC ^{\top }\right ). \end {align*}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxiv}\begin {alignat}{2} &\mathbb {E} {\left ( \vt _{\vlambda }\left (\rvvu \right ) - \vmu \right )}^{\top } \mSigma \, \left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu \right ) \nonumber \\ &\;= \mathbb {E}\, {\vt _{\vlambda }\left (\rvvu \right )}^{\top } \mSigma \, {\vt _{\vlambda }\left (\rvvu \right )} -2\, \vmu ^{\top } {\mSigma } \, \mathbb {E}\vt _{\vlambda }\left (\rvvu \right ) + \vmu ^{\top } {\mSigma } \, \vmu , \nonumber \shortintertext {where \(\mathbb {E}\vt _{\vlambda }\left (\rvvu \right ) = \mC \mathbb {E}{\rvvu } + \vm \), and by \cref {assumption:symmetric_standard},} &\;= \mathbb {E}\, {\vt _{\vlambda }\left (\rvvu \right )}^{\top } \mSigma \, {\vt _{\vlambda }\left (\rvvu \right )} -2\, \vmu ^{\top } {\mSigma } \, \vm + \vmu ^{\top } {\mSigma } \, \vmu .\label {eq:thm:general_quad_reparam_eq1} \end {alignat} Furthermore, \begin {alignat*}{2} &\mathbb {E} {\vt _{\vlambda }\left (\rvvu \right )}^{\top } \mSigma \, {\vt _{\vlambda }\left (\rvvu \right )} \\ &\;= \mathbb {E}{\left (\mC \rvvu + \vm \right )}^{\top } \mSigma \left (\mC \rvvu + \vm \right ) \\ &\;= \mathbb {E} \rvvu ^{\top } \mC ^{\top } \mSigma \, \mC \rvvu + \vm ^{\top } \mSigma \, \mC \, \mathbb {E} \rvvu + \mathbb {E} \rvvu ^{\top } \mC ^{\top } \mSigma \vm ^{\top } + \vm ^{\top } \mSigma \, \vm , \shortintertext {by \cref {assumption:symmetric_standard},} &\;= \mathbb {E} \rvvu ^{\top } \mC ^{\top } {\mSigma } \, \mC \rvvu + \vm ^{\top } \mSigma \, \vm , \shortintertext {invoking the trace trick,} &\;= \mathbb {E} \mathrm {tr}\left ( \rvvu ^{\top } \mC ^{\top } {\mSigma }\, \mC \rvvu \right ) + \vm ^{\top } \mSigma \, \vm , \shortintertext {pusing the expectation into the trace,} &\;= \mathrm {tr}\left (\mathbb {E} \rvvu \rvvu ^{\top } \mC ^{\top } {\mSigma }\, \mC \right ) + \vm ^{\top } \mSigma \, \vm , \shortintertext {invoking \cref {thm:u_identities},} &\;= \mathrm {tr}\left (\mC ^{\top } {\mSigma }\, \mC \right ) + \vm ^{\top } \mSigma \, \vm \\ &\;= \mathrm {tr}\left ({\mSigma } \, \mC \mC ^{\top }\right ) + \vm ^{\top } \mSigma \, \vm . \end {alignat*} Applying this to \cref {eq:thm:general_quad_reparam_eq1}, \begin {alignat*}{2} &\mathbb {E} {\left ( \vt _{\vlambda }\left (\rvvu \right ) - \vmu \right )}^{\top } {\mSigma }^{-1} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu \right ) \\ &\;= \mathrm {tr}\left ({\mSigma }^{-1} \mC \mC ^{\top }\right ) + \vm ^{\top } \mSigma ^{-1} \vm -2\, \vmu ^{\top } {\mSigma }^{-1} \vm + \vmu ^{\top } {\mSigma }^{-1} \vmu \\ &\;= {\left (\vm - \vmu \right )}^{\top } {\mSigma }^{-1} \left (\vm - \vmu \right ) + \mathrm {tr}\left ({\mSigma }^{-1} \mC \mC ^{\top }\right ). \end {alignat*}\end{proof}

\begin{restatable}[]{corollary}{prAtEndRestatexv}\label{thm:prAtEndxv}\label {thm:q_quad_reparam} Let \(\vt _{\vlambda }: \mathbb {R}^d \mapsto \mathbb {R}^d\) be defined as in \cref {def:reparam} with parameters \(\vlambda = \left (\vm , \mC \right )\) such that \(\vm \in \mathbb {R}^d\) and \(\mC \in \mathbb {R}^{d \times d}\). Also, let \(\rvvu \sim \varphi \) be a vector-valued random variable, where \(\varphi \) is defined as in \cref {assumption:symmetric_standard}. Then, \begin {align*} \mathbb {E} \, {\left ( \vt _{\vlambda }\left (\rvvu \right ) - \vm \right )}^{\top } {\left (\mC \mC ^{\top }\right )}^{-1} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right ) = d. \end {align*}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxv}From, \cref {thm:general_quad_reparam} we have \begin {alignat*}{2} &\mathbb {E} \, {\left ( \vt _{\vlambda }\left (\rvvu \right ) - \vm \right )}^{\top } {\left (\mC \mC ^{\top }\right )}^{-1} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right ) \\ &\;= {\left (\vm - \vm \right )}^{\top } {\left (\mC \mC ^{\top }\right )}^{-1} \left (\vm - \vm \right ) + \mathrm {tr}\left ({\left ( \mC \mC ^{\top } \right )}^{-1} \mC \mC ^{\top }\right ) \\ &\;= \mathrm {tr}\left (\mI \right ) \\ &\;= d. \end {alignat*}\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexvi}\label{thm:prAtEndxvi}\label {thm:general_grad_norm_reparam} Let \(\vt _{\vlambda }: \mathbb {R}^d \mapsto \mathbb {R}^d\) be defined as in \cref {def:reparam} with parameters \(\vlambda = \left (\vm , \mC \right )\) such that \(\vm \in \mathbb {R}^d\) and \(\mC \in \mathbb {R}^{d \times d}\). Also, let \(\mSigma _1, \mSigma _2 \in \mathbb {R}^{d \times d}\) be some matrices, \(\vmu _1, \vmu _2 \in \mathbb {R}^{d}\) be some vectors, and \(\rvvu = \left (\rvu _1, \ldots , \rvu _d \right )\) be a vector-valued random variable sampled as \(\rvvu \sim \varphi \), where \(\varphi \) is defined as in \cref {assumption:symmetric_standard} with kurtosis \(\kappa = \mathbb {E}\rvu _i^4\). Then, \begin {alignat*}{2} &\mathbb {E} {\left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu _1\right )}^{\top } \mSigma _1 \mSigma _2 \left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu _2\right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \\ &\;= \left (d + 1\right ) \vmu _1^{\top } \mSigma _1 \mSigma _2 \vmu _2 + \left (d + \kappa \right ) \mathrm {tr}\left (\mC \mC ^{\top } \mSigma _1 \mSigma _2 \right ). \end {alignat*}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxvi}\begin {alignat}{2} &\mathbb {E} {\left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu _1\right )}^{\top } \mSigma _1 \mSigma _2 \left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu _2\right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\;= \mathbb {E} {\vt _{\vlambda }\left (\rvvu \right )}^{\top } \mSigma _1 \mSigma _2 \, \vt _{\vlambda }\left (\rvvu \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\qquad - \vmu _1^{\top } \mSigma _1 \mSigma _2 \, \mathbb {E} \vt _{\vlambda }\left (\rvvu \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\qquad - \mathbb {E} {\left (\vt _{\vlambda }\left (\rvvu \right ) \left ( 1 + \norm {\rvvu }_2^2 \right )\right )}^{\top } \mSigma _1 \mSigma _2 \vmu _1 \nonumber \\ &\qquad + \vmu _1^{\top } \mSigma _1 \mSigma _2 \vmu _2 \, \mathbb {E}\left ( 1 + \norm {\rvvu }_2^2 \right ), \nonumber \shortintertext {invoking \cref {thm:u_identities},} &\;= \mathbb {E} {\vt _{\vlambda }\left (\rvvu \right )}^{\top } \mSigma _1 \mSigma _2 \, \vt _{\vlambda }\left (\rvvu \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\qquad - \mathbb {E}\rvu _i^3 \, \vmu _1^{\top } \mSigma _1 \mSigma _2 \mathbf {1} \nonumber \\ &\qquad - \mathbb {E}\rvu _i^3 \, \mathbf {1}^{\top } \mSigma _1 \mSigma _2 \vmu _1 \nonumber \\ &\qquad + \left ( 1 + d\,\mathbb {E}\rvu _i^2 \right ) \vmu _1^{\top } \mSigma _1 \mSigma _2 \vmu _2, \nonumber \shortintertext {and due to \cref {assumption:symmetric_standard},} &\;= \mathbb {E} {\vt _{\vlambda }\left (\rvvu \right )}^{\top } \mSigma _1 \mSigma _2 \, \vt _{\vlambda }\left (\rvvu \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \label {eq:general_grad_norm reparam_eq1} \\ &\qquad + \left ( 1 + d \right ) \vmu _1^{\top } \mSigma _1 \mSigma _2 \vmu _2.\label {eq:general_grad_norm reparam_eq2} \end {alignat} Now for \cref {eq:general_grad_norm reparam_eq1}, \begin {alignat}{2} &\mathbb {E} {\vt _{\vlambda }\left (\rvvu \right )}^{\top } \mSigma _1 \mSigma _2 \, \vt _{\vlambda }\left (\rvvu \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\;= \mathbb {E} {\left (\mC \rvvu + \vm \right )}^{\top } \mSigma _1 \mSigma _2 \left (\mC \rvvu + \vm \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\;= \mathbb {E} \mathrm {tr}\left ( \rvvu ^{\top } \mC ^{\top } \mSigma _1 \mSigma _2 \mC \rvvu \right ) \nonumber \\ &\qquad + \mathbb {E} \mathrm {tr}\left ( \rvvu ^{\top } \mC ^{\top } \mSigma _1 \mSigma _2 \mC \, \rvvu \rvvu ^{\top } \rvvu \right ) \label {eq:thm:general_grad_norm_reparam_eq1} \\ &\qquad + \vm ^{\top } \mSigma _1 \mSigma _2 \mC \, \mathbb {E} \rvvu \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\qquad + \mathbb {E} \rvvu ^{\top } \left ( 1 + \norm {\rvvu }_2^2 \right ) \mC ^{\top } \mSigma _1 \mSigma _2 \vm \nonumber \\ &\qquad + \vm ^{\top } \mSigma _1 \mSigma _2 \vm \, \mathbb {E} \rvvu \left ( 1 + \norm {\rvvu }_2^2 \right ), \nonumber \shortintertext {using the cyclic property of the trace on \cref {eq:thm:general_grad_norm_reparam_eq1},} &\;= \mathrm {tr}\left ( \mathbb {E} \rvvu \rvvu ^{\top } \mC ^{\top } \mSigma _1 \mSigma _2 \mC \right ) \nonumber \\ &\qquad + \mathrm {tr}\left ( \mC ^{\top } \mSigma _1 \mSigma _2 \mC \, \mathbb {E} \rvvu \rvvu ^{\top } \rvvu \rvvu ^{\top } \right ) \nonumber \\ &\qquad + \vm ^{\top } \mSigma _1 \mSigma _2 \mC \, \mathbb {E} \rvvu \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\qquad + \mathbb {E} \rvvu ^{\top } \left ( 1 + \norm {\rvvu }_2^2 \right ) \mC ^{\top } \mSigma _1 \mSigma _2 \, \vm \nonumber \\ &\qquad + \vm ^{\top } \mSigma _1 \mSigma _2 \vm \, \mathbb {E} \rvvu \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \shortintertext {invoking \cref {thm:u_identities},} &\;= \mathrm {tr}\left ( \left (\mathbb {E}\rvu _i^2\right ) \mI \mC ^{\top } \mSigma _1 \mSigma _2 \mC \right ) \nonumber \\ &\qquad + \mathrm {tr}\left ( \mC ^{\top } \mSigma _1 \mSigma _2 \mC \left (\left (d-1\right ) {\left (\mathbb {E}\rvu _i^2\right )}^2 + \mathbb {E}\rvu _i^4 \right ) \mI \right ) \nonumber \\ &\qquad + \vm ^{\top } \mSigma _1 \mSigma _2 \mC \, \left (\mathbb {E} \rvu _i^3\right ) \mathbf {1} \nonumber \\ &\qquad + \left (\mathbb {E} \rvu _i^3\right ) \mathbf {1}^{\top } \mC ^{\top } \mSigma _1 \mSigma _2 \vm \nonumber \\ &\qquad + \vm ^{\top } \mSigma _1 \mSigma _2 \vm \, \left ( \mathbb {E} \rvu _i^3 \right ) \mathbf {1}, \nonumber \shortintertext {and due to \cref {assumption:symmetric_standard},} &\;= \mathrm {tr}\left ( \mC ^{\top } \mSigma _1 \mSigma _2 \mC \right ) + \left (d - 1 + \kappa \right ) \mathrm {tr}\left ( \mC ^{\top } \mSigma _1 \mSigma _2 \mC \right ) \nonumber \\ &\;= \left (d + \kappa \right ) \mathrm {tr}\left (\mC ^{\top } \mSigma _1 \mSigma _2 \mC \right ) \nonumber \\ &\;= \left (d + \kappa \right ) \mathrm {tr}\left (\mC \mC ^{\top } \mSigma _1 \mSigma _2 \right ). \nonumber \end {alignat} Finally, applying this to \cref {eq:general_grad_norm reparam_eq2}, \begin {alignat*}{2} &\mathbb {E} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu _1\right ) \mSigma _1 \mSigma _2 \left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu _2\right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\;= \left (d + 1\right ) \vmu _1^{\top } \mSigma _1 \mSigma _2 \vmu _2 + \left (d + \kappa \right ) \mathrm {tr}\left (\mC \mC ^{\top } \mSigma _1 \mSigma _2 \right ). \end {alignat*}\end{proof}

\begin{restatable}[]{corollary}{prAtEndRestatexvii}\label{thm:prAtEndxvii}\label {thm:q_grad_norm_reparam} Let \(\vt _{\vlambda }: \mathbb {R}^d \mapsto \mathbb {R}^d\) be defined as in \cref {def:reparam} with parameters \(\vlambda = \left (\vm , \mC \right )\) such that \(\vm \in \mathbb {R}^d\) and \(\mC \in \mathbb {R}^{d \times d}\). Also, let \(\rvvu = \left (\rvu _1, \ldots , \rvu _d \right )\) be a vector-valued random variable sampled as \(\rvvu \sim \varphi \), where \(\varphi \) is defined as in \cref {assumption:symmetric_standard} with kurtosis \(\kappa = \mathbb {E}\rvu _i^4\). Then, \begin {alignat*}{2} &\mathbb {E} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right ) {\left ( \mC \mC ^{\top }\right )}^{-\top } {\left ( \mC \mC ^{\top }\right )}^{-1} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \\ &\;= \left (d + 1\right ) \vm ^{\top } {\left ( \mC \mC ^{\top }\right )}^{-\top } {\left ( \mC \mC ^{\top }\right )}^{-1} \vm + \left (d + \kappa \right ) \mathrm {tr}\left ( {\left ( \mC \mC ^{\top } \right )}^{-1} \right ). \end {alignat*}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxvii}From \cref {thm:general_grad_norm_reparam}, we have \begin {alignat}{2} &\mathbb {E} {\left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right )}^{\top } {\left ( \mC \mC ^{\top }\right )}^{-\top } {\left ( \mC \mC ^{\top }\right )}^{-1} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\;= \left (d + 1\right ) \vm ^{\top } {\left ( \mC \mC ^{\top }\right )}^{-\top } {\left ( \mC \mC ^{\top }\right )}^{-1} \vm \nonumber \\ &\quad + \left (d + \kappa \right ) \mathrm {tr}\left (\mC \mC ^{\top } {\left ( \mC \mC ^{\top }\right )}^{-\top } {\left ( \mC \mC ^{\top }\right )}^{-1}\right ).\label {thm:q_grad_norm_reparam_eq1} \end {alignat} Since, by the basic properties of the trace, \begin {alignat*}{2} \mathrm {tr}\left (\mC \mC ^{\top } {\left ( \mC \mC ^{\top }\right )}^{-\top } {\left ( \mC \mC ^{\top }\right )}^{-1}\right ) &= \mathrm {tr}\left ( {\left ( \mC \mC ^{\top }\right )}^{-1} \mC \mC ^{\top } {\left ( \mC \mC ^{\top }\right )}^{-\top } \right ) \\ &= \mathrm {tr}\left ( \mI \, {\left ( \mC \mC ^{\top }\right )}^{-\top } \right ) \\ &= \mathrm {tr}\left ( {\left ( \mC \mC ^{\top }\right )}^{-\top } \right ) \\ &= \mathrm {tr}\left ( {\left ( \mC \mC ^{\top } \right )}^{-1} \right ), \end {alignat*} \cref {thm:q_grad_norm_reparam_eq1} becomes \begin {alignat*}{2} &\mathbb {E} {\left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right )}^{\top } {\left ( \mC \mC ^{\top }\right )}^{-\top } {\left ( \mC \mC ^{\top }\right )}^{-1} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \\ &\;= \left (d + 1\right ) \vm ^{\top } {\left ( \mC \mC ^{\top }\right )}^{-\top } {\left ( \mC \mC ^{\top }\right )}^{-1} \vm + \left (d + \kappa \right ) \mathrm {tr}\left ( {\left ( \mC \mC ^{\top } \right )}^{-1} \right ). \end {alignat*}\end{proof}


==> main-figure0-pratendlowerboundtheorem.tex <==


\prAtEndRestatexviii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxviii}\par The STL estimator is obtained by setting \begin {alignat*}{2} f\left ( \vz \right ) = -\log p\left (\vz , \vx \right ) + \log q_{\vgamma }\left ( \vz \right ) \lvert _{\vgamma = \vlambda }. \end {alignat*} We first consider the log joint likelihood of the model to be \begin {alignat*}{2} \log p\left (\vz , \vx \right ) = -\frac {1}{2} {\left (\vz - \vmu \right )}^{-1} \mSigma ^{-1} \left (\vz - \vmu \right ), \end {alignat*} which is the unnormalized log probability density of a multivariate normal distribution with mean \(\vmu \) and covariance \(\mSigma \). We also set the variational family to be multivariate normal with mean (location) \(\vm \) and covariance (scale) \(\mC \mC ^{\top }\). Given these, the objective function is \begin {alignat*}{2} F\left (\vlambda \right ) &= \mathbb {E} f\left (\vt _{\vlambda }\left (\rvvu \right )\right ) \\ &= \mathbb {E}\log p\left (\vt _{\vlambda }\left (\rvvu \right )\right ) - \mathbb {E}\log q_{\vgamma }\left (\vt _{\vlambda }\left (\rvvu \right )\right ) \big \lvert _{\vgamma = \vlambda } \end {alignat*} \par From~\cref {thm:general_quad_reparam}, the likelihood term is \begin {alignat*}{2} &\mathbb {E}\log p\left (\vt _{\vlambda }\left (\rvvu \right )\right ) \\ &\;= -\frac {1}{2} {\left (\vm - \vmu \right )}^{\top } \mSigma ^{-1} \left (\vm - \vmu \right ) - \frac {1}{2} \mathrm {tr}\left (\mSigma ^{-1} \mC \mC ^{\top } \right ), \end {alignat*} while from~\cref {thm:q_quad_reparam}, the entropy term is \begin {alignat*}{2} &\mathbb {E}\log q_{\vlambda }\left (\vt _{\vlambda }\left (\rvvu \right )\right ) \\ &\;= -\frac {1}{2} \mathbb {E} {\left ( \vt _{\vlambda }\left (\rvvu \right ) - \vm \right )}^{\top } \mS ^{-1} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right ) - \frac {1}{2}\log \abs {\mS } + Z, \\ &\;= -\frac {1}{2} d - \frac {1}{2}\log \abs {\mS } + Z, \end {alignat*} where, \(\mS = \mC \mC ^{\top }\) and \(Z\) is a constant independent of \(\vm \) and \(\mC \). The derivative of the \(f\) is given as \begin {alignat}{2} &\nabla f\left (\vt _{\vlambda }\left (\vu \right )\right ) \nonumber \\ &\;= -\nabla \log p\left (\vt _{\vlambda }\left (\vu \right )\right ) + \nabla \log q_{\vgamma }\left (\vt _{\vlambda }\left (\vu \right )\right ) \lvert _{\vgamma = \vlambda } \nonumber \\ &\;= \mSigma ^{-1} \left (\vt _{\vlambda }\left (\vu \right ) - \vmu \right ) - {\mS }^{-1} \left ( \vt _{\vgamma }\left (\vu \right ) - \vm \right ) \lvert _{\vgamma = \vlambda }.\label {eq:gradient_lower_bound_f_derivative} \end {alignat} \par \begin {alignat*}{2} \mathbb {E} \norm {\vg \left (\vlambda \right )}_2^2 = \frac {1}{M} \mathbb {E} \norm { \nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\rvvu \right ) \right ) }_2^2 + \frac {M-1}{M} \norm { \nabla F\left (\vlambda \right ) }_2^2 \end {alignat*} \par We now compute the expectation of the squared gradient norm. First, by starting from \cref {thm:variational_gradient_norm_identity}, \begin {alignat}{2} &\mathbb {E}\norm { \nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\rvvu \right ) \right ) }_2^2 \nonumber \\ &\;= \mathbb {E} \norm { \nabla f\left ( \vt _{\vlambda }\left (\rvvu \right ) \right ) }_2^2 \left ( 1 + \norm {\rvvu }_2^2 \right ), \nonumber \shortintertext {plugging in \cref {eq:gradient_lower_bound_f_derivative},} &\;= \mathbb {E} \norm {\, \mSigma ^{-1} \left (\vt _{\vlambda }\left (\vu \right ) - \vmu \right ) - {\mS }^{-1} \left ( \vt _{\vlambda }\left (\vu \right ) - \vm \right )\,}^2_2 \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\;= \mathbb {E} {\left (\vt _{\vlambda }\left (\vu \right ) - \vmu \right )}^{\top } \mSigma ^{-\top } \mSigma ^{-1} \left (\vt _{\vlambda }\left (\vu \right ) - \vmu \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\qquad - 2\,\mathbb {E} {\left (\vt _{\vlambda }\left (\vu \right ) - \vmu \right )}^{\top } \mSigma ^{-\top } \mS ^{-1} \left (\vt _{\vlambda }\left (\vu \right ) - \vm \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\qquad + \mathbb {E} {\left (\vt _{\vlambda }\left (\vu \right ) - \vm \right )}^{\top } \mS ^{-\top } \mS ^{-1} \left (\vt _{\vlambda }\left (\vu \right ) - \vm \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ), \nonumber \shortintertext {applying \cref {thm:general_grad_norm_reparam},} &\;= \left (d+1\right ) \vmu ^{\top } \mSigma ^{-\top } \mSigma ^{-1} \vmu + \left (d+\kappa \right ) \mathrm {tr}\left (\mS \mSigma ^{-\top } \mSigma ^{-1}\right ) \nonumber \\ &\qquad - 2 \, \left (d+1\right ) \vmu ^{\top } \mSigma ^{-\top } \mS ^{-1} \vm - 2\,\left (d+\kappa \right ) \mathrm {tr}\left (\mS \mSigma ^{-\top } \mS ^{-1}\right ) \nonumber \\ &\qquad + \left (d+1\right ) \vm ^{\top } \mS ^{-\top } \mS ^{-1} \vm + \left (d+\kappa \right ) \mathrm {tr}\left (\mS ^{-1}\right ), \nonumber \\ \shortintertext {and after regroupping the terms,} &\;= \left (d+1\right ) \left ( \vmu ^{\top } \mSigma ^{-\top } \mSigma ^{-1} \vmu - 2 \vmu ^{\top } \mSigma ^{-\top } \mS ^{-1} \vm + \vm ^{\top } \mS ^{-\top } \mS ^{-1} \vm \right ) \nonumber \\ &\qquad + \left (d+\kappa \right ) \left ( \mathrm {tr}\left (\mS \mSigma ^{-\top } \mSigma ^{-1}\right ) -2 \mathrm {tr}\left (\mS \mSigma ^{-\top } \mS ^{-1}\right ) + \mathrm {tr}\left (\mS ^{-1}\right ) \right ). \nonumber \end {alignat} This expression itself is not very convenient to work with due to the inner product term of \(\vmu \) and \(\vm \). Thus, we focus on the special case \(\vmu = \mathbf {0}\). Then, \begin {alignat}{2} &\mathbb {E}\norm { \nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\rvvu \right ) \right ) }_2^2 \nonumber \\ &\;= \left (d+1\right )\vm ^{\top } \mS ^{-\top } \mS ^{-1} \vm \nonumber \\ &\quad + \left (d+\kappa \right ) \left ( \mathrm {tr}\left (\mS \mSigma ^{-\top } \mSigma ^{-1}\right ) -2 \, \mathrm {tr}\left (\mSigma ^{-\top }\right ) + \mathrm {tr}\left (\mS ^{-1}\right ) \right ) \nonumber \\ &\;= \left (d+1\right )\vm ^{\top } \mS ^{-\top } \mS ^{-1} \vm \nonumber \\ &\quad + \left (d+\kappa \right ) \left ( \mathrm {tr}\left (\mS \mSigma ^{-\top } \mSigma ^{-1}\right ) + \mathrm {tr}\left (\mS ^{-1}\right ) \right ) \nonumber \\ &\quad - \underbrace { 2 \left (d+\kappa \right ) \mathrm {tr}\left (\mSigma ^{-\top }\right ) }_{\text {constant with respect to \(\vlambda \)}} \end {alignat} This also simplifies the suboptimality gap as \begin {alignat}{2} & F\left (\vlambda \right ) - F\left (\vlambda ^{*}\right ) \nonumber \\ &\;= \frac {1}{2} \vm ^{\top } \mSigma ^{-1} \vm + \frac {1}{2} \left ( \mathrm {tr}\left (\mSigma ^{-1} \mS \right ) + \mathrm {tr}\left (\mSigma ^{-1} \mS ^* \right ) \right ) \nonumber \\ &\qquad + \frac {1}{2} \left ( -\log \abs {\mS } + \log \abs {\mS ^*} \right ). \nonumber \\ &\;= \frac {1}{2} \vm ^{\top } \mSigma ^{-1} \vm + \frac {1}{2} \left ( \mathrm {tr}\left (\mSigma ^{-1} \mS \right ) - \log \abs {\mS } \right ) \nonumber \\ &\qquad - \underbrace {\frac {1}{2} \,\left (\mathrm {tr}\left (\mSigma ^{-1} \mS ^* \right ) - \log \abs {\mS ^*}\right )}_{\text {constant with respect to \(\vlambda \)}}. \nonumber \end {alignat} \par Showing \begin {alignat}{2} &\vm ^{\top } \mS ^{-\top } \mS ^{-1} \vm \; &&\succeq \; \vm ^{\top } \mSigma ^{-1} \vm \\ &\mathrm {tr}\left (\mS \mSigma ^{-\top } \mSigma ^{-1}\right ) \; &&\succeq \; \mathrm {tr}\left (\mSigma ^{-1} \mS \right ) \\ &\mathrm {tr}\left (\mS ^{-1}\right ) \; &&\succeq \; -\log \abs {\mS } \end {alignat}for proves the statement.\end{proof}

\prAtEndRestatexix*


==> main-figure0-pratendupperboundkeylemmagradientnormbound.tex <==


\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndiii}The proof continues from the result of \cref {thm:general_variational_gradient_norm_identity}. \par \paragraph {Proof for Cholesky} \cref {thm:general_variational_gradient_norm_identity} shows that \begin {alignat*}{2} \norm { \nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) }_2^2 = {\lVert \vg _{f} \rVert }_2^2 + \vg _{f}^{\top } \mY \vg _{f} + \vg _{f}^{\top } \mU \left ( \mPhi - \mI \right ) \vg _{f}. \end {alignat*} \par By the 1-Lipschitz assumption, the entries of the diagonal matrix \(\Phi \) satisfy \begin {align*} \Phi _{ii} = {\phi ^{\prime }\left (d_i\right )}^2 \leq 1, \end {align*} which means \begin {alignat*}{2} \mPhi \preceq \mI \;\Rightarrow \; \mU \left ( \mPhi - \mI \right ) \preceq 0 \;\Rightarrow \; {\vg _{f}}^{\top } \mU \left ( \mPhi - \mI \right ) \vg _{f} \leq 0. \end {alignat*} Therefore, for the full rank Cholesky parameterization and a 1-Lipschitz positive map \(\phi \), \begin {alignat*}{2} &\norm {\nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vu \right ) \right )}_2^2 \\ &\;= {\lVert \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \rVert }_2^2 + {\vg _{f}}^{\top } \mY \vg _{f} + {\vg _{f}}^{\top } \mU \left ( \mPhi - \mI \right ) \vg _{f} \\ &\;\leq {\lVert \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \rVert }_2^2 + {\vg _{f}}^{\top } \mY \vg _{f} \\ &\;\leq {\lVert \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \rVert }_2^2 + \norm { \mY }_{2,2} {\lVert \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \rVert }_2^2 \\ &\;= {\lVert \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \rVert }_2^2 + \left ( \sum ^{d}_{i=1} u_{i}^2 \right ) {\lVert \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \rVert }_2^2 \\ &\;= \left (1 + \norm {\vu }^2_2\right ) {\lVert \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \rVert }_2^2, \end {alignat*} where \(\norm {\mU }_{2,2}\) is the \(L_2\) operator norm of \(\mU \). This upper bound coincides with that of the matrix square root parameteration. Thus, unforunately, this bound fails to acknowledge the lower variance of the Cholesky, coinciding with that of the matrix square root parameterization. \par \paragraph {Proof for Mean-field (\cref {def:meanfield})} For the mean-field parameterization,~\cref {thm:general_variational_gradient_norm_identity} shows that \begin {alignat*}{2} \norm { \nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) }_2^2 = {\lVert \vg _{f} \rVert }_2^2 + \mathrm {tr}\left ( \vg _{f} \vg _{f}^{\top } \mU \mPhi \right ), \end {alignat*} \par For the second term, \begin {alignat*}{2} \mathrm {tr}\left ( \vg _{f} \vg _{f}^{\top } \mU \mPhi \right ) &= \vg _{f}^{\top } \left ( \mU \mPhi \right ) \vg _{f} \\ &\leq {\lVert \mU \rVert }_{2,2} {\lVert \mPhi \rVert }_{2,2} {\lVert \vg _{f} \rVert }^2_2. \end {alignat*} By the \(1\)-Lipschitzness of \(\phi \), \[ {\lVert \mPhi \rVert }_{2,2} = \sigma _{\mathrm {max}}\left ( \mPhi \right ) = \max _{i = 1, \ldots , d} {\phi ^{\prime }\left ( s_i \right )}^2 \leq 1. \] Then, \begin {alignat}{2} \vg _{f}^{\top } \left ( \mU \mPhi \right ) \vg _{f} &\leq {\lVert \mU \rVert }_{2,2} \, {\lVert \vg _{f} \rVert }^2_2 \label {eq:variational_gradient_norm_identity_mf_eq1} \\ &\leq {\lVert \mU \rVert }_{\mathrm {F}} \, {\lVert \vg _{f} \rVert }^2_2, \label {eq:variational_gradient_norm_identity_mf_eq2} \end {alignat} which gives the result. Here, unlike the bounds on \(\mPhi \), the bounds in \cref {eq:variational_gradient_norm_identity_mf_eq1,eq:variational_gradient_norm_identity_mf_eq2} are quite loose, and become looser as the dimensionality increases. \par \end{proof}


==> main-figure0-pratendupperboundkeylemmagradientnormidentity.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndii}\begin {alignat}{2} &\norm {\nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) }_2^2 \nonumber \\ &\;= {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \nonumber \\ &\;= {\nabla f^{\top }\left ( \vt _{\vlambda }\left (\vu \right ) \right )} {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \nonumber \\ &\;= {\vg _{f}^{\top }} {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \vg _{f}.\label {eq:variational_gradient_norm_identity_eq1} \end {alignat} \par \paragraph {Proof for Cholesky} \par Let \(p\) denote the number of scalar variational parameters such that \(\vlambda = (\lambda _1, \ldots , \lambda _p)\). Then, \begin {alignat*}{2} &{\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \\ &\;= \sum ^{d}_{i=1} \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial m_i } {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial m_i } \right )}^{\top } + \sum ^{d}_{i=1} \sum ^{d}_{j \leq i} \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } \right )}^{\top }, \end {alignat*} where \(\lambda _{C_{ij}}\) denote the parameter responsible for the \(ij\)-th entry of \(\mC \), \(C_{ij}\). Notice that, unlike for the matrix square root parameterization~\citep {domke_provable_2019}, the sum for \(C_{ij}\) is only over the lower triangular section. \par For the derivatives with respect to \(m_i\) and \(C_{ij}\), \citet {domke_provable_2020, domke_provable_2019} show that \begin {alignat}{2} \frac {\partial \vt _{\vlambda }\left (\vu \right ) }{ \partial m_i } &= \ve _i \quad \frac {\partial \vt _{\vlambda }\left (\vu \right ) }{ \partial C_{ij} } &= \ve _i u_j,\label {eq:covariance_derivative} \end {alignat} where \(\ve _i\) is the unit basis of the \(i\)th component. \par Therefore, \begin {alignat}{2} &{\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \nonumber \\ &\;= \sum ^{d}_{i=1} \ve _i \ve _i^{\top } + \sum ^{d}_{i=1} \sum _{j \leq i} \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } \right )}^{\top } \nonumber \\ &\;= \mI + \underbrace { \sum ^{d}_{i=1} \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ii}} } {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ii}} } \right )}^{\top } }_{\text {diagonal of \(\mC \)}} \nonumber \\ &\qquad + \underbrace { \sum ^{d}_{i=1} \sum _{j < i} \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } \right )}^{\top }}_{\text {off-diagonal of \(\mC \)}}, \label {eq:thm:variational_gradient_norm_identity_eq2} \end {alignat} leaving us with the derivatives of the scale term. \par The gradient with respect to \(\lambda _{C_{ij}}\), however, depends on the parameterization. That is, \begin {alignat}{2} \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } &= \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial C_{ij} } \frac { \partial C_{ij} }{ \partial \lambda _{C_{ij}} } &= \ve _i u_j \frac { \partial C_{ij} }{ \partial \lambda _{C_{ij}} }. \label {eq:thm:variational_gradient_norm_identity_covderivative} \end {alignat} \par For the diagonal elements, \(\lambda _{C_{ii}} = d_i\). Thus, \begin {align} \frac { \partial C_{ii} }{ \partial s_i } = \frac { \partial \phi \left (s_i\right ) }{ \partial s_i } = \phi ^{\prime }\left (s_i\right ). \label {eq:thm:variational_gradient_norm_identity_diag} \end {align} And for the off-diagonal elements, \(\lambda _{L_{ij}} = L_{ij}\), and \begin {align} \frac { \partial C_{ij} }{ \partial L_{ij} } = 1. \label {eq:thm:variational_gradient_norm_identity_offdiag} \end {align} \par Plugging \cref {eq:thm:variational_gradient_norm_identity_diag,eq:thm:variational_gradient_norm_identity_offdiag,eq:thm:variational_gradient_norm_identity_covderivative} into \cref {eq:thm:variational_gradient_norm_identity_eq2}, \begin {alignat}{2} &{\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \nonumber \\ &\;= \mI + \underbrace { \sum ^{d}_{i=1} {\left ( u_i \phi ^{\prime }\left (s_i\right ) \right )}^2 \ve _i \ve _i^{\top } }_{\text {diagonal of \(\mC \)}} + \underbrace { \sum ^{d}_{i=1} \sum _{j=1, j < i} u_j^2 \, \ve _i \ve _i^{\top } }_{\text {off-diagonal of \(\mC \)}} \nonumber \\ &\;= \mI + \underbrace { \sum ^{d}_{i=1} u_i^2 {\left (\phi ^{\prime }\left (s_i\right ) \right )}^2 \ve _i \ve _i^{\top } }_{\text {diagonal of \(\mC \)}} + \underbrace { \sum ^{d}_{i=1} \sum _{j \leq i} u_j^2 \, \ve _i \ve _i^{\top } - \sum ^{d}_{i=1} u_i^2 \, \ve _i \ve _i^{\top } }_{\text {off-diagonal of \(\mC \)}} \nonumber \\ &\;= \mI + \underbrace { \mU \, \mPhi }_{\text {diagonal of \(\mC \)}} + \underbrace { \mY - \mU }_{\text {off-diagonal of \(\mC \)}} \nonumber \\ &\;= \left ( \mI + \mY \right ) + \mU \left ( \mPhi - \mI \right ), \label {eq:variational_gradient_norm_identity_jacinner} \end {alignat} where \(\mU ,\mPhi \) are diagonal matrices defined as \begin {alignat*}{2} & \mPhi &&= \mathrm {diag}\left ( \left [ {\phi ^{\prime }\left (s_1\right )}^2, \ldots , {\phi ^{\prime }\left (s_d\right )}^2 \right ] \right ) \\ &\mU &&= \mathrm {diag}\left ( \left [ u_1^2, \ldots , u_d^2 \right ] \right ) \\ &\mY &&= \mathrm {diag}\left ( \left [ u_1^2, u_1^2 + u_2^2,\, \ldots \,, {\textstyle \sum ^{d}_{i=1} u_i^2} \right ] \right ). \end {alignat*} The major difference with the proof of \citet [Lemma 8]{domke_provable_2019} for the matrix square root case is that we sum of the \(u_j^2 \ve _i \ve _i^{\top }\) terms is over the \textit {lower diagonal elements} instead of all the elements. This is the variance reduction effect we get for using the Cholesky parameterization. \par Coming back to \cref {eq:variational_gradient_norm_identity_eq1}, \begin {alignat}{2} &\norm {\nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vu \right ) \right )}_2^2 \nonumber \\ \;&= \vg _f^{\top } {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \vg \nonumber \\ &= \vg _{f}^{\top } \Big ( \left ( \mI + \mY \right ) + \mU \left ( \mPhi - \mI \right ) \Big ) \vg _{f} \nonumber \\ &= {\lVert \vg _{f} \rVert }_2^2 + \vg _{f}^{\top } \mY \vg _{f} + \vg _{f}^{\top } \mU \left ( \mPhi - \mI \right ) \vg _{f}. \label {eq:variational_gradient_norm_identity_conclusion} \end {alignat} \par \paragraph {Proof for Mean-field} For the mean-field variational family, the covariance has only diagonal elements. Therefore, \cref {eq:variational_gradient_norm_identity_jacinner} becomes \begin {alignat}{2} {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } &= \mI + \mU \mPhi , \nonumber \end {alignat} and \cref {eq:variational_gradient_norm_identity_conclusion} becomes \begin {alignat}{2} \norm {\nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vu \right ) \right )} = \vg _{f}^{\top } \left ( \mI + \mU \mPhi \right ) \vg _{f} = {\lVert \vg _{f} \rVert }_2^2 + \vg _{f}^{\top } \mU \mPhi \vg _{f}. \nonumber \end {alignat}\end{proof}


==> main-figure0-pratendupperboundkeylemmameanfield.tex <==


\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndiv}The key idea is to prove a similar result as \cref {thm:reparam_u_identity}. For terms that zero-out during during the proof of \cref {thm:reparam_u_identity}, we apply \cref {thm:meanfield_superiority} to zero-out those same terms. \par \begin {alignat}{2} &\mathbb {E}\norm {\vt _{\vlambda }\left (\rvvu \right ) - \vz }_2^2 \, \left ( 1 + \norm {\mU }_{\mathrm {F}} \right ) \nonumber \\ &\;= \mathbb {E} \rvvu ^{\top } \mC ^{\top } \mC \rvvu \, \left ( 1 + \norm {\mU }_{\mathrm {F}} \right ) \nonumber \\ &\;\quad + 2\,\mathbb {E} \rvvu ^{\top } \mC ^{\top } \left ( \vm - \vz \right ) \left ( 1 + \norm {\mU }_{\mathrm {F}} \right ) \nonumber \\ &\;\quad + {\left ( \vm - \vz \right )}^{\top } \left ( \vm - \vz \right ) \left ( 1 + \mathbb {E} \norm {\mU }_{\mathrm {F}} \right ) \nonumber \shortintertext {invoking the trace trick,} &\;= \norm {\vm - \vz } \left ( 1 + \mathbb {E} \norm {\mU }_{\mathrm {F}}\right ). \nonumber \\ &\;\quad + 2\,\mathbb {E} \left ( 1 + \norm {\mU }_{\mathrm {F}} \right ) \, \rvvu ^{\top } \mC ^{\top } \left ( \vm - \vz \right ) \nonumber \\ &\;\quad + \mathrm {tr}\left ( \mC ^{\top } \mC \, \mathbb {E} \rvvu \rvvu ^{\top } \left ( 1 + \norm {\mU }_{\mathrm {F}}\right ) \right ) \nonumber \end {alignat} \par \begin {alignat*}{2} \mathbb {E} \norm {\mathbfsf {U}}_{\mathrm {F}} &\;= \mathbb {E} \sqrt { \mathrm {tr}\left ( \mathbfsf {U} \mathbfsf {U} \right ) } \\ &\;= \mathbb {E} \sqrt { \sum _{i=1}^d \rvu _i^4 }, \shortintertext {using Jensen's inequality,} &\;\leq \sqrt { \mathbb {E} \sum _{i=1}^d \rvu _i^4 } \\ &\;= \sqrt { d \kappa }. \end {alignat*} \par \begin {alignat*}{2} \mathbb {E} \left ( \norm {\mathbfsf {U}}_{\mathrm {F}} + 1\right ) \rvu _i &\;= \mathbb {E} \left ( \sqrt { \sum ^d_{i=1} \rvu _i^4 } + 1\right ) \rvu _i , \shortintertext {applying \(\sqrt {a + b} \leq \sqrt {a} + \sqrt {b}\),} &\;\leq \mathbb {E} \left ( \sum ^d_{i=1} \rvu _i^2 + 1\right ) \rvu _i \\ &\;= \mathbb {E} \, \rvu _i \, \sum _{j \neq i} \rvu _j^2 + \rvu _i^3 + \rvu _i, \shortintertext {and applying \cref {assumption:symmetric_standard},} &\;= 0. \end {alignat*} \par \begin {alignat*}{2} \mathbb {E} \rvu _i \rvu _j \norm {\mathbfsf {U}}_{\mathrm {F}} &\;= \mathbb {E} \rvu _i \rvu _j \left ( \sqrt { \sum _{k=1}^d \rvu _k^4 } \right ), \shortintertext {again, applying \(\sqrt {a + b} \leq \sqrt {a} + \sqrt {b}\),} &\;\leq \mathbb {E} \rvu _i \rvu _j \sum _{k=1}^d \rvu _k^2, \shortintertext {decomposing the sum,} &\;= \mathbb {E} \rvu _i^3 + \rvu _j^3 + \rvu _i \rvu _j \sum _{k \neq i, k \neq j} \rvu _k^2, \shortintertext {and applying \cref {assumption:symmetric_standard},} &\;= 0. \end {alignat*} \par \begin {alignat*}{2} \mathbb {E} \rvu _i \rvu _i \norm {\mathbfsf {U}}_{\mathrm {F}} &\;= \mathbb {E} \rvu _i^2 \left ( \sqrt { \sum _{k=1}^d \rvu _k^4 } \right ), \shortintertext {applying Cauchy-Schwarz's inequality for expectations,} &\;\leq \sqrt { \left ( \mathbb {E} \sum _{k=1}^d \rvu _k^4 \right ) \left ( \mathbb {E} \rvu _i^4 \right ) }, \shortintertext {and given \cref {assumption:symmetric_standard},} &\;= \sqrt { \left ( d \kappa \right ) \left ( \kappa \right ) } \\ &\;= \kappa \sqrt { d }. \end {alignat*} \par Combining all the results, \begin {alignat*}{2} &\mathbb {E}\norm {\vt _{\vlambda }\left (\rvvu \right ) - \vz }_2^2 \, \left ( 1 + \norm {\mU }_{\mathrm {F}} \right ) \\ &\;\leq \norm { \vm - \vz }_2^2 \left ( \vm - \vz \right ) \left ( 1 + \mathbb {E} \norm {\mU }_{\mathrm {F}}\right ) \\ &\;\quad + 2\,\mathbb {E} \left ( 1 + \norm {\mU }_{\mathrm {F}} \right ) \, \rvvu ^{\top } \mC ^{\top } \left ( \vm - \vz \right ) \\ &\;\quad + \mathrm {tr}\left ( \mC ^{\top } \mC \, \mathbb {E} \rvvu \rvvu ^{\top } \left ( 1 + \norm {\mU }_{\mathrm {F}}\right ) \right ) \\ &\;\leq \sqrt {d \kappa } \norm { \vm - \vz }_2^2 + \mathrm {tr}\left ( \mC ^{\top } \mC \left (\mI + \kappa \sqrt {d} \mI \right ) \right ) \\ &\;= \sqrt {d \kappa } \norm { \vm - \vz }_2^2 + \left (\kappa \sqrt {d} + 1\right ) \mathrm {tr}\left ( \mC ^{\top } \mC \right ) \\ &\;= \sqrt {d \kappa } \norm { \vm - \vz }_2^2 + \left (\kappa \sqrt {d} + 1\right ) \norm { \mC }_{\mathrm {F}}^2. \end {alignat*} \par \end{proof}


==> main-figure0-pratendupperboundkeylemmavariancegeneral.tex <==


\prAtEndRestateviii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndviii}From the definition of variance, \begin {alignat}{2} &\mathbb {E} \norm {\vg _M }^2_2 \nonumber \\ &\;= \mathrm {tr}\,\V { \vg _M } + \norm {\mathbb {E} \vg }^2_2, \nonumber \shortintertext {following the definition in \cref {eq:def_gradient_M_est},} &\;= \mathrm {tr}\,\V { \frac {1}{M} \sum _{m=1}^M \vg _m } + \norm { \nabla F\left (\vlambda \right ) }^2_2, \nonumber \shortintertext {and then the definition in \cref {eq:def_gradient_m_est},} &\;= \mathrm {tr}\,\V { \frac {1}{M} \sum _{m=1}^M \nabla _{\vlambda } f\left (\vt _{\vlambda }\left (\rvvu _m\right )\right ) + \nabla h\left (\vlambda \right ) } + \norm { \nabla F\left (\vlambda \right ) }^2_2, \nonumber \shortintertext {by the linearity of variance,} &\;= \frac {1}{M} \mathrm {tr}\,\V { \nabla _{\vlambda } f\left (\vt _{\vlambda }\left (\rvvu \right )\right ) } + \norm { \nabla F\left (\vlambda \right ) }^2_2 \\ &\;= \frac {1}{M} \left ( \mathbb {E}{ \norm {\nabla _{\vlambda } f\left (\vt _{\vlambda }\left (\rvvu \right )\right )}_2^2 } - \norm { \mathbb {E}{ \nabla _{\vlambda } f\left (\vt _{\vlambda }\left (\rvvu \right )\right )} }_2^2 \right ) + \norm { \nabla F\left (\vlambda \right ) }^2_2 \nonumber \\ &\;\leq \frac {1}{M} \mathbb {E}{ \norm { \nabla _{\vlambda } f\left (\vt _{\vlambda }\left (\rvvu \right )\right ) }_2^2 } + \norm { \nabla F\left (\vlambda \right ) }^2_2. \nonumber \end {alignat} The results follow from applying \cref {thm:general_variational_gradient_norm_bound} accordingly. \par \todo [inline]{ I think it might be possible to do something about the \[ -\norm {\mathbb {E}{ \nabla _{\vlambda } f\left (\vt _{\vlambda }\left (\rvvu \right )\right )}}_2^2 \] term instead of just upper bounding it by 0. In fact, it is possible to generalize \cref {thm:general_variational_gradient_norm_identity} such that \begin {align*} &\inner { \nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) }{ \nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vv \right ) \right ) } \\ &\;= \left (1 + \inner {\vu }{\vv }\right ) \inner {\vg _{f,\vu }}{\vg _{f,\vv }} + \mathrm {tr}\left ( \vg _{f,\vu } \vg _{f,\vv }^{\top }\, \vv \vu ^{\top } \left ( \Phi ^2 - \mI \right ) \right ), \end {align*} where \(\vg _{f,\vu } = \nabla f\left (\vt _{\vlambda }\left (\vu \right )\right )\). }\end{proof}


==> main-figure0-pratendupperboundlemma.tex <==


\begin{restatable}[]{lemma}{prAtEndRestateix}\label{thm:prAtEndix}\label {thm:reparam_quadratic} Let \(\vt _{\vlambda }: \mathbb {R}^d \mapsto \mathbb {R}^d\) be defined as in \cref {def:reparam} with parameters \(\vlambda = \left (\vm , \mC \right )\) such that \(\vm \in \mathbb {R}^d\) and \(\mC \in \mathbb {R}^{d \times d}\). Also, let \(\vz \in \mathbb {R}^d\) be some vector, and \(\rvvu \sim \varphi \) be some vector-valued random variable, where \(\varphi \) is defined as in \cref {assumption:symmetric_standard}. Then, \begin {alignat*}{2} \mathbb {E}\norm {\vt _{\vlambda }\left (\rvvu \right ) - \vz }_2^2 &= \norm {\vm - \vz }^2_2 + \norm {\mC }_{\mathrm {F}}^2. \end {alignat*}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndix}\begin {alignat}{2} \mathbb {E}\norm { \vt _{\vlambda }\left (\rvvu \right ) - \vz }_2^2 &= \mathbb {E}\norm { \mC \rvvu + \vm - \vz }_2^2 \nonumber \\ &= \mathbb {E} \rvvu ^{\top } \mC ^{\top } \mC \rvvu + 2\,\mathbb {E} \rvvu ^{\top } \mC ^{\top } \vm - 2\,\mathbb {E} \rvvu ^{\top } \mC ^{\top } \vz \nonumber \\ &\;\quad + \vm ^{\top } \vm - 2\,\vm ^{\top } \vz + \vz ^{\top } \vz . \label {eq:reparam_quadratic_eq1} \end {alignat} The first three terms follow as \begin {alignat*}{2} &\mathbb {E} \rvvu ^{\top } \mC ^{\top } \mC \rvvu + 2\,\mathbb {E} \rvvu ^{\top } \mC ^{\top } \vm - 2\,\mathbb {E} \rvvu ^{\top } \mC ^{\top } \vz \\ &\;= \mathbb {E} \mathrm {tr}\left (\rvvu ^{\top } \mC ^{\top } \mC \rvvu \right ) + 2\,\mathbb {E} \rvvu ^{\top } \mC ^{\top } \vm - 2\,\mathbb {E} \rvvu ^{\top } \mC ^{\top } \vz \\ &\;= \mathrm {tr}\left ( \mC ^{\top } \mC \mathbb {E} \rvvu \rvvu ^{\top }\right ) + 2\,\mathbb {E} \rvvu ^{\top } \mC ^{\top } \vm - 2\,\mathbb {E} \rvvu ^{\top } \mC ^{\top } \vz , \shortintertext {applying \cref {thm:u_identities},} &\;= \mathrm {tr}\left ( \mC ^{\top } \mC \right ) \\ &\;= \norm { \mC }_{\mathrm {F}}^2. \end {alignat*} Applying this to \cref {eq:reparam_quadratic_eq1}, \begin {alignat*}{2} \mathbb {E}\norm {\vt _{\vlambda }\left (\rvvu \right ) - \vz }_2^2 &= \vm ^{\top } \vm - 2\,\vm ^{\top } \vz + \vz ^{\top } \vz + \norm {\mC }_{\mathrm {F}}^2 \\ &= \norm {\vm - \vz }^2_2 + \norm {\mC }_{\mathrm {F}}^2. \end {alignat*}\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatex}\label{thm:prAtEndx}\label {thm:tspace_distance} Let \(\vt _{\vlambda }: \mathbb {R}^d \mapsto \mathbb {R}^d\) be defined as in \cref {def:reparam} with parameters \(\vlambda = \left (\vm , \mC \right )\) such that \(\vm \in \mathbb {R}^d\) and \(\mC \in \mathbb {R}^{d \times d}\). Also, let \(\rvvu \sim \varphi \) be some vector-valued random variable, where \(\varphi \) is defined as in \cref {assumption:symmetric_standard}. Then, \begin {alignat*}{2} \mathbb {E}\norm {\vt _{\vlambda }\left (\rvvu \right ) - \vt _{\vlambda ^{\prime }}\left (\rvvu \right )}_2^2 &= \norm {\vm - \vm ^{\prime }}^2_2 + \norm {\mC - \mC ^{\prime }}_{\mathrm {F}}^2. \end {alignat*}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndx}\begin {alignat}{2} \mathbb {E}\norm { \vt _{\vlambda }\left (\rvvu \right ) - \vt _{\vlambda ^{\prime }}\left (\rvvu \right ) }_2^2 &= \mathbb {E}\norm { \left (\mC \rvvu + \vm \right ) - \left ( \mC ^{\prime }\rvvu + \vm ^{\prime } \right ) }_2^2 \nonumber \\ &= \mathbb {E}\norm { \left (\mC - \mC ^{\prime }\right )\rvvu + \left (\vm - \vm ^{\prime }\right ) }_2^2 \nonumber \\ &= \mathbb {E}\rvvu ^{\top } {\left (\mC - \mC ^{\prime }\right )}^{\top } \left (\mC - \mC ^{\prime }\right )\rvvu \nonumber \\ &\;\quad + 2 \mathbb {E} \rvvu ^{\top } {\left (\mC - \mC ^{\prime }\right )}^{\top } {\left (\vm - \vm ^{\prime }\right )} \nonumber \\ &\;\quad + {\left (\vm - \vm \right )}^{\top } \left (\vm - \vm ^{\prime }\right ), \nonumber \shortintertext {invoking the trace trick,} &= \mathbb {E} \mathrm {tr}\left ( \rvvu ^{\top } {\left (\mC - \mC ^{\prime }\right )}^{\top } \left (\mC - \mC ^{\prime }\right )\rvvu \right ) \nonumber \\ &\;\quad + 2 \mathbb {E} \rvvu ^{\top } {\left (\mC - \mC ^{\prime }\right )}^{\top } {\left (\vm - \vm ^{\prime }\right )} \nonumber \\ &\;\quad + {\left (\vm - \vm ^{\prime }\right )}^{\top } \left (\vm - \vm ^{\prime }\right ), \nonumber \shortintertext {using the cyclic property of the trace,} &= \mathrm {tr}\left ( {\left (\mC - \mC ^{\prime }\right )}^{\top } \left (\mC - \mC ^{\prime }\right ) \mathbb {E} \rvvu \rvvu ^{\top } \right ) \nonumber \\ &\;\quad + 2 \mathbb {E} \rvvu ^{\top } {\left (\mC - \mC ^{\prime }\right )}^{\top } {\left (\vm - \vm \right )} \nonumber \\ &\;\quad + {\left (\vm - \vm ^{\prime }\right )}^{\top } \left (\vm - \vm ^{\prime }\right ), \nonumber \shortintertext {and applying \cref {thm:u_identities},} &= \mathrm {tr}\left ( {\left (\mC - \mC ^{\prime }\right )}^{\top } \left (\mC - \mC ^{\prime }\right ) \right ) \nonumber \\ &\;\quad + {\left (\vm - \vm ^{\prime }\right )}^{\top } \left (\vm - \vm ^{\prime }\right ) \nonumber \\ &= \norm { \mC - \mC ^{\prime } }_{\mathrm {F}}^2 + \norm { \vm - \vm ^{\prime } }_2^2. \nonumber \end {alignat}\end{proof}


==> main-figure0-pratendupperboundtheoremboundedentropy.tex <==


\prAtEndRestatexii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxii}The proof is very similar to that of \cref {thm:gradient_upper_bound}. However, we use the fact that the entropic regularizer is bounded such that \[ -h\left (\vlambda \right ) < -h^*. \] From this, we have shown in the \textit {proof sketch} that \begin {alignat}{2} &\mathbb {E} {\lVert \vt _{\vlambda }\left (\rvvu \right ) - \bar {\vzeta }_{\text {H}} \rVert }_2^2 \nonumber \\ &\quad \leq \frac {2}{\mu _{\mathrm {H}}} \left ( F\left (\vlambda \right ) - F^* \right ) + \frac {2}{\mu _{\mathrm {H}}} \left ( F^* - f^*_{\text {H}} - h^*\right ). \label {eq:thm_upper_bound_f_H_quadratic} \end {alignat} \par The proof resumes from \cref {eq:thm1_parameter_suboptimality_unified} as \begin {alignat}{2} &\mathbb {E}\norm {\nabla _{\vlambda } f_{\mathrm {H}}\left (\vt _{\vlambda }\left (\rvvu \right )\right )}_2^2 \nonumber \\ &\;\leq L^2_{\mathrm {H}} C\left (d, \kappa \right ) \mathbb {E} {\Vert \vt _{\vlambda }\left (\rvvu \right ) - \bar {\vzeta }_{\mathrm {H}} \rVert }_2^2, \nonumber \shortintertext {and by applying \cref {eq:thm_upper_bound_f_H_quadratic},} &\;= \frac {2 L^2_{\mathrm {H}} }{\mu _{\mathrm {H}}} C\left (d, \kappa \right ) \left ( F\left (\vlambda \right ) - F^* \right ) + \frac {2 L^2_{\mathrm {H}} }{\mu _{\mathrm {H}}} C\left (d, \kappa \right ) \left ( F^* - f^*_{\text {H}} - h^* \right ). \nonumber \end {alignat} Plugging this to \cref {thm:gradient_variance_general_upper_bound} proves the result.\end{proof}


==> main-figure0-pratendupperboundtheoremklform.tex <==


\prAtEndRestatexi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxi}This proof uses the smoothness of \(f_{\mathrm {KL}}\) instead of \(f_{\mathrm {H}}\). That is, \begin {align} &\mathbb {E} \norm { \nabla f_{\mathrm {KL}}\left (\vt _{\vlambda }\left (\rvvu \right )\right ) }_2^2 \nonumber \\ &\;= \mathbb {E} {\lVert \nabla f_{\mathrm {KL}}\left (\vt _{\vlambda }\left (\rvvu \right )\right ) + \nabla f_{\mathrm {KL}}\left ( \bar {\vzeta }_{\mathrm {KL}} \right ) \rVert }_2^2 \nonumber \shortintertext {applying \cref {eq:thm_upper_bound_smoothness},} &\;\leq L^2_{\mathrm {KL}} \, \mathbb {E} {\lVert \vt _{\vlambda }\left (\rvvu \right ) + \bar {\vzeta }_{\mathrm {KL}} \rVert }_2^2, \label {eq:thm3_kl_smoothness} \end {align} where \(\bar {\vzeta }_{\mathrm {KL}}\) is a stationary point of \(f_{\mathrm {KL}}\). \par Substituting \cref {eq:thm3_kl_smoothness} in \cref {eq:thm1_parameter_suboptimality_unified}, \begin {alignat}{2} &\mathbb {E}\norm {\nabla _{\vlambda } f_{\mathrm {KL}}\left (\vt _{\vlambda }\left (\rvvu \right )\right )}_2^2 \nonumber \\ &\;\leq L^2_{\mathrm {KL}} C\left (d, \kappa \right ) \mathbb {E} {\Vert \vt _{\vlambda }\left (\rvvu \right ) - \bar {\vzeta }_{\mathrm {KL}} \rVert }_2^2, \nonumber \shortintertext {and by applying \cref {eq:thm_upper_bound_f_quadratic} for \(f_{\mathrm {KL}}\),} &\;= \frac {2 L^2_{\mathrm {KL}} }{\mu _{\mathrm {KL}}} C\left (d, \kappa \right ) \left ( F\left (\vlambda \right ) - F^* \right ) + \frac {2 L^2_{\mathrm {KL}} }{\mu _{\mathrm {KL}}} C\left (d, \kappa \right ) \left ( F^* - f^*_{\text {KL}} \right ). \nonumber \end {alignat} Plugging this to \cref {thm:gradient_variance_general_upper_bound} proves the result.\end{proof}


==> main-pratendcommon.tex <==


\prAtEndRestatexi*

\prAtEndRestatexii*

\prAtEndRestatexiii*


==> main-pratendconvexity.tex <==


\prAtEndRestatexx*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxx}Recall that \begin {align} F\left (\vlambda \right ) = \underbrace {\mathbb {E} f\left (\vt _{\vlambda }\left (\rvvu \right )\right )}_{\text {likelihood term}} + \underbrace {h\left (\vlambda \right )}_{\text {regularization term}}. \end {align} We first establish the strong convexity of the likelihood term and then the convexity of the regularization term. \par \paragraph {Strong Convexity of likelihood term} For the matrix square root parameterization (\cref {def:squareroot}), if \(f\) is \(\mu \)-strongly convex, then the likelihood term is also \(\mu \)-strongly convex \citep {domke_provable_2020}. This means that, \begin {align} & \mathbb {E} f\left (\vt _{\vlambda }\left (\rvvu \right )\right ) - \mathbb {E} f\left (\vt _{\vlambda ^{\prime }}\left (\rvvu \right )\right ) \nonumber \\ &\;= \inner {\nabla _{\vlambda ^{\prime }} \mathbb {E} f\left ( \vt _{\vlambda ^{\prime }}\left (\rvvu \right ) \right ) }{ \vlambda - \vlambda ^{\prime } } + \frac {\mu }{2} \mathbb {E}\norm {\vt _{\vlambda }\left (\rvvu \right ) - \vt _{\vlambda ^{\prime }}\left (\rvvu \right )}_2^2 \nonumber \\ &= \inner { \mathbb {E} \frac { \partial \vt _{\vlambda ^{\prime }}\left (\rvvu \right ) }{ \partial \vlambda ^{\prime } } \nabla f \left ( \vt _{\vlambda ^{\prime }}\left (\rvvu \right ) \right ) }{ \vlambda - \vlambda ^{\prime } } + \frac {\mu }{2} \mathbb {E}\norm {\vt _{\vlambda }\left (\rvvu \right ) - \vt _{\vlambda ^{\prime }}\left (\rvvu \right )}_2^2. \label {eq:thm_convexity_inequality} \end {align} Focusing on the inner product term, \begin {align*} &\inner { \mathbb {E} \frac { \partial \vt _{\vlambda ^{\prime }}\left (\rvvu \right ) }{ \partial \vlambda ^{\prime } } \nabla f \left ( \vt _{\vlambda ^{\prime }}\left (\rvvu \right ) \right ) }{ \vlambda - \vlambda ^{\prime } } \\ &\;= \inner { \mathbb {E} \frac { \partial \vt _{\vlambda ^{\prime }}\left (\rvvu \right ) }{ \partial \vm ^{\prime } } \nabla f \left ( \vt _{\vlambda ^{\prime }}\left (\rvvu \right ) \right ) }{ \vm - \vm ^{\prime } } \\ &\;\quad + \sum ^d_{j=1} \sum ^d_{i=1} \left ( \mathbb {E} \frac { \partial \vt _{\vlambda ^{\prime }}\left (\rvvu \right ) }{ \partial C_{ij}^{\prime } } \nabla f \left ( \vt _{\vlambda ^{\prime }}\left (\rvvu \right ) \right ) \right ) \left (C_{ij} - C_{ij}^{\prime }\right ) \\ &\;= \inner { \mathbb {E} \frac { \partial \vt _{\vlambda }\left (\rvvu \right ) }{ \partial \vm ^{\prime } } \nabla f \left ( \vt _{\vlambda ^{\prime }}\left (\rvvu \right ) \right ) }{ \vm - \vm ^{\prime } } \\ &\;\quad + \underbrace { \sum ^d_{j=1} \sum ^d_{i=1,\,i \neq j} \left ( \mathbb {E} \frac { \partial \vt _{\vlambda ^{\prime }}\left (\rvvu \right ) }{ \partial C_{ij}^{\prime } } \nabla f \left ( \vt _{\vlambda ^{\prime }}\left (\rvvu \right ) \right ) \right ) \left (C_{ij} - C_{ij}^{\prime }\right ) }_{\text {off-diagonal of \(\mC \)}} \\ &\;\quad + \underbrace { \sum ^d_{i=1} \left ( \mathbb {E} \frac { \partial \vt _{\vlambda ^{\prime }}\left (\rvvu \right ) }{ \partial C_{ii}^{\prime } } \nabla f \left ( \vt _{\vlambda ^{\prime }}\left (\rvvu \right ) \right ) \right ) \left (C_{ii} - C_{ii}^{\prime }\right ) }_{\text {diagonal of \(\mC \)}}. \end {align*} Furthermore, the diagonal terms can be shown to satisfy \begin {align} &\sum ^d_{i=1} \left ( \mathbb {E} \frac { \partial \vt _{\vlambda ^{\prime }}\left (\rvvu \right ) }{ \partial C_{ii}^{\prime } } \nabla f \left ( \vt _{\vlambda ^{\prime }}\left (\rvvu \right ) \right ) \right ) \left (C_{ii} - C_{ii}^{\prime }\right ) \nonumber \\ &\;= \sum ^d_{i=1} \mathbb {E} u_i \ve _i^{\top } \nabla f \left ( \vt _{\vlambda ^{\prime }}\left (\rvvu \right ) \right ) \left (C_{ii} - C_{ii}^{\prime }\right ).\label {eq:thm_convexity_diagonal_squareroot} \end {align} For the parameterizations in \cref {def:meanfield} and \cref {def:fullrank}, the derivatives only differ for the diagonal of \(\mC \). Specifically, since the diagonals are \(C_{\mathrm {FR},ii} = \phi \left (s_i\right )\), the inner product term of the diagonal entries of the full rank parameterization (\cref {def:fullrank}) is now \begin {align*} &\sum ^d_{i=1} \left ( \mathbb {E} \frac { \partial \vt _{\vlambda ^{\prime }}\left (\rvvu \right ) }{ \partial C_{\mathrm {FR},ii}^{\prime } } \nabla f \left ( \vt _{\vlambda ^{\prime }}\left (\rvvu \right ) \right ) \right ) \left (C_{\mathrm {FR},ii} - C_{\mathrm {FR},ii}^{\prime }\right ) \\ &\;= \sum ^d_{i=1} \mathbb {E} \phi ^{\prime }\left (s_i^{\prime }\right ) u_i \ve _i^{\top } \nabla f \left ( \vt _{\vlambda ^{\prime }}\left (\rvvu \right ) \right ) \left (C_{\mathrm {FR},ii} - C_{\mathrm {FR},ii}^{\prime }\right ) \\ &\;\leq \sum ^d_{i=1} \mathbb {E} u_i \ve _i^{\top } \nabla f \left ( \vt _{\vlambda ^{\prime }}\left (\rvvu \right ) \right ) \left (C_{\mathrm {FR},ii} - C_{\mathrm {FR},ii}^{\prime }\right ), \end {align*} which is equal to~\cref {eq:thm_convexity_diagonal_squareroot}. Therefore, the bound in \cref {eq:thm_convexity_inequality} is preserved, where the strong convexity term \par \paragraph {Convexity of regularization term} For the full-rank Cholesky parameterization \cref {def:fullrank}, the regularization term is \begin {align*} h\left (\vlambda \right ) &= - \mathrm {H}\left (q_{\vlambda }\right ) \\ &= - \mathrm {H}\left (\varphi \right ) - \log \abs { \mC } \\ &= - \mathrm {H}\left (\varphi \right ) - \sum _{i=1}^{d} \log \phi \left (s_i\right ). \end {align*} Showing that \(-\log \phi \) is convex shows that \(h\) is convex since the sum of convex functions is convex. Now, since \begin {align*} -\frac {d^2 \log \phi }{ds^2} = \frac { {\phi ^{\prime }\left (s\right )}^{2} - \phi ^{\prime \prime }\left (x\right ) }{ {\phi \left (s\right )}^{2} } \end {align*} and \(\phi \left (s\right ) > 0\) for all \(s\), any \(\phi \) satisfying results in \(h\) being convex.\end{proof}


==> main-pratenddefaultcategory.tex <==


\prAtEndRestateviii*


==> main-pratendlowerbound.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatex}\label{thm:prAtEndx}Let \(\vt _{\vlambda }: \mathbb {R}^d \mapsto \mathbb {R}^d\) be defined as in \cref {def:reparam} with parameters \(\vlambda = \left (\vm , \mC \right )\) such that \(\vm \in \mathbb {R}^d\) and \(\mC \in \mathbb {R}^{d \times d}\). Also, let \(\rvvu \sim \varphi \), where \(\varphi \) is defined as in \cref {assumption:symmetric_standard}. Then, \begin {alignat*}{2} \mathbb {E}\vt _{\vlambda }\left (\rvvu \right ) \left (1 + \norm {\rvvu }_2^2\right ) = \left (d + 1\right ) \vm . \end {alignat*}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndx}Since \(\rvu _i\) follows a symmetric and standardized distribution, \(\mathbb {E}\rvu _i^3 = 0, \mathbb {E} \rvu _i^2 = 1\). Then, \begin {alignat*}{2} \mathbb {E}\vt _{\vlambda }\left (\rvvu \right ) \left (1 + \norm {\rvvu }_2^2\right ) &= \mathbb {E} \left (\mC \rvvu + \vm \right ) \left (1 + \norm {\rvvu }_2^2\right ) \\ &= \mC \, \mathbb {E} \rvvu \left (1 + \norm {\rvvu }_2^2\right ) + \vm \left (1 + \mathbb {E} \norm {\rvvu }_2^2\right ), \shortintertext {applying \cref {thm:u_identities},} &= \left ( \mathbb {E}\rvu _i^3 \right ) \mC \mathbf {1} + \vm \left (1 + d \, \mathbb {E} \rvu _i^2\right ), \shortintertext {and by~\cref {assumption:symmetric_standard},} &= \left (d + 1\right ) \vm . \end {alignat*}\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexi}\label{thm:prAtEndxi}\label {thm:general_quad_reparam} Let \(\vt _{\vlambda }: \mathbb {R}^d \mapsto \mathbb {R}^d\) be defined as in \cref {def:reparam} with parameters \(\vlambda = \left (\vm , \mC \right )\) such that \(\vm \in \mathbb {R}^d\) and \(\mC \in \mathbb {R}^{d \times d}\). Also, let \(\mSigma \in \mathbb {R}^{d \times d}\) be some matrix, \(\vmu \in \mathbb {R}^d\) be some vector, and \(\rvvu \sim \varphi \) be a vector-valued random variable, where \(\varphi \) is defined as in \cref {assumption:symmetric_standard}. Then, \begin {align*} &\mathbb {E} \, {\left ( \vt _{\vlambda }\left (\rvvu \right ) - \vmu \right )}^{\top } \mSigma \left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu \right ) \\ &\;= {\left (\vm - \vmu \right )}^{\top } \mSigma \left (\vm - \vmu \right ) + \mathrm {tr}\left ({\mSigma }^{-1} \mC \mC ^{\top }\right ). \end {align*}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxi}\begin {alignat}{2} &\mathbb {E} {\left ( \vt _{\vlambda }\left (\rvvu \right ) - \vmu \right )}^{\top } \mSigma \, \left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu \right ) \nonumber \\ &\;= \mathbb {E}\, {\vt _{\vlambda }\left (\rvvu \right )}^{\top } \mSigma \, {\vt _{\vlambda }\left (\rvvu \right )} -2\, \vmu ^{\top } {\mSigma } \, \mathbb {E}\vt _{\vlambda }\left (\rvvu \right ) + \vmu ^{\top } {\mSigma } \, \vmu , \nonumber \shortintertext {where \(\mathbb {E}\vt _{\vlambda }\left (\rvvu \right ) = \mC \mathbb {E}{\rvvu } + \vm \), and by \cref {assumption:symmetric_standard},} &\;= \mathbb {E}\, {\vt _{\vlambda }\left (\rvvu \right )}^{\top } \mSigma \, {\vt _{\vlambda }\left (\rvvu \right )} -2\, \vmu ^{\top } {\mSigma } \, \vm + \vmu ^{\top } {\mSigma } \, \vmu .\label {eq:thm:general_quad_reparam_eq1} \end {alignat} Furthermore, \begin {alignat*}{2} &\mathbb {E} {\vt _{\vlambda }\left (\rvvu \right )}^{\top } \mSigma \, {\vt _{\vlambda }\left (\rvvu \right )} \\ &\;= \mathbb {E}{\left (\mC \rvvu + \vm \right )}^{\top } \mSigma \left (\mC \rvvu + \vm \right ) \\ &\;= \mathbb {E} \rvvu ^{\top } \mC ^{\top } \mSigma \, \mC \rvvu + \vm ^{\top } \mSigma \, \mC \, \mathbb {E} \rvvu + \mathbb {E} \rvvu ^{\top } \mC ^{\top } \mSigma \vm ^{\top } + \vm ^{\top } \mSigma \, \vm , \shortintertext {by \cref {assumption:symmetric_standard},} &\;= \mathbb {E} \rvvu ^{\top } \mC ^{\top } {\mSigma } \, \mC \rvvu + \vm ^{\top } \mSigma \, \vm , \shortintertext {invoking the trace trick,} &\;= \mathbb {E} \mathrm {tr}\left ( \rvvu ^{\top } \mC ^{\top } {\mSigma }\, \mC \rvvu \right ) + \vm ^{\top } \mSigma \, \vm , \shortintertext {pusing the expectation into the trace,} &\;= \mathrm {tr}\left (\mathbb {E} \rvvu \rvvu ^{\top } \mC ^{\top } {\mSigma }\, \mC \right ) + \vm ^{\top } \mSigma \, \vm , \shortintertext {invoking \cref {thm:u_identities},} &\;= \mathrm {tr}\left (\mC ^{\top } {\mSigma }\, \mC \right ) + \vm ^{\top } \mSigma \, \vm \\ &\;= \mathrm {tr}\left ({\mSigma } \, \mC \mC ^{\top }\right ) + \vm ^{\top } \mSigma \, \vm . \end {alignat*} Applying this to \cref {eq:thm:general_quad_reparam_eq1}, \begin {alignat*}{2} &\mathbb {E} {\left ( \vt _{\vlambda }\left (\rvvu \right ) - \vmu \right )}^{\top } {\mSigma }^{-1} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu \right ) \\ &\;= \mathrm {tr}\left ({\mSigma }^{-1} \mC \mC ^{\top }\right ) + \vm ^{\top } \mSigma ^{-1} \vm -2\, \vmu ^{\top } {\mSigma }^{-1} \vm + \vmu ^{\top } {\mSigma }^{-1} \vmu \\ &\;= {\left (\vm - \vmu \right )}^{\top } {\mSigma }^{-1} \left (\vm - \vmu \right ) + \mathrm {tr}\left ({\mSigma }^{-1} \mC \mC ^{\top }\right ). \end {alignat*}\end{proof}

\begin{restatable}[]{corollary}{prAtEndRestatexii}\label{thm:prAtEndxii}\label {thm:q_quad_reparam} Let \(\vt _{\vlambda }: \mathbb {R}^d \mapsto \mathbb {R}^d\) be defined as in \cref {def:reparam} with parameters \(\vlambda = \left (\vm , \mC \right )\) such that \(\vm \in \mathbb {R}^d\) and \(\mC \in \mathbb {R}^{d \times d}\). Also, let \(\rvvu \sim \varphi \) be a vector-valued random variable, where \(\varphi \) is defined as in \cref {assumption:symmetric_standard}. Then, \begin {align*} \mathbb {E} \, {\left ( \vt _{\vlambda }\left (\rvvu \right ) - \vm \right )}^{\top } {\left (\mC \mC ^{\top }\right )}^{-1} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right ) = d. \end {align*}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxii}From, \cref {thm:general_quad_reparam} we have \begin {alignat*}{2} &\mathbb {E} \, {\left ( \vt _{\vlambda }\left (\rvvu \right ) - \vm \right )}^{\top } {\left (\mC \mC ^{\top }\right )}^{-1} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right ) \\ &\;= {\left (\vm - \vm \right )}^{\top } {\left (\mC \mC ^{\top }\right )}^{-1} \left (\vm - \vm \right ) + \mathrm {tr}\left ({\left ( \mC \mC ^{\top } \right )}^{-1} \mC \mC ^{\top }\right ) \\ &\;= \mathrm {tr}\left (\mI \right ) \\ &\;= d. \end {alignat*}\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexiii}\label{thm:prAtEndxiii}\label {thm:general_grad_norm_reparam} Let \(\vt _{\vlambda }: \mathbb {R}^d \mapsto \mathbb {R}^d\) be defined as in \cref {def:reparam} with parameters \(\vlambda = \left (\vm , \mC \right )\) such that \(\vm \in \mathbb {R}^d\) and \(\mC \in \mathbb {R}^{d \times d}\). Also, let \(\mSigma _1, \mSigma _2 \in \mathbb {R}^{d \times d}\) be some matrices, \(\vmu _1, \vmu _2 \in \mathbb {R}^{d}\) be some vectors, and \(\rvvu = \left (\rvu _1, \ldots , \rvu _d \right )\) be a vector-valued random variable sampled as \(\rvvu \sim \varphi \), where \(\varphi \) is defined as in \cref {assumption:symmetric_standard} with kurtosis \(\kappa = \mathbb {E}\rvu _i^4\). Then, \begin {alignat*}{2} &\mathbb {E} {\left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu _1\right )}^{\top } \mSigma _1 \mSigma _2 \left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu _2\right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \\ &\;= \left (d + 1\right ) \vmu _1^{\top } \mSigma _1 \mSigma _2 \vmu _2 + \left (d + \kappa \right ) \mathrm {tr}\left (\mC \mC ^{\top } \mSigma _1 \mSigma _2 \right ). \end {alignat*}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxiii}\begin {alignat}{2} &\mathbb {E} {\left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu _1\right )}^{\top } \mSigma _1 \mSigma _2 \left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu _2\right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\;= \mathbb {E} {\vt _{\vlambda }\left (\rvvu \right )}^{\top } \mSigma _1 \mSigma _2 \, \vt _{\vlambda }\left (\rvvu \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\qquad - \vmu _1^{\top } \mSigma _1 \mSigma _2 \, \mathbb {E} \vt _{\vlambda }\left (\rvvu \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\qquad - \mathbb {E} {\left (\vt _{\vlambda }\left (\rvvu \right ) \left ( 1 + \norm {\rvvu }_2^2 \right )\right )}^{\top } \mSigma _1 \mSigma _2 \vmu _1 \nonumber \\ &\qquad + \vmu _1^{\top } \mSigma _1 \mSigma _2 \vmu _2 \, \mathbb {E}\left ( 1 + \norm {\rvvu }_2^2 \right ), \nonumber \shortintertext {invoking \cref {thm:u_identities},} &\;= \mathbb {E} {\vt _{\vlambda }\left (\rvvu \right )}^{\top } \mSigma _1 \mSigma _2 \, \vt _{\vlambda }\left (\rvvu \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\qquad - \mathbb {E}\rvu _i^3 \, \vmu _1^{\top } \mSigma _1 \mSigma _2 \mathbf {1} \nonumber \\ &\qquad - \mathbb {E}\rvu _i^3 \, \mathbf {1}^{\top } \mSigma _1 \mSigma _2 \vmu _1 \nonumber \\ &\qquad + \left ( 1 + d\,\mathbb {E}\rvu _i^2 \right ) \vmu _1^{\top } \mSigma _1 \mSigma _2 \vmu _2, \nonumber \shortintertext {and due to \cref {assumption:symmetric_standard},} &\;= \mathbb {E} {\vt _{\vlambda }\left (\rvvu \right )}^{\top } \mSigma _1 \mSigma _2 \, \vt _{\vlambda }\left (\rvvu \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \label {eq:general_grad_norm reparam_eq1} \\ &\qquad + \left ( 1 + d \right ) \vmu _1^{\top } \mSigma _1 \mSigma _2 \vmu _2.\label {eq:general_grad_norm reparam_eq2} \end {alignat} Now for \cref {eq:general_grad_norm reparam_eq1}, \begin {alignat}{2} &\mathbb {E} {\vt _{\vlambda }\left (\rvvu \right )}^{\top } \mSigma _1 \mSigma _2 \, \vt _{\vlambda }\left (\rvvu \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\;= \mathbb {E} {\left (\mC \rvvu + \vm \right )}^{\top } \mSigma _1 \mSigma _2 \left (\mC \rvvu + \vm \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\;= \mathbb {E} \mathrm {tr}\left ( \rvvu ^{\top } \mC ^{\top } \mSigma _1 \mSigma _2 \mC \rvvu \right ) \nonumber \\ &\qquad + \mathbb {E} \mathrm {tr}\left ( \rvvu ^{\top } \mC ^{\top } \mSigma _1 \mSigma _2 \mC \, \rvvu \rvvu ^{\top } \rvvu \right ) \label {eq:thm:general_grad_norm_reparam_eq1} \\ &\qquad + \vm ^{\top } \mSigma _1 \mSigma _2 \mC \, \mathbb {E} \rvvu \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\qquad + \mathbb {E} \rvvu ^{\top } \left ( 1 + \norm {\rvvu }_2^2 \right ) \mC ^{\top } \mSigma _1 \mSigma _2 \vm \nonumber \\ &\qquad + \vm ^{\top } \mSigma _1 \mSigma _2 \vm \, \mathbb {E} \rvvu \left ( 1 + \norm {\rvvu }_2^2 \right ), \nonumber \shortintertext {using the cyclic property of the trace on \cref {eq:thm:general_grad_norm_reparam_eq1},} &\;= \mathrm {tr}\left ( \mathbb {E} \rvvu \rvvu ^{\top } \mC ^{\top } \mSigma _1 \mSigma _2 \mC \right ) \nonumber \\ &\qquad + \mathrm {tr}\left ( \mC ^{\top } \mSigma _1 \mSigma _2 \mC \, \mathbb {E} \rvvu \rvvu ^{\top } \rvvu \rvvu ^{\top } \right ) \nonumber \\ &\qquad + \vm ^{\top } \mSigma _1 \mSigma _2 \mC \, \mathbb {E} \rvvu \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\qquad + \mathbb {E} \rvvu ^{\top } \left ( 1 + \norm {\rvvu }_2^2 \right ) \mC ^{\top } \mSigma _1 \mSigma _2 \, \vm \nonumber \\ &\qquad + \vm ^{\top } \mSigma _1 \mSigma _2 \vm \, \mathbb {E} \rvvu \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \shortintertext {invoking \cref {thm:u_identities},} &\;= \mathrm {tr}\left ( \left (\mathbb {E}\rvu _i^2\right ) \mI \mC ^{\top } \mSigma _1 \mSigma _2 \mC \right ) \nonumber \\ &\qquad + \mathrm {tr}\left ( \mC ^{\top } \mSigma _1 \mSigma _2 \mC \left (\left (d-1\right ) {\left (\mathbb {E}\rvu _i^2\right )}^2 + \mathbb {E}\rvu _i^4 \right ) \mI \right ) \nonumber \\ &\qquad + \vm ^{\top } \mSigma _1 \mSigma _2 \mC \, \left (\mathbb {E} \rvu _i^3\right ) \mathbf {1} \nonumber \\ &\qquad + \left (\mathbb {E} \rvu _i^3\right ) \mathbf {1}^{\top } \mC ^{\top } \mSigma _1 \mSigma _2 \vm \nonumber \\ &\qquad + \vm ^{\top } \mSigma _1 \mSigma _2 \vm \, \left ( \mathbb {E} \rvu _i^3 \right ) \mathbf {1}, \nonumber \shortintertext {and due to \cref {assumption:symmetric_standard},} &\;= \mathrm {tr}\left ( \mC ^{\top } \mSigma _1 \mSigma _2 \mC \right ) + \left (d - 1 + \kappa \right ) \mathrm {tr}\left ( \mC ^{\top } \mSigma _1 \mSigma _2 \mC \right ) \nonumber \\ &\;= \left (d + \kappa \right ) \mathrm {tr}\left (\mC ^{\top } \mSigma _1 \mSigma _2 \mC \right ) \nonumber \\ &\;= \left (d + \kappa \right ) \mathrm {tr}\left (\mC \mC ^{\top } \mSigma _1 \mSigma _2 \right ). \nonumber \end {alignat} Finally, applying this to \cref {eq:general_grad_norm reparam_eq2}, \begin {alignat*}{2} &\mathbb {E} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu _1\right ) \mSigma _1 \mSigma _2 \left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu _2\right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\;= \left (d + 1\right ) \vmu _1^{\top } \mSigma _1 \mSigma _2 \vmu _2 + \left (d + \kappa \right ) \mathrm {tr}\left (\mC \mC ^{\top } \mSigma _1 \mSigma _2 \right ). \end {alignat*}\end{proof}

\begin{restatable}[]{corollary}{prAtEndRestatexiv}\label{thm:prAtEndxiv}\label {thm:q_grad_norm_reparam} Let \(\vt _{\vlambda }: \mathbb {R}^d \mapsto \mathbb {R}^d\) be defined as in \cref {def:reparam} with parameters \(\vlambda = \left (\vm , \mC \right )\) such that \(\vm \in \mathbb {R}^d\) and \(\mC \in \mathbb {R}^{d \times d}\). Also, let \(\rvvu = \left (\rvu _1, \ldots , \rvu _d \right )\) be a vector-valued random variable sampled as \(\rvvu \sim \varphi \), where \(\varphi \) is defined as in \cref {assumption:symmetric_standard} with kurtosis \(\kappa = \mathbb {E}\rvu _i^4\). Then, \begin {alignat*}{2} &\mathbb {E} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right ) {\left ( \mC \mC ^{\top }\right )}^{-\top } {\left ( \mC \mC ^{\top }\right )}^{-1} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \\ &\;= \left (d + 1\right ) \vm ^{\top } {\left ( \mC \mC ^{\top }\right )}^{-\top } {\left ( \mC \mC ^{\top }\right )}^{-1} \vm + \left (d + \kappa \right ) \mathrm {tr}\left ( {\left ( \mC \mC ^{\top } \right )}^{-1} \right ). \end {alignat*}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxiv}From \cref {thm:general_grad_norm_reparam}, we have \begin {alignat}{2} &\mathbb {E} {\left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right )}^{\top } {\left ( \mC \mC ^{\top }\right )}^{-\top } {\left ( \mC \mC ^{\top }\right )}^{-1} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\;= \left (d + 1\right ) \vm ^{\top } {\left ( \mC \mC ^{\top }\right )}^{-\top } {\left ( \mC \mC ^{\top }\right )}^{-1} \vm \nonumber \\ &\quad + \left (d + \kappa \right ) \mathrm {tr}\left (\mC \mC ^{\top } {\left ( \mC \mC ^{\top }\right )}^{-\top } {\left ( \mC \mC ^{\top }\right )}^{-1}\right ).\label {thm:q_grad_norm_reparam_eq1} \end {alignat} Since, by the basic properties of the trace, \begin {alignat*}{2} \mathrm {tr}\left (\mC \mC ^{\top } {\left ( \mC \mC ^{\top }\right )}^{-\top } {\left ( \mC \mC ^{\top }\right )}^{-1}\right ) &= \mathrm {tr}\left ( {\left ( \mC \mC ^{\top }\right )}^{-1} \mC \mC ^{\top } {\left ( \mC \mC ^{\top }\right )}^{-\top } \right ) \\ &= \mathrm {tr}\left ( \mI \, {\left ( \mC \mC ^{\top }\right )}^{-\top } \right ) \\ &= \mathrm {tr}\left ( {\left ( \mC \mC ^{\top }\right )}^{-\top } \right ) \\ &= \mathrm {tr}\left ( {\left ( \mC \mC ^{\top } \right )}^{-1} \right ), \end {alignat*} \cref {thm:q_grad_norm_reparam_eq1} becomes \begin {alignat*}{2} &\mathbb {E} {\left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right )}^{\top } {\left ( \mC \mC ^{\top }\right )}^{-\top } {\left ( \mC \mC ^{\top }\right )}^{-1} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \\ &\;= \left (d + 1\right ) \vm ^{\top } {\left ( \mC \mC ^{\top }\right )}^{-\top } {\left ( \mC \mC ^{\top }\right )}^{-1} \vm + \left (d + \kappa \right ) \mathrm {tr}\left ( {\left ( \mC \mC ^{\top } \right )}^{-1} \right ). \end {alignat*}\end{proof}

\prAtEndRestatexv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxv}\par The STL estimator is obtained by setting \begin {alignat*}{2} f\left ( \vz \right ) = -\log p\left (\vz , \vx \right ) + \log q_{\vgamma }\left ( \vz \right ) \lvert _{\vgamma = \vlambda }. \end {alignat*} We first consider the log joint likelihood of the model to be \begin {alignat*}{2} \log p\left (\vz , \vx \right ) = -\frac {1}{2} {\left (\vz - \vmu \right )}^{-1} \mSigma ^{-1} \left (\vz - \vmu \right ), \end {alignat*} which is the unnormalized log probability density of a multivariate normal distribution with mean \(\vmu \) and covariance \(\mSigma \). We also set the variational family to be multivariate normal with mean (location) \(\vm \) and covariance (scale) \(\mC \mC ^{\top }\). Given these, the objective function is \begin {alignat*}{2} F\left (\vlambda \right ) &= \mathbb {E} f\left (\vt _{\vlambda }\left (\rvvu \right )\right ) \\ &= \mathbb {E}\log p\left (\vt _{\vlambda }\left (\rvvu \right )\right ) - \mathbb {E}\log q_{\vgamma }\left (\vt _{\vlambda }\left (\rvvu \right )\right ) \big \lvert _{\vgamma = \vlambda } \end {alignat*} \par From~\cref {thm:general_quad_reparam}, the likelihood term is \begin {alignat*}{2} &\mathbb {E}\log p\left (\vt _{\vlambda }\left (\rvvu \right )\right ) \\ &\;= -\frac {1}{2} {\left (\vm - \vmu \right )}^{\top } \mSigma ^{-1} \left (\vm - \vmu \right ) - \frac {1}{2} \mathrm {tr}\left (\mSigma ^{-1} \mC \mC ^{\top } \right ), \end {alignat*} while from~\cref {thm:q_quad_reparam}, the entropy term is \begin {alignat*}{2} &\mathbb {E}\log q_{\vlambda }\left (\vt _{\vlambda }\left (\rvvu \right )\right ) \\ &\;= -\frac {1}{2} \mathbb {E} {\left ( \vt _{\vlambda }\left (\rvvu \right ) - \vm \right )}^{\top } \mS ^{-1} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right ) - \frac {1}{2}\log \abs {\mS } + Z, \\ &\;= -\frac {1}{2} d - \frac {1}{2}\log \abs {\mS } + Z, \end {alignat*} where, \(\mS = \mC \mC ^{\top }\) and \(Z\) is a constant independent of \(\vm \) and \(\mC \). The derivative of the \(f\) is given as \begin {alignat}{2} &\nabla f\left (\vt _{\vlambda }\left (\vu \right )\right ) \nonumber \\ &\;= -\nabla \log p\left (\vt _{\vlambda }\left (\vu \right )\right ) + \nabla \log q_{\vgamma }\left (\vt _{\vlambda }\left (\vu \right )\right ) \lvert _{\vgamma = \vlambda } \nonumber \\ &\;= \mSigma ^{-1} \left (\vt _{\vlambda }\left (\vu \right ) - \vmu \right ) - {\mS }^{-1} \left ( \vt _{\vgamma }\left (\vu \right ) - \vm \right ) \lvert _{\vgamma = \vlambda }.\label {eq:gradient_lower_bound_f_derivative} \end {alignat} \par Given \cref {thm:sample_mean_estimator}, the second moment of the \(M\)-sample gradient can be decomposed as \begin {alignat*}{2} \mathbb {E} \norm {\vg \left (\vlambda \right )}_2^2 = \frac {1}{M} \mathbb {E} \norm { \nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\rvvu \right ) \right ) }_2^2 + \frac {M-1}{M} \norm { \nabla F\left (\vlambda \right ) }_2^2 \end {alignat*} \par We now compute the expectation of the squared gradient norm. First, by starting from \cref {thm:variational_gradient_norm_identity}, \begin {alignat}{2} &\mathbb {E}\norm { \nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\rvvu \right ) \right ) }_2^2 \nonumber \\ &\;= \mathbb {E} \norm { \nabla f\left ( \vt _{\vlambda }\left (\rvvu \right ) \right ) }_2^2 \left ( 1 + \norm {\rvvu }_2^2 \right ), \nonumber \shortintertext {plugging in \cref {eq:gradient_lower_bound_f_derivative},} &\;= \mathbb {E} \norm {\, \mSigma ^{-1} \left (\vt _{\vlambda }\left (\vu \right ) - \vmu \right ) - {\mS }^{-1} \left ( \vt _{\vlambda }\left (\vu \right ) - \vm \right )\,}^2_2 \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\;= \mathbb {E} {\left (\vt _{\vlambda }\left (\vu \right ) - \vmu \right )}^{\top } \mSigma ^{-\top } \mSigma ^{-1} \left (\vt _{\vlambda }\left (\vu \right ) - \vmu \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\qquad - 2\,\mathbb {E} {\left (\vt _{\vlambda }\left (\vu \right ) - \vmu \right )}^{\top } \mSigma ^{-\top } \mS ^{-1} \left (\vt _{\vlambda }\left (\vu \right ) - \vm \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\qquad + \mathbb {E} {\left (\vt _{\vlambda }\left (\vu \right ) - \vm \right )}^{\top } \mS ^{-\top } \mS ^{-1} \left (\vt _{\vlambda }\left (\vu \right ) - \vm \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ), \nonumber \shortintertext {applying \cref {thm:general_grad_norm_reparam},} &\;= \left (d+1\right ) \vmu ^{\top } \mSigma ^{-\top } \mSigma ^{-1} \vmu + \left (d+\kappa \right ) \mathrm {tr}\left (\mS \mSigma ^{-\top } \mSigma ^{-1}\right ) \nonumber \\ &\qquad - 2 \, \left (d+1\right ) \vmu ^{\top } \mSigma ^{-\top } \mS ^{-1} \vm - 2\,\left (d+\kappa \right ) \mathrm {tr}\left (\mS \mSigma ^{-\top } \mS ^{-1}\right ) \nonumber \\ &\qquad + \left (d+1\right ) \vm ^{\top } \mS ^{-\top } \mS ^{-1} \vm + \left (d+\kappa \right ) \mathrm {tr}\left (\mS ^{-1}\right ), \nonumber \\ \shortintertext {and after regroupping the terms,} &\;= \left (d+1\right ) \left ( \vmu ^{\top } \mSigma ^{-\top } \mSigma ^{-1} \vmu - 2 \vmu ^{\top } \mSigma ^{-\top } \mS ^{-1} \vm + \vm ^{\top } \mS ^{-\top } \mS ^{-1} \vm \right ) \nonumber \\ &\qquad + \left (d+\kappa \right ) \left ( \mathrm {tr}\left (\mS \mSigma ^{-\top } \mSigma ^{-1}\right ) -2 \mathrm {tr}\left (\mS \mSigma ^{-\top } \mS ^{-1}\right ) + \mathrm {tr}\left (\mS ^{-1}\right ) \right ). \nonumber \end {alignat} This expression itself is not very convenient to work with due to the inner product term of \(\vmu \) and \(\vm \). Thus, we focus on the special case \(\vmu = \mathbf {0}\). Then, \begin {alignat}{2} &\mathbb {E}\norm { \nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\rvvu \right ) \right ) }_2^2 \nonumber \\ &\;= \left (d+1\right )\vm ^{\top } \mS ^{-\top } \mS ^{-1} \vm \nonumber \\ &\quad + \left (d+\kappa \right ) \left ( \mathrm {tr}\left (\mS \mSigma ^{-\top } \mSigma ^{-1}\right ) -2 \, \mathrm {tr}\left (\mSigma ^{-\top }\right ) + \mathrm {tr}\left (\mS ^{-1}\right ) \right ) \nonumber \\ &\;= \left (d+1\right )\vm ^{\top } \mS ^{-\top } \mS ^{-1} \vm \nonumber \\ &\quad + \left (d+\kappa \right ) \left ( \mathrm {tr}\left (\mS \mSigma ^{-\top } \mSigma ^{-1}\right ) + \mathrm {tr}\left (\mS ^{-1}\right ) \right ) \nonumber \\ &\quad - \underbrace { 2 \left (d+\kappa \right ) \mathrm {tr}\left (\mSigma ^{-\top }\right ) }_{\text {constant with respect to \(\vlambda \)}} \end {alignat} This also simplifies the suboptimality gap as \begin {alignat}{2} & F\left (\vlambda \right ) - F\left (\vlambda ^{*}\right ) \nonumber \\ &\;= \frac {1}{2} \vm ^{\top } \mSigma ^{-1} \vm + \frac {1}{2} \left ( \mathrm {tr}\left (\mSigma ^{-1} \mS \right ) + \mathrm {tr}\left (\mSigma ^{-1} \mS ^* \right ) \right ) \nonumber \\ &\qquad + \frac {1}{2} \left ( -\log \abs {\mS } + \log \abs {\mS ^*} \right ). \nonumber \\ &\;= \frac {1}{2} \vm ^{\top } \mSigma ^{-1} \vm + \frac {1}{2} \left ( \mathrm {tr}\left (\mSigma ^{-1} \mS \right ) - \log \abs {\mS } \right ) \nonumber \\ &\qquad - \underbrace {\frac {1}{2} \,\left (\mathrm {tr}\left (\mSigma ^{-1} \mS ^* \right ) - \log \abs {\mS ^*}\right )}_{\text {constant with respect to \(\vlambda \)}}. \nonumber \end {alignat} \par Showing \begin {alignat}{2} &\vm ^{\top } \mS ^{-\top } \mS ^{-1} \vm \; &&\succeq \; \vm ^{\top } \mSigma ^{-1} \vm \\ &\mathrm {tr}\left (\mS \mSigma ^{-\top } \mSigma ^{-1}\right ) \; &&\succeq \; \mathrm {tr}\left (\mSigma ^{-1} \mS \right ) \\ &\mathrm {tr}\left (\mS ^{-1}\right ) \; &&\succeq \; -\log \abs {\mS } \end {alignat}for proves the statement.\end{proof}


==> main-pratendlowerboundlemma.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatexiii}\label{thm:prAtEndxiii}Let \(\vt _{\vlambda }: \mathbb {R}^d \mapsto \mathbb {R}^d\) be defined as in \cref {def:reparam} with parameters \(\vlambda = \left (\vm , \mC \right )\) such that \(\vm \in \mathbb {R}^d\) and \(\mC \in \mathbb {R}^{d \times d}\). Also, let \(\rvvu \sim \varphi \), where \(\varphi \) is defined as in \cref {assumption:symmetric_standard}. Then, \begin {alignat*}{2} \mathbb {E}\vt _{\vlambda }\left (\rvvu \right ) \left (1 + \norm {\rvvu }_2^2\right ) = \left (d + 1\right ) \vm . \end {alignat*}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxiii}Since \(\rvu _i\) follows a symmetric and standardized distribution, \(\mathbb {E}\rvu _i^3 = 0, \mathbb {E} \rvu _i^2 = 1\). Then, \begin {alignat*}{2} \mathbb {E}\vt _{\vlambda }\left (\rvvu \right ) \left (1 + \norm {\rvvu }_2^2\right ) &= \mathbb {E} \left (\mC \rvvu + \vm \right ) \left (1 + \norm {\rvvu }_2^2\right ) \\ &= \mC \, \mathbb {E} \rvvu \left (1 + \norm {\rvvu }_2^2\right ) + \vm \left (1 + \mathbb {E} \norm {\rvvu }_2^2\right ), \shortintertext {applying \cref {thm:u_identities},} &= \left ( \mathbb {E}\rvu _i^3 \right ) \mC \mathbf {1} + \vm \left (1 + d \, \mathbb {E} \rvu _i^2\right ), \shortintertext {and by~\cref {assumption:symmetric_standard},} &= \left (d + 1\right ) \vm . \end {alignat*}\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexiv}\label{thm:prAtEndxiv}\label {thm:general_quad_reparam} Let \(\vt _{\vlambda }: \mathbb {R}^d \mapsto \mathbb {R}^d\) be defined as in \cref {def:reparam} with parameters \(\vlambda = \left (\vm , \mC \right )\) such that \(\vm \in \mathbb {R}^d\) and \(\mC \in \mathbb {R}^{d \times d}\). Also, let \(\mSigma \in \mathbb {R}^{d \times d}\) be some matrix, \(\vmu \in \mathbb {R}^d\) be some vector, and \(\rvvu \sim \varphi \) be a vector-valued random variable, where \(\varphi \) is defined as in \cref {assumption:symmetric_standard}. Then, \begin {align*} &\mathbb {E} \, {\left ( \vt _{\vlambda }\left (\rvvu \right ) - \vmu \right )}^{\top } \mSigma \left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu \right ) \\ &\;= {\left (\vm - \vmu \right )}^{\top } \mSigma \left (\vm - \vmu \right ) + \mathrm {tr}\left ({\mSigma }^{-1} \mC \mC ^{\top }\right ). \end {align*}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxiv}\begin {alignat}{2} &\mathbb {E} {\left ( \vt _{\vlambda }\left (\rvvu \right ) - \vmu \right )}^{\top } \mSigma \, \left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu \right ) \nonumber \\ &\;= \mathbb {E}\, {\vt _{\vlambda }\left (\rvvu \right )}^{\top } \mSigma \, {\vt _{\vlambda }\left (\rvvu \right )} -2\, \vmu ^{\top } {\mSigma } \, \mathbb {E}\vt _{\vlambda }\left (\rvvu \right ) + \vmu ^{\top } {\mSigma } \, \vmu , \nonumber \shortintertext {where \(\mathbb {E}\vt _{\vlambda }\left (\rvvu \right ) = \mC \mathbb {E}{\rvvu } + \vm \), and by \cref {assumption:symmetric_standard},} &\;= \mathbb {E}\, {\vt _{\vlambda }\left (\rvvu \right )}^{\top } \mSigma \, {\vt _{\vlambda }\left (\rvvu \right )} -2\, \vmu ^{\top } {\mSigma } \, \vm + \vmu ^{\top } {\mSigma } \, \vmu .\label {eq:thm:general_quad_reparam_eq1} \end {alignat} Furthermore, \begin {alignat*}{2} &\mathbb {E} {\vt _{\vlambda }\left (\rvvu \right )}^{\top } \mSigma \, {\vt _{\vlambda }\left (\rvvu \right )} \\ &\;= \mathbb {E}{\left (\mC \rvvu + \vm \right )}^{\top } \mSigma \left (\mC \rvvu + \vm \right ) \\ &\;= \mathbb {E} \rvvu ^{\top } \mC ^{\top } \mSigma \, \mC \rvvu + \vm ^{\top } \mSigma \, \mC \, \mathbb {E} \rvvu + \mathbb {E} \rvvu ^{\top } \mC ^{\top } \mSigma \vm ^{\top } + \vm ^{\top } \mSigma \, \vm , \shortintertext {by \cref {assumption:symmetric_standard},} &\;= \mathbb {E} \rvvu ^{\top } \mC ^{\top } {\mSigma } \, \mC \rvvu + \vm ^{\top } \mSigma \, \vm , \shortintertext {invoking the trace trick,} &\;= \mathbb {E} \mathrm {tr}\left ( \rvvu ^{\top } \mC ^{\top } {\mSigma }\, \mC \rvvu \right ) + \vm ^{\top } \mSigma \, \vm , \shortintertext {pusing the expectation into the trace,} &\;= \mathrm {tr}\left (\mathbb {E} \rvvu \rvvu ^{\top } \mC ^{\top } {\mSigma }\, \mC \right ) + \vm ^{\top } \mSigma \, \vm , \shortintertext {invoking \cref {thm:u_identities},} &\;= \mathrm {tr}\left (\mC ^{\top } {\mSigma }\, \mC \right ) + \vm ^{\top } \mSigma \, \vm \\ &\;= \mathrm {tr}\left ({\mSigma } \, \mC \mC ^{\top }\right ) + \vm ^{\top } \mSigma \, \vm . \end {alignat*} Applying this to \cref {eq:thm:general_quad_reparam_eq1}, \begin {alignat*}{2} &\mathbb {E} {\left ( \vt _{\vlambda }\left (\rvvu \right ) - \vmu \right )}^{\top } {\mSigma }^{-1} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu \right ) \\ &\;= \mathrm {tr}\left ({\mSigma }^{-1} \mC \mC ^{\top }\right ) + \vm ^{\top } \mSigma ^{-1} \vm -2\, \vmu ^{\top } {\mSigma }^{-1} \vm + \vmu ^{\top } {\mSigma }^{-1} \vmu \\ &\;= {\left (\vm - \vmu \right )}^{\top } {\mSigma }^{-1} \left (\vm - \vmu \right ) + \mathrm {tr}\left ({\mSigma }^{-1} \mC \mC ^{\top }\right ). \end {alignat*}\end{proof}

\begin{restatable}[]{corollary}{prAtEndRestatexv}\label{thm:prAtEndxv}\label {thm:q_quad_reparam} Let \(\vt _{\vlambda }: \mathbb {R}^d \mapsto \mathbb {R}^d\) be defined as in \cref {def:reparam} with parameters \(\vlambda = \left (\vm , \mC \right )\) such that \(\vm \in \mathbb {R}^d\) and \(\mC \in \mathbb {R}^{d \times d}\). Also, let \(\rvvu \sim \varphi \) be a vector-valued random variable, where \(\varphi \) is defined as in \cref {assumption:symmetric_standard}. Then, \begin {align*} \mathbb {E} \, {\left ( \vt _{\vlambda }\left (\rvvu \right ) - \vm \right )}^{\top } {\left (\mC \mC ^{\top }\right )}^{-1} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right ) = d. \end {align*}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxv}From, \cref {thm:general_quad_reparam} we have \begin {alignat*}{2} &\mathbb {E} \, {\left ( \vt _{\vlambda }\left (\rvvu \right ) - \vm \right )}^{\top } {\left (\mC \mC ^{\top }\right )}^{-1} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right ) \\ &\;= {\left (\vm - \vm \right )}^{\top } {\left (\mC \mC ^{\top }\right )}^{-1} \left (\vm - \vm \right ) + \mathrm {tr}\left ({\left ( \mC \mC ^{\top } \right )}^{-1} \mC \mC ^{\top }\right ) \\ &\;= \mathrm {tr}\left (\mI \right ) \\ &\;= d. \end {alignat*}\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexvi}\label{thm:prAtEndxvi}\label {thm:general_grad_norm_reparam} Let \(\vt _{\vlambda }: \mathbb {R}^d \mapsto \mathbb {R}^d\) be defined as in \cref {def:reparam} with parameters \(\vlambda = \left (\vm , \mC \right )\) such that \(\vm \in \mathbb {R}^d\) and \(\mC \in \mathbb {R}^{d \times d}\). Also, let \(\mSigma _1, \mSigma _2 \in \mathbb {R}^{d \times d}\) be some matrices, \(\vmu _1, \vmu _2 \in \mathbb {R}^{d}\) be some vectors, and \(\rvvu = \left (\rvu _1, \ldots , \rvu _d \right )\) be a vector-valued random variable sampled as \(\rvvu \sim \varphi \), where \(\varphi \) is defined as in \cref {assumption:symmetric_standard} with kurtosis \(\kappa = \mathbb {E}\rvu _i^4\). Then, \begin {alignat*}{2} &\mathbb {E} {\left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu _1\right )}^{\top } \mSigma _1 \mSigma _2 \left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu _2\right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \\ &\;= \left (d + 1\right ) \vmu _1^{\top } \mSigma _1 \mSigma _2 \vmu _2 + \left (d + \kappa \right ) \mathrm {tr}\left (\mC \mC ^{\top } \mSigma _1 \mSigma _2 \right ). \end {alignat*}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxvi}\begin {alignat}{2} &\mathbb {E} {\left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu _1\right )}^{\top } \mSigma _1 \mSigma _2 \left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu _2\right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\;= \mathbb {E} {\vt _{\vlambda }\left (\rvvu \right )}^{\top } \mSigma _1 \mSigma _2 \, \vt _{\vlambda }\left (\rvvu \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\qquad - \vmu _1^{\top } \mSigma _1 \mSigma _2 \, \mathbb {E} \vt _{\vlambda }\left (\rvvu \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\qquad - \mathbb {E} {\left (\vt _{\vlambda }\left (\rvvu \right ) \left ( 1 + \norm {\rvvu }_2^2 \right )\right )}^{\top } \mSigma _1 \mSigma _2 \vmu _1 \nonumber \\ &\qquad + \vmu _1^{\top } \mSigma _1 \mSigma _2 \vmu _2 \, \mathbb {E}\left ( 1 + \norm {\rvvu }_2^2 \right ), \nonumber \shortintertext {invoking \cref {thm:u_identities},} &\;= \mathbb {E} {\vt _{\vlambda }\left (\rvvu \right )}^{\top } \mSigma _1 \mSigma _2 \, \vt _{\vlambda }\left (\rvvu \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\qquad - \mathbb {E}\rvu _i^3 \, \vmu _1^{\top } \mSigma _1 \mSigma _2 \mathbf {1} \nonumber \\ &\qquad - \mathbb {E}\rvu _i^3 \, \mathbf {1}^{\top } \mSigma _1 \mSigma _2 \vmu _1 \nonumber \\ &\qquad + \left ( 1 + d\,\mathbb {E}\rvu _i^2 \right ) \vmu _1^{\top } \mSigma _1 \mSigma _2 \vmu _2, \nonumber \shortintertext {and due to \cref {assumption:symmetric_standard},} &\;= \mathbb {E} {\vt _{\vlambda }\left (\rvvu \right )}^{\top } \mSigma _1 \mSigma _2 \, \vt _{\vlambda }\left (\rvvu \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \label {eq:general_grad_norm reparam_eq1} \\ &\qquad + \left ( 1 + d \right ) \vmu _1^{\top } \mSigma _1 \mSigma _2 \vmu _2.\label {eq:general_grad_norm reparam_eq2} \end {alignat} Now for \cref {eq:general_grad_norm reparam_eq1}, \begin {alignat}{2} &\mathbb {E} {\vt _{\vlambda }\left (\rvvu \right )}^{\top } \mSigma _1 \mSigma _2 \, \vt _{\vlambda }\left (\rvvu \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\;= \mathbb {E} {\left (\mC \rvvu + \vm \right )}^{\top } \mSigma _1 \mSigma _2 \left (\mC \rvvu + \vm \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\;= \mathbb {E} \mathrm {tr}\left ( \rvvu ^{\top } \mC ^{\top } \mSigma _1 \mSigma _2 \mC \rvvu \right ) \nonumber \\ &\qquad + \mathbb {E} \mathrm {tr}\left ( \rvvu ^{\top } \mC ^{\top } \mSigma _1 \mSigma _2 \mC \, \rvvu \rvvu ^{\top } \rvvu \right ) \label {eq:thm:general_grad_norm_reparam_eq1} \\ &\qquad + \vm ^{\top } \mSigma _1 \mSigma _2 \mC \, \mathbb {E} \rvvu \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\qquad + \mathbb {E} \rvvu ^{\top } \left ( 1 + \norm {\rvvu }_2^2 \right ) \mC ^{\top } \mSigma _1 \mSigma _2 \vm \nonumber \\ &\qquad + \vm ^{\top } \mSigma _1 \mSigma _2 \vm \, \mathbb {E} \rvvu \left ( 1 + \norm {\rvvu }_2^2 \right ), \nonumber \shortintertext {using the cyclic property of the trace on \cref {eq:thm:general_grad_norm_reparam_eq1},} &\;= \mathrm {tr}\left ( \mathbb {E} \rvvu \rvvu ^{\top } \mC ^{\top } \mSigma _1 \mSigma _2 \mC \right ) \nonumber \\ &\qquad + \mathrm {tr}\left ( \mC ^{\top } \mSigma _1 \mSigma _2 \mC \, \mathbb {E} \rvvu \rvvu ^{\top } \rvvu \rvvu ^{\top } \right ) \nonumber \\ &\qquad + \vm ^{\top } \mSigma _1 \mSigma _2 \mC \, \mathbb {E} \rvvu \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\qquad + \mathbb {E} \rvvu ^{\top } \left ( 1 + \norm {\rvvu }_2^2 \right ) \mC ^{\top } \mSigma _1 \mSigma _2 \, \vm \nonumber \\ &\qquad + \vm ^{\top } \mSigma _1 \mSigma _2 \vm \, \mathbb {E} \rvvu \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \shortintertext {invoking \cref {thm:u_identities},} &\;= \mathrm {tr}\left ( \left (\mathbb {E}\rvu _i^2\right ) \mI \mC ^{\top } \mSigma _1 \mSigma _2 \mC \right ) \nonumber \\ &\qquad + \mathrm {tr}\left ( \mC ^{\top } \mSigma _1 \mSigma _2 \mC \left (\left (d-1\right ) {\left (\mathbb {E}\rvu _i^2\right )}^2 + \mathbb {E}\rvu _i^4 \right ) \mI \right ) \nonumber \\ &\qquad + \vm ^{\top } \mSigma _1 \mSigma _2 \mC \, \left (\mathbb {E} \rvu _i^3\right ) \mathbf {1} \nonumber \\ &\qquad + \left (\mathbb {E} \rvu _i^3\right ) \mathbf {1}^{\top } \mC ^{\top } \mSigma _1 \mSigma _2 \vm \nonumber \\ &\qquad + \vm ^{\top } \mSigma _1 \mSigma _2 \vm \, \left ( \mathbb {E} \rvu _i^3 \right ) \mathbf {1}, \nonumber \shortintertext {and due to \cref {assumption:symmetric_standard},} &\;= \mathrm {tr}\left ( \mC ^{\top } \mSigma _1 \mSigma _2 \mC \right ) + \left (d - 1 + \kappa \right ) \mathrm {tr}\left ( \mC ^{\top } \mSigma _1 \mSigma _2 \mC \right ) \nonumber \\ &\;= \left (d + \kappa \right ) \mathrm {tr}\left (\mC ^{\top } \mSigma _1 \mSigma _2 \mC \right ) \nonumber \\ &\;= \left (d + \kappa \right ) \mathrm {tr}\left (\mC \mC ^{\top } \mSigma _1 \mSigma _2 \right ). \nonumber \end {alignat} Finally, applying this to \cref {eq:general_grad_norm reparam_eq2}, \begin {alignat*}{2} &\mathbb {E} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu _1\right ) \mSigma _1 \mSigma _2 \left (\vt _{\vlambda }\left (\rvvu \right ) - \vmu _2\right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\;= \left (d + 1\right ) \vmu _1^{\top } \mSigma _1 \mSigma _2 \vmu _2 + \left (d + \kappa \right ) \mathrm {tr}\left (\mC \mC ^{\top } \mSigma _1 \mSigma _2 \right ). \end {alignat*}\end{proof}

\begin{restatable}[]{corollary}{prAtEndRestatexvii}\label{thm:prAtEndxvii}\label {thm:q_grad_norm_reparam} Let \(\vt _{\vlambda }: \mathbb {R}^d \mapsto \mathbb {R}^d\) be defined as in \cref {def:reparam} with parameters \(\vlambda = \left (\vm , \mC \right )\) such that \(\vm \in \mathbb {R}^d\) and \(\mC \in \mathbb {R}^{d \times d}\). Also, let \(\rvvu = \left (\rvu _1, \ldots , \rvu _d \right )\) be a vector-valued random variable sampled as \(\rvvu \sim \varphi \), where \(\varphi \) is defined as in \cref {assumption:symmetric_standard} with kurtosis \(\kappa = \mathbb {E}\rvu _i^4\). Then, \begin {alignat*}{2} &\mathbb {E} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right ) {\left ( \mC \mC ^{\top }\right )}^{-\top } {\left ( \mC \mC ^{\top }\right )}^{-1} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \\ &\;= \left (d + 1\right ) \vm ^{\top } {\left ( \mC \mC ^{\top }\right )}^{-\top } {\left ( \mC \mC ^{\top }\right )}^{-1} \vm + \left (d + \kappa \right ) \mathrm {tr}\left ( {\left ( \mC \mC ^{\top } \right )}^{-1} \right ). \end {alignat*}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxvii}From \cref {thm:general_grad_norm_reparam}, we have \begin {alignat}{2} &\mathbb {E} {\left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right )}^{\top } {\left ( \mC \mC ^{\top }\right )}^{-\top } {\left ( \mC \mC ^{\top }\right )}^{-1} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \nonumber \\ &\;= \left (d + 1\right ) \vm ^{\top } {\left ( \mC \mC ^{\top }\right )}^{-\top } {\left ( \mC \mC ^{\top }\right )}^{-1} \vm \nonumber \\ &\quad + \left (d + \kappa \right ) \mathrm {tr}\left (\mC \mC ^{\top } {\left ( \mC \mC ^{\top }\right )}^{-\top } {\left ( \mC \mC ^{\top }\right )}^{-1}\right ).\label {thm:q_grad_norm_reparam_eq1} \end {alignat} Since, by the basic properties of the trace, \begin {alignat*}{2} \mathrm {tr}\left (\mC \mC ^{\top } {\left ( \mC \mC ^{\top }\right )}^{-\top } {\left ( \mC \mC ^{\top }\right )}^{-1}\right ) &= \mathrm {tr}\left ( {\left ( \mC \mC ^{\top }\right )}^{-1} \mC \mC ^{\top } {\left ( \mC \mC ^{\top }\right )}^{-\top } \right ) \\ &= \mathrm {tr}\left ( \mI \, {\left ( \mC \mC ^{\top }\right )}^{-\top } \right ) \\ &= \mathrm {tr}\left ( {\left ( \mC \mC ^{\top }\right )}^{-\top } \right ) \\ &= \mathrm {tr}\left ( {\left ( \mC \mC ^{\top } \right )}^{-1} \right ), \end {alignat*} \cref {thm:q_grad_norm_reparam_eq1} becomes \begin {alignat*}{2} &\mathbb {E} {\left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right )}^{\top } {\left ( \mC \mC ^{\top }\right )}^{-\top } {\left ( \mC \mC ^{\top }\right )}^{-1} \left (\vt _{\vlambda }\left (\rvvu \right ) - \vm \right ) \left ( 1 + \norm {\rvvu }_2^2 \right ) \\ &\;= \left (d + 1\right ) \vm ^{\top } {\left ( \mC \mC ^{\top }\right )}^{-\top } {\left ( \mC \mC ^{\top }\right )}^{-1} \vm + \left (d + \kappa \right ) \mathrm {tr}\left ( {\left ( \mC \mC ^{\top } \right )}^{-1} \right ). \end {alignat*}\end{proof}


==> main-pratendlowerboundtheorem.tex <==


\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndx}When using the matrix square root parameterization,~\citet {domke_provable_2020} have shown that if $f$ is $L$-smooth, $\mathbb {E} f\left (\vt _{\vlambda }\left (\rvvu \right )\right )$ is also $L$-smooth. Therefore, we have \begin {align} \norm {\mathbb {E}{ \nabla _{\vlambda } f\left (\vt _{\vlambda }\left (\rvvu \right )\right )} }_2^2 \leq 2 L \left (\mathbb {E} f\left (\vt _{\vlambda }\left (\rvvu \right )\right ) - f^*\right ). \label {eq:thm_lower_bound_eq1} \end {align} \par Furthermore, let $\bar {\vzeta }$ be the minimizer of $f$, namely $f^* = f\left (\bar {\vzeta }\right )$. From \cref {thm:variational_gradient_norm_identity}, we have \begin {align*} \mathbb {E}{\norm {\nabla _{\vlambda } f\left (\vt _{\vlambda }\left (\rvvu \right )\right )}_2^2} & = \mathbb {E}{\norm {\nabla f\left (\vt _{\vlambda }\left (\rvvu \right )\right )}_2^2 \left (1 + \norm {\rvvu }_2^2\right )}, \shortintertext {by the \(\mu \)-strong convexity of \(f\),} & \geq 2 \mu \, \mathbb {E}{\left (f\left (\vt _{\vlambda }\left (\rvvu \right )\right ) - f^*\right ) \left (1 + \norm {\rvvu }_2^2\right )} \\ & \geq \mu ^2 \, \mathbb {E}{{\lVert \vt _{\vlambda }\left (\rvvu \right ) - \bar {\vzeta }\rVert }^2_2 \left (1 + \norm {\rvvu }_2^2\right )}, \shortintertext {applying \Cref {thm:reparam_u_identity},} & = \mu ^2 \, \left (\left (d + 1\right ) {\lVert \vm - \bar {\vzeta } \rVert }^2_2 + \left (d + \kappa \right ) \norm {\mC }_{\mathrm {F}}^2\right ), \shortintertext {and by the property of the kurtosis that \(\kappa \geq 1\),} & \geq \mu ^2 \, \left (d + 1\right ) {\lVert \vlambda - \bar {\vlambda } \rVert }^2_2, \end {align*} where $\bar {\vlambda } = \left (\bar {\vzeta }, \boldupright {O}\right )$. \par Observe that $\bar {\vlambda }$ is the minimizer of $\mathbb {E}{f\left (\vt _{\vlambda }\left (\rvvu \right )\right )}$ such that \[ \mathbb {E}{f\left (\vt _{\bar {\vlambda }}\left (\rvvu \right )\right )} = f\left (\bar {\vzeta }\right ) = f^* \leq \mathbb {E}{f\left (\vt _{\vlambda }\left (\rvvu \right )\right )} \] for any $\vlambda $. Furthermore, from the $L$-smoothness of $\mathbb {E}{f\left (\vt _{\vlambda }\left (\rvvu \right )\right )}$, we have \begin {align*} &\mu ^2 \left (d + 1\right ) {\lVert \vlambda - \bar {\vlambda } \rVert }^2_2 \\ &\quad \geq \frac {2 \mu ^2 \left (d + 1\right )}{L} \left (\mathbb {E}{f\left (\vt _{\vlambda }\left (\rvvu \right )\right )} - \mathbb {E}{f\left (\vt _{\bar {\vlambda }}\left (\rvvu \right )\right )}\right ). \end {align*} Thus, we have \begin {align} \mathbb {E}{\norm {\nabla _{\vlambda } f\left (\vt _{\vlambda }\left (\rvvu \right )\right )}_2^2} &\geq \frac {2 \mu ^2 \left (d + 1\right )}{L} \left (\mathbb {E}{f\left (\vt _{\vlambda }\left (\rvvu \right )\right )} - f^*\right ). \label {eq:thm_lower_bound_eq2} \end {align} \par Now, from \cref {eq:thm_gradient_variance_general_definition}, \begin {align*} \mathbb {E}\norm { \vg _M }_2^2 &= \frac {1}{M} \left ( \mathbb {E}{ \norm {\nabla _{\vlambda } f\left (\vt _{\vlambda }\left (\rvvu \right )\right )}_2^2 } - \norm {\mathbb {E}{ \nabla _{\vlambda } f\left (\vt _{\vlambda }\left (\rvvu \right )\right )} }_2^2 \right ) \\ &\qquad + \norm { \nabla F\left (\vlambda \right ) }^2_2, \shortintertext {applying \cref {eq:thm_lower_bound_eq1},} &\geq \frac {1}{M} \left ( \mathbb {E}{ \norm {\nabla _{\vlambda } f\left (\vt _{\vlambda }\left (\rvvu \right )\right )}_2^2 } - 2 L^2 \left (\mathbb {E}{f\left (\vt _{\vlambda }\left (\rvvu \right )\right )} - f^*\right ) \right ) \\ &\qquad + \norm { \nabla F\left (\vlambda \right ) }^2_2 \shortintertext {applying \cref {eq:thm_lower_bound_eq2},} &\geq \frac {2 \mu ^2 \left (d + 1\right ) - 2L^2}{ML} \left (\mathbb {E}{f\left (\vt _{\vlambda }\left (\rvvu \right )\right )} - f^*\right ) \\ &\qquad + \norm { \nabla F\left (\vlambda \right ) }^2_2 \\ &\geq \frac {2 \mu ^2 \left (d + 1\right ) - 2L^2}{ML} \left (F\left (\vlambda \right ) - h\left (\vlambda \right ) - f^*\right ) \\ &\qquad + \norm { \nabla F\left (\vlambda \right ) }^2_2 \\ &= \frac {2 \mu ^2 \left (d + 1\right ) - 2L^2}{ML} \left (F\left (\vlambda \right ) - F^*\right ) + \norm { \nabla F\left (\vlambda \right ) }^2_2 \\ &\qquad + \frac {2 \mu ^2 \left (d + 1\right ) - 2 L^2}{ML} \left (F^* - f^* - h\left (\vlambda \right ) \right ). \end {align*} The last term \begin {align*} \frac {2 \mu ^2 \left (d + 1\right ) - 2 L^2}{ML} \left (F^* - f^* - h\left (\vlambda \right ) \right ) \end {align*} can be shown to be positive if $\vlambda $ is sufficiently close to the optimum. Let $\vlambda ^* = \argmin _{\vlambda } F\left (\vlambda \right )$ be the minimizer of $F$. Then, we have \begin {align*} F^* - f^* - h\left (\vlambda \right ) &= \mathbb {E}{f\left (\vt _{\vlambda ^*}\left (\vu \right )\right )} + h\left (\vlambda ^*\right ) - f^* - h\left (\vlambda \right ) \\ &= \left (\mathbb {E}{f\left (\vt _{\vlambda ^*}\left (\vu \right )\right )} - f^*\right ) + \left (h\left (\vlambda ^*\right ) - h\left (\vlambda \right )\right ), \end {align*} where the first term is strictly positive and the second term goes to zero as $\vlambda \to \vlambda ^*$.\end{proof}


==> main-pratendsmoothness.tex <==


\prAtEndRestatexxi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxxi}Notice that \begin {align*} \gamma _1\left (x\right ) &= \frac { e^x }{ e^x } = 1 \\ \gamma _2\left (x\right ) &= \frac { e^x }{ e^{2x} } = e^{-x} \\ \gamma _3\left (x\right ) &= e^x e^x = e^{2x}. \nonumber \end {align*} Therefore, \begin {enumerate}[label=(\roman *)] \item holds trivially. \item holds trivially. \item The Lipschitzness of \(\gamma _2\left (x\right )\) is equivalent to whether \(e^x\) is Lipschitness, which it is not. \item The Lipschitzness of \(\gamma _3\left (x\right )\) is equivalent to whether \(e^{2x}\) is Lipschitness, which it is not. \end {enumerate}\end{proof}

\prAtEndRestatexxii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxxii}First, the log probability density of the half-normal distribution is given as \begin {align} \log f\left (x; \sigma \right ) = \left (\alpha - 1\right ) \log x - \beta x \nonumber \end {align} where \(\log Z\) is a constant normalizer. The derivatives of the inverse gamma distribution with a bijection \(\psi ^{-1}\) is given as \begin {align*} &\frac {d \log f\left (\psi ^{-1}\left (x\right ); \sigma \right )}{dx} \\ &\;= \frac {d \log f\left (\psi ^{-1}\left (x\right ); \sigma \right )}{d\psi } \frac {d \psi ^{-1}}{dx} \\ &\;= \frac {d \psi ^{-1}}{dx} \left ( \left (\alpha - 1\right ) \frac {1}{\psi ^{-1}\left (x\right )} - \beta \right ) \\ &\;= \left (\alpha - 1 \right ) \frac { {\left ( \psi ^{-1} \right )}^{\prime } \left (x\right ) }{\psi ^{-1}\left (x\right )} + \beta \psi ^{-1}\left (x\right ). \\ &\;= \left (\alpha - 1 \right ) \gamma _1\left (x\right ) + \beta {\left ( \psi ^{-1} \right )}^{\prime } \left (x\right ) \end {align*} Thus, the smoothness is euquivalent to the Lipschitzness of \(\gamma _3\left (x\right )\). \par By the triangle inequlity, the two-way inequality \begin {alignat*}{2} &\abs { \left (\alpha - 1 \right ) \abs { \gamma _1\left (x\right ) - \gamma _1\left (y\right ) } - \beta \abs { {\left ( \psi ^{-1} \right )}^{\prime } \left (x\right ) - {\left ( \psi ^{-1} \right )}^{\prime } \left (y\right ) } } \\ &\quad \leq \abs { \frac {d \log f\left (\psi ^{-1}\left (x\right ); \alpha , \beta \right )}{dx} - \frac {d \log f\left (\psi ^{-1}\left (y\right ); \alpha , \beta \right )}{dy} } \\ &\quad \quad \leq \left ( \alpha - 1 \right ) \abs { \gamma _1\left (x\right ) - \gamma _1\left (y\right ) } + \beta \abs { {\left ( \psi ^{-1} \right )}^{\prime } \left (x\right ) - {\left ( \psi ^{-1} \right )}^{\prime } \left (y\right ) } \end {alignat*} holds. The upper bound proves the implication (\(\Rightarrow \)), while the lower bounds (\(\Leftarrow \)) proves the converse by contraposition.\end{proof}

\prAtEndRestatexxiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxxiii}First, the log probability density of an inverse gamma distribution is given as \begin {align} \log f\left (x; \alpha , \beta \right ) = \left (-\alpha - 1\right ) \log x - \frac {\beta }{x} + \log Z, \nonumber \end {align} where \(\log Z\) is a constant normalizer. The derivatives of the inverse gamma distribution with a bijection \(\psi ^{-1}\) is given as \begin {align*} &\frac {d \log f\left (\psi ^{-1}\left (x\right ); \alpha , \beta \right )}{dx} \\ &\;= \frac {d \log f\left (\psi ^{-1}\left (x\right ); \alpha , \beta \right )}{d\psi } \frac {d \psi ^{-1}}{dx} \\ &\;= \frac {d \psi ^{-1}}{dx} \left ( \left ( - \alpha - 1 \right ) \frac {1}{\psi ^{-1}\left (x\right )} + \beta \frac {1}{{\psi ^{-1}\left (x\right )}^2} \right ) \\ &\;= \left ( - \alpha - 1 \right ) \frac { {\left ( \psi ^{-1} \right )}^{\prime } \left (x\right ) }{\psi ^{-1}\left (x\right )} + \beta \frac { {\left ( \psi ^{-1} \right )}^{\prime } \left (x\right ) }{{\psi ^{-1}\left (x\right )}^2}. \\ &\;= \left ( - \alpha - 1 \right ) \gamma _1\left (x\right ) + \beta \gamma _2\left (x\right ). \end {align*} \par By the triangle inequlity, the two-way inequality \begin {alignat*}{2} &\abs { \left ( \alpha + 1 \right ) \abs { \gamma _1\left (x\right ) - \gamma _1\left (y\right ) } - \beta \abs { \gamma _2\left (x\right ) - \gamma _2\left (y\right ) } } \\ &\quad \leq \abs { \frac {d \log f\left (\psi ^{-1}\left (x\right ); \alpha , \beta \right )}{dx} - \frac {d \log f\left (\psi ^{-1}\left (y\right ); \alpha , \beta \right )}{dy} } \\ &\quad \quad \leq \left ( \alpha + 1 \right ) \abs { \gamma _1\left (x\right ) - \gamma _1\left (y\right ) } + \beta \abs { \gamma _2\left (x\right ) - \gamma _2\left (y\right ) } \end {alignat*} holds. The upper bound proves the implication (\(\Rightarrow \)), while the lower bounds (\(\Leftarrow \)) proves the converse by contraposition.\end{proof}

\prAtEndRestatexxiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxxiv}First, the log probability density of the half-normal distribution is given as \begin {align} \log f\left (x; \sigma \right ) = -\frac {x^2}{2\sigma ^2} + \log Z, \nonumber \end {align} where \(\log Z\) is a constant normalizer. The derivatives of the inverse gamma distribution with a bijection \(\psi ^{-1}\) is given as \begin {align*} &\frac {d \log f\left (\psi ^{-1}\left (x\right ); \sigma \right )}{dx} \\ &\;= \frac {d \log f\left (\psi ^{-1}\left (x\right ); \sigma \right )}{d\psi } \frac {d \psi ^{-1}}{dx} \\ &\;= \frac {d \psi ^{-1}}{dx} \left ( -\frac { \psi ^{-1}\left (x\right ) }{\sigma ^2} \right ) \\ &\;= -\frac {1}{\sigma ^2} {\left ( \psi ^{-1} \right )}^{\prime }\left (x\right ) \psi ^{-1}\left (x\right ) \\ &\;= -\frac {1}{\sigma ^2} \gamma _3\left (x\right ) \end {align*} Thus, the smoothness is euquivalent to the Lipschitzness of \(\gamma _3\left (x\right )\).\end{proof}


==> main-pratendupperbound.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndii}\begin {alignat}{2} &\norm {\nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) }_2^2 \nonumber \\ &\;= {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \nonumber \\ &\;= {\nabla f^{\top }\left ( \vt _{\vlambda }\left (\vu \right ) \right )} {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \nonumber \\ &\;= {\vg _{f}^{\top }} {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \vg _{f}.\label {eq:thm:variational_gradient_norm_identity_eq1} \end {alignat} \par \paragraph {Proof for Full-Rank Cholesky (\cref {def:fullrank})} \par Let \(p\) denote the number of scalar variational parameters such that \(\vlambda = (\lambda _1, \ldots , \lambda _p)\). Then, \begin {alignat*}{2} &{\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \\ &\;= \sum ^{d}_{i=1} \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial m_i } {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial m_i } \right )}^{\top } + \sum ^{d}_{i=1} \sum ^{d}_{j=1} \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } \right )}^{\top }, \end {alignat*} where \(\lambda _{C_{ij}}\) denote the parameter responsible for the \(ij\)-th entry of \(\mC \), \(C_{ij}\). \par For the derivatives with respect to \(m_i\) and \(C_{ij}\), \citet {domke_provable_2020, domke_provable_2019} show that \begin {alignat}{2} \frac {\partial \vt _{\vlambda }\left (\vu \right ) }{ \partial m_i } &= \ve _i \quad \frac {\partial \vt _{\vlambda }\left (\vu \right ) }{ \partial C_{ij} } &= \ve _i u_j,\label {eq:covariance_derivative} \end {alignat} where \(\ve _i\) is the unit basis of the \(i\)th component. \par Therefore, \begin {alignat}{2} &{\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \nonumber \\ &\;= \sum ^{d}_{i=1} \ve _i \ve _i^{\top } + \sum ^{d}_{i=1} \sum ^{d}_{j=1} \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } \right )}^{\top } \nonumber \\ &\;= \mI + \underbrace { \sum ^{d}_{i=1} \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ii}} } {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ii}} } \right )}^{\top } }_{\text {diagonal of \(\mC \)}} \nonumber \\ &\qquad + \underbrace { \sum ^{d}_{i=1} \sum ^{d}_{j=1, j \neq i} \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } \right )}^{\top }}_{\text {off-diagonal of \(\mC \)}}, \label {eq:thm:variational_gradient_norm_identity_eq2} \end {alignat} leaving us with the derivatives of the scale term. \par The gradient with respect to \(\lambda _{C_{ij}}\), however, depends on the parameterization. That is, \begin {alignat}{2} \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } &= \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial C_{ij} } \frac { \partial C_{ij} }{ \partial \lambda _{C_{ij}} } &= \ve _i u_j \frac { \partial C_{ij} }{ \partial \lambda _{C_{ij}} }. \label {eq:thm:variational_gradient_norm_identity_covderivative} \end {alignat} \par For the diagonal elements, \(\lambda _{C_{ii}} = d_i\). Thus, \begin {align} \frac { \partial C_{ii} }{ \partial d_i } = \frac { \partial \phi _+\left (d_i\right ) }{ \partial d_i } = \phi _+^{\prime }\left (d_i\right ). \label {eq:thm:variational_gradient_norm_identity_diag} \end {align} And for the off-diagonal elements, \(\lambda _{L_{ij}} = L_{ij}\), and \begin {align} \frac { \partial C_{ij} }{ \partial L_{ij} } = 1. \label {eq:thm:variational_gradient_norm_identity_offdiag} \end {align} \par Plugging \cref {eq:thm:variational_gradient_norm_identity_diag,eq:thm:variational_gradient_norm_identity_offdiag,eq:thm:variational_gradient_norm_identity_covderivative} into \cref {eq:thm:variational_gradient_norm_identity_eq2}, \begin {alignat}{2} &{\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \nonumber \\ &\;= \mI + \underbrace { \sum ^{d}_{i=1} {\left ( u_j \phi _+^{\prime }\left (d_i\right ) \right )}^2 \ve _i \ve _i^{\top } }_{\text {diagonal of \(\mC \)}} + \underbrace { \sum ^{d}_{i=1} \sum ^{d}_{j=1, j \neq i} u_j^2 \, \ve _i \ve _i^{\top } }_{\text {off-diagonal of \(\mC \)}} \nonumber \\ &\;= \mI + \sum ^{d}_{i=1} u_i^2 {\left (\phi _+^{\prime }\left (d_i\right ) \right )}^2 \ve _i \ve _i^{\top } + \sum ^{d}_{i=1} \sum ^{d}_{j=1} u_j^2 \, \ve _i \ve _i^{\top } - \vu \vu ^{\top } \nonumber \\ &\;= \mI + \left (\vu \vu ^{\top }\right ) \Phi \Phi + \norm {\vu }_2^2 \, \mI - \vu \vu ^{\top } \nonumber \\ &\;= \left ( 1 + \norm {\vu }_2^2 \right )\mI + \left (\vu \vu ^{\top }\right ) \left ( \Phi \Phi - \mI \right ), \label {eq:eq:thm:variational_gradient_norm_identity_jacinner} \end {alignat} where \(\Phi \) is a diagonal matrix containing the derivatives of \(\phi _+\) as \begin {align*} \Phi = \mathrm {diag}\left ( \left [ \phi _+^{\prime }\left (d_1\right ), \ldots , \phi _+^{\prime }\left (d_d\right ) \right ] \right ). \end {align*} \par Coming back to \cref {eq:thm:variational_gradient_norm_identity_eq1}, \begin {alignat}{2} &\norm {\nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vu \right ) \right )} \nonumber \\ &\;= \vg _f^{\top } {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \vg \nonumber \\ &\;= \vg _{f}^{\top } \left \{\, \left (1 + \norm {\vu }_2^2 \right )\mI + \left (\vu \vu ^{\top }\right ) \left ( \Phi ^2 - \mI \right ) \,\right \} \vg _{f} \nonumber \\ &\;= \left (1 + \norm {\vu }_2^2\right ){\lVert \vg _{f} \rVert }_2^2 + \vg _{f}^{\top } \left (\vu \vu ^{\top }\right ) \left ( \Phi ^2 - \mI \right ) \vg _{f} \nonumber \\ &\;= \left (1 + \norm {\vu }_2^2\right ){\lVert \vg _{f} \rVert }_2^2 + \mathrm {tr}\left ( \vg _{f} \vg _{f}^{\top }\, \vu \vu ^{\top } \left ( \Phi ^2 - \mI \right ) \right ). \label {eq:eq:thm:variational_gradient_norm_identity_conclusion} \end {alignat} \par \paragraph {Proof for Mean-field (\cref {def:meanfield})} For the mean-field variational family, the covariance has only diagonal elements. Therefore, \cref {eq:eq:thm:variational_gradient_norm_identity_jacinner} becomes \begin {alignat}{2} {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } &= \mI + \left (\vu \vu ^{\top }\right ) \Phi ^2, \nonumber \end {alignat} and \cref {eq:eq:thm:variational_gradient_norm_identity_conclusion} becomes \begin {alignat}{2} \norm {\nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vu \right ) \right )} &= \vg _{f}^{\top } \left ( \mI + \left (\vu \vu ^{\top }\right ) \Phi ^2 \right ) \vg _{f} \nonumber \\ &= {\lVert \vg _{f} \rVert }_2^2 + \mathrm {tr}\left ( \vg _{f} \vg _{f}^{\top } \, \vu \vu ^{\top } \Phi ^2 \right ). \nonumber \end {alignat}\end{proof}


==> main-pratendupperboundkeylemm.tex <==


\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndix}\begin {alignat}{2} \mathbb {E}\norm {\vt _{\vlambda }\left (\rvvu \right ) - \vz }_2^2 \end {alignat}\end{proof}


==> main-pratendupperboundkeylemma.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndii}\begin {alignat}{2} &\norm {\nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) }_2^2 \nonumber \\ &\;= {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \nonumber \\ &\;= {\nabla f^{\top }\left ( \vt _{\vlambda }\left (\vu \right ) \right )} {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \nonumber \\ &\;= {\vg _{f}^{\top }} {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \vg _{f}.\label {eq:variational_gradient_norm_identity_eq1} \end {alignat} \par \paragraph {Proof for Cholesky} \par Let \(p\) denote the number of scalar variational parameters such that \(\vlambda = (\lambda _1, \ldots , \lambda _p)\). Then, \begin {alignat*}{2} &{\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \\ &\;= \sum ^{d}_{i=1} \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial m_i } {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial m_i } \right )}^{\top } + \sum ^{d}_{i=1} \sum ^{d}_{j \leq i} \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } \right )}^{\top }, \end {alignat*} where \(\lambda _{C_{ij}}\) denote the parameter responsible for the \(ij\)-th entry of \(\mC \), \(C_{ij}\). Notice that, unlike for the matrix square root parameterization~\citep {domke_provable_2019}, the sum for \(C_{ij}\) is only over the lower triangular section. \par For the derivatives with respect to \(m_i\) and \(C_{ij}\), \citet {domke_provable_2020, domke_provable_2019} show that \begin {alignat}{2} \frac {\partial \vt _{\vlambda }\left (\vu \right ) }{ \partial m_i } &= \ve _i \quad \frac {\partial \vt _{\vlambda }\left (\vu \right ) }{ \partial C_{ij} } &= \ve _i u_j,\label {eq:covariance_derivative} \end {alignat} where \(\ve _i\) is the unit basis of the \(i\)th component. \par Therefore, \begin {alignat}{2} &{\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \nonumber \\ &\;= \sum ^{d}_{i=1} \ve _i \ve _i^{\top } + \sum ^{d}_{i=1} \sum _{j \leq i} \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } \right )}^{\top } \nonumber \\ &\;= \mI + \underbrace { \sum ^{d}_{i=1} \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ii}} } {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ii}} } \right )}^{\top } }_{\text {diagonal of \(\mC \)}} \nonumber \\ &\qquad + \underbrace { \sum ^{d}_{i=1} \sum _{j < i} \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } \right )}^{\top }}_{\text {off-diagonal of \(\mC \)}}, \label {eq:thm:variational_gradient_norm_identity_eq2} \end {alignat} leaving us with the derivatives of the scale term. \par The gradient with respect to \(\lambda _{C_{ij}}\), however, depends on the parameterization. That is, \begin {alignat}{2} \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } &= \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial C_{ij} } \frac { \partial C_{ij} }{ \partial \lambda _{C_{ij}} } &= \ve _i u_j \frac { \partial C_{ij} }{ \partial \lambda _{C_{ij}} }. \label {eq:thm:variational_gradient_norm_identity_covderivative} \end {alignat} \par For the diagonal elements, \(\lambda _{C_{ii}} = d_i\). Thus, \begin {align} \frac { \partial C_{ii} }{ \partial s_i } = \frac { \partial \phi \left (s_i\right ) }{ \partial s_i } = \phi ^{\prime }\left (s_i\right ). \label {eq:thm:variational_gradient_norm_identity_diag} \end {align} And for the off-diagonal elements, \(\lambda _{L_{ij}} = L_{ij}\), and \begin {align} \frac { \partial C_{ij} }{ \partial L_{ij} } = 1. \label {eq:thm:variational_gradient_norm_identity_offdiag} \end {align} \par Plugging \cref {eq:thm:variational_gradient_norm_identity_diag,eq:thm:variational_gradient_norm_identity_offdiag,eq:thm:variational_gradient_norm_identity_covderivative} into \cref {eq:thm:variational_gradient_norm_identity_eq2}, \begin {alignat}{2} &{\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \nonumber \\ &\;= \mI + \underbrace { \sum ^{d}_{i=1} {\left ( u_j \phi ^{\prime }\left (s_i\right ) \right )}^2 \ve _i \ve _i^{\top } }_{\text {diagonal of \(\mC \)}} + \underbrace { \sum ^{d}_{i=1} \sum _{j=1, j < i} u_j^2 \, \ve _i \ve _i^{\top } }_{\text {off-diagonal of \(\mC \)}} \nonumber \\ &\;= \mI + \underbrace { \sum ^{d}_{i=1} u_i^2 {\left (\phi ^{\prime }\left (s_i\right ) \right )}^2 \ve _i \ve _i^{\top } }_{\text {diagonal of \(\mC \)}} + \underbrace { \sum ^{d}_{i=1} \sum _{j \leq i} u_j^2 \, \ve _i \ve _i^{\top } - \sum ^{d}_{i=1} u_i^2 \, \ve _i \ve _i^{\top } }_{\text {off-diagonal of \(\mC \)}} \nonumber \\ &\;= \mI + \underbrace { \mU \, \mPhi }_{\text {diagonal of \(\mC \)}} + \underbrace { \mY - \mU }_{\text {off-diagonal of \(\mC \)}} \nonumber \\ &\;= \left ( \mI + \mY \right ) + \mU \left ( \mPhi - \mI \right ), \label {eq:variational_gradient_norm_identity_jacinner} \end {alignat} where \(\mU ,\dot {\Phi }\) are diagonal matrices defined as \begin {alignat*}{2} & \mPhi &&= \mathrm {diag}\left ( \left [ {\phi ^{\prime }\left (s_1\right )}^2, \ldots , {\phi ^{\prime }\left (s_d\right )}^2 \right ] \right ) \\ &\mU &&= \mathrm {diag}\left ( \left [ u_1^2, \ldots , u_d^2 \right ] \right ) \\ &\mY &&= \mathrm {diag}\left ( \left [ u_1^2, u_1^2 + u_2^2,\, \ldots \,, {\textstyle \sum ^{d}_{i=1} u_i^2} \right ] \right ). \end {alignat*} The major difference with the proof of \citet [Lemma 8]{domke_provable_2019} for the matrix square root case is that we sum of the \(u_j^2 \ve _i \ve _i^{\top }\) terms is over the \textit {lower diagonal elements} instead of all the elements. This is the variance reduction effect we get for using the Cholesky parameterization. \par Coming back to \cref {eq:variational_gradient_norm_identity_eq1}, \begin {alignat}{2} &\norm {\nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vu \right ) \right )}_2^2 \nonumber \\ \;&= \vg _f^{\top } {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \vg \nonumber \\ &= \vg _{f}^{\top } \Big ( \left ( \mI + \mY \right ) + \mU \left ( \mPhi - \mI \right ) \Big ) \vg _{f} \nonumber \\ &= {\lVert \vg _{f} \rVert }_2^2 + \vg _{f}^{\top } \mY \vg _{f} + \vg _{f}^{\top } \mU \left ( \mPhi - \mI \right ) \vg _{f} \nonumber \\ &= {\lVert \vg _{f} \rVert }_2^2 + {\lVert \vg _{f} \rVert }_{\mY }^2 + \mathrm {tr}\left ( \vg _{f} \vg _{f}^{\top } \mU \left ( \mPhi - \mI \right ) \right ). \label {eq:variational_gradient_norm_identity_conclusion} \end {alignat} \par \paragraph {Proof for Mean-field} For the mean-field variational family, the covariance has only diagonal elements. Therefore, \cref {eq:variational_gradient_norm_identity_jacinner} becomes \begin {alignat}{2} {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } &= \mI + \mU \mPhi , \nonumber \end {alignat} and \cref {eq:variational_gradient_norm_identity_conclusion} becomes \begin {alignat}{2} \norm {\nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vu \right ) \right )} = \vg _{f}^{\top } \left ( \mI + \mU \mPhi \right ) \vg _{f} = {\lVert \vg _{f} \rVert }_2^2 + \mathrm {tr}\left ( \vg _{f} \vg _{f}^{\top } \, \mU \mPhi \right ). \nonumber \end {alignat}\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndiii}The proof continues from the result of \cref {thm:general_variational_gradient_norm_identity}. \par \paragraph {Proof for Cholesky} \cref {thm:general_variational_gradient_norm_identity} shows that \begin {alignat*}{2} \norm { \nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) }_2^2 = {\lVert \vg _{f} \rVert }_2^2 + {\lVert \vg _{f} \rVert }_{\mY }^2 + \mathrm {tr}\left ( \vg _{f} \vg _{f}^{\top } \mU \left ( \mPhi - \mI \right ) \right ). \end {alignat*} \par By the 1-Lipschitz assumption, the entries of the diagonal matrix \(\Phi \) satisfy \begin {align*} \Phi _{ii} = {\phi ^{\prime }\left (d_i\right )}^2 \leq 1, \end {align*} which means \(\mPhi \preceq \mI \) and thus \(\left ( \mPhi - \mI \right ) \preceq 0\). Also, \(\mU \), \(\vg _{f} \vg _{f}^{\top }\), and \(\left ( \mPhi - \mI \right )\) are all Hermitian. Based on this fact, applying \cref {thm:generalized_ruhe_inequality} reveals that \begin {alignat}{2} \mathrm {tr}\left ( \vg _{f} \vg _{f}^{\top }\, \mU \left ( \mPhi - \mI \right ) \right ) &\leq \sum _{i=1}^d \sigma _{i}\left (\vg _{f} \vg _{f}^{\top } \mU \right ) \sigma _i\left (\mPhi - \mI \right ) \nonumber \\ &\leq 0. \nonumber \end {alignat} Therefore, for the full rank Cholesky parameterization and a 1-Lipschitz positive map \(\phi \), \begin {alignat*}{2} \norm {\nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vu \right ) \right )} &= {\lVert \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \rVert }_2^2 + {\lVert \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \rVert }_{\mY }^2 \\ &\leq {\lVert \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \rVert }_2^2 + \norm { \mY }_{2,2} {\lVert \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \rVert }_2^2 \\ &= {\lVert \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \rVert }_2^2 + \left ( \sum ^{d}_{i=1} u_{i}^2 \right ) {\lVert \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \rVert }_2^2 \\ &= \left (1 + \norm {\vu }^2_2\right ) {\lVert \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \rVert }_2^2, \end {alignat*} where \(\norm {\mU }_{2,2}\) is the \(L_2\) operator norm of \(\mU \). This upper bound coincides with that of the matrix square root parameteration. Thus, unforunately, this bound will be loose for the Cholesky parameterization. \par \paragraph {Proof for Mean-field (\cref {def:meanfield})} For the mean-field parameterization,~\cref {thm:general_variational_gradient_norm_identity} shows that \begin {alignat*}{2} \norm { \nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) }_2^2 = {\lVert \vg _{f} \rVert }_2^2 + \mathrm {tr}\left ( \vg _{f} \vg _{f}^{\top } \mU \mPhi \right ), \end {alignat*} \par For the second term, \begin {alignat*}{2} \mathrm {tr}\left ( \vg _{f} \vg _{f}^{\top } \mU \mPhi \right ) &= \vg _{f}^{\top } \left ( \mU \mPhi \right ) \vg _{f} \\ &\leq {\lVert \mU \rVert }_{2,2} {\lVert \mPhi \rVert }_{2,2} {\lVert \vg _{f} \rVert }^2_2. \end {alignat*} By the \(1\)-Lipschitzness of \(\phi \), \[ {\lVert \mPhi \rVert }_{2,2} = \sigma _{\mathrm {max}}\left ( \mPhi \right ) = \max _{i = 1, \ldots , d} {\phi ^{\prime }\left ( s_i \right )}^2 \leq 1. \] Then, \begin {alignat}{2} \vg _{f}^{\top } \left ( \mU \mPhi \right ) \vg _{f} &\leq {\lVert \mU \rVert }_{2,2} \, {\lVert \vg _{f} \rVert }^2_2 \label {eq:variational_gradient_norm_identity_mf_eq1} \\ &\leq {\lVert \mU \rVert }_{\mathrm {F}} \, {\lVert \vg _{f} \rVert }^2_2, \label {eq:variational_gradient_norm_identity_mf_eq2} \end {alignat} which gives the result. Here, unlike the bounds on \(\mPhi \), the bounds in \cref {eq:variational_gradient_norm_identity_mf_eq1,eq:variational_gradient_norm_identity_mf_eq2} are quite loose, and become looser as the dimensionality increases. \par \end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndiv}The key idea is to prove a similar result as \cref {thm:reparam_u_identity}. For terms that zero-out during during the proof of \cref {thm:reparam_u_identity}, we apply \cref {thm:meanfield_superiority} to zero-out those same terms. \par \begin {alignat}{2} &\mathbb {E}\norm {\vt _{\vlambda }\left (\rvvu \right ) - \vz }_2^2 \, \left ( 1 + \norm {\mU }_{\mathrm {F}} \right ) \nonumber \\ &\;= \mathbb {E} \rvvu ^{\top } \mC ^{\top } \mC \rvvu \, \left ( 1 + \norm {\mU }_{\mathrm {F}} \right ) \nonumber \\ &\;\quad + 2\,\mathbb {E} \rvvu ^{\top } \mC ^{\top } \left ( \vm - \vz \right ) \left ( 1 + \norm {\mU }_{\mathrm {F}} \right ) \nonumber \\ &\;\quad + {\left ( \vm - \vz \right )}^{\top } \left ( \vm - \vz \right ) \left ( 1 + \mathbb {E} \norm {\mU }_{\mathrm {F}} \right ) \nonumber \shortintertext {invoking the trace trick,} &\;= \norm {\vm - \vz } \left ( 1 + \mathbb {E} \norm {\mU }_{\mathrm {F}}\right ). \nonumber \\ &\;\quad + 2\,\mathbb {E} \left ( 1 + \norm {\mU }_{\mathrm {F}} \right ) \, \rvvu ^{\top } \mC ^{\top } \left ( \vm - \vz \right ) \nonumber \\ &\;\quad + \mathrm {tr}\left ( \mC ^{\top } \mC \, \mathbb {E} \rvvu \rvvu ^{\top } \left ( 1 + \norm {\mU }_{\mathrm {F}}\right ) \right ) \nonumber \end {alignat} \par \begin {alignat*}{2} \mathbb {E} \norm {\mathbfsf {U}}_{\mathrm {F}} &\;= \mathbb {E} \sqrt { \mathrm {tr}\left ( \mathbfsf {U} \mathbfsf {U} \right ) } \\ &\;= \mathbb {E} \sqrt { \sum _{i=1}^d \rvu _i^4 }, \shortintertext {using Jensen's inequality,} &\;\leq \sqrt { \mathbb {E} \sum _{i=1}^d \rvu _i^4 } \\ &\;= \sqrt { d \kappa }. \end {alignat*} \par \begin {alignat*}{2} \mathbb {E} \left ( \norm {\mathbfsf {U}}_{\mathrm {F}} + 1\right ) \rvu _i &\;= \mathbb {E} \left ( \sqrt { \sum ^d_{i=1} \rvu _i^4 } + 1\right ) \rvu _i \\ &\;\leq \mathbb {E} \left ( \sum ^d_{i=1} \rvu _i^2 + 1\right ) \rvu _i \\ &\;= \mathbb {E} \, \rvu _i \, \sum _{j \neq i} \rvu _j^2 + \rvu _i^3 + \rvu _i \shortintertext {applying \cref {assumption:symmetric_standard},} &\;= 0. \end {alignat*} \par \begin {alignat*}{2} \mathbb {E} \rvu _i \rvu _j \norm {\mathbfsf {U}}_{\mathrm {F}} &\;= \mathbb {E} \rvu _i \rvu _j \left ( \sqrt { \sum _{k=1}^d \rvu _k^4 } \right ) \\ &\;\leq \mathbb {E} \rvu _i \rvu _j \sum _{k=1}^d \rvu _k^2 \\ &\;= \mathbb {E} \rvu _i^3 + \rvu _j^3 + \rvu _i \rvu _j \sum _{k \neq i, j} \rvu _k^2 \\ &\;= 0. \end {alignat*} \par \begin {alignat*}{2} \mathbb {E} \rvu _i \rvu _i \norm {\mathbfsf {U}}_{\mathrm {F}} &\;= \mathbb {E} \rvu _i^2 \left ( \sqrt { \sum _{k=1}^d \rvu _k^4 } \right ), \shortintertext {applying Cauchy-Schwarz's inequality for expectations,} &\;\leq \sqrt { \left ( \mathbb {E} \sum _{k=1}^d \rvu _k^4 \right ) \left ( \mathbb {E} \rvu _i^4 \right ) }, \shortintertext {and given \cref {assumption:symmetric_standard},} &\;= \sqrt { \left ( d \kappa \right ) \left ( \kappa \right ) } \\ &\;= \kappa \sqrt { d }. \end {alignat*} \par Combining all the results, \begin {alignat*}{2} &\mathbb {E}\norm {\vt _{\vlambda }\left (\rvvu \right ) - \vz }_2^2 \, \left ( 1 + \norm {\mU }_{\mathrm {F}} \right ) \\ &\;\leq \norm { \vm - \vz }_2^2 \left ( \vm - \vz \right ) \left ( 1 + \mathbb {E} \norm {\mU }_{\mathrm {F}}\right ) \\ &\;\quad + 2\,\mathbb {E} \left ( 1 + \norm {\mU }_{\mathrm {F}} \right ) \, \rvvu ^{\top } \mC ^{\top } \left ( \vm - \vz \right ) \\ &\;\quad + \mathrm {tr}\left ( \mC ^{\top } \mC \, \mathbb {E} \rvvu \rvvu ^{\top } \left ( 1 + \norm {\mU }_{\mathrm {F}}\right ) \right ) \\ &\;\leq \sqrt {d \kappa } \norm { \vm - \vz }_2^2 + \mathrm {tr}\left ( \mC ^{\top } \mC \left (\mI + \kappa \sqrt {d} \mI \right ) \right ) \\ &\;= \sqrt {d \kappa } \norm { \vm - \vz }_2^2 + \left (\kappa \sqrt {d} + 1\right ) \mathrm {tr}\left ( \mC ^{\top } \mC \right ) \\ &\;= \sqrt {d \kappa } \norm { \vm - \vz }_2^2 + \left (\kappa \sqrt {d} + 1\right ) \norm { \mC }_{\mathrm {F}}^2. \end {alignat*} \par \end{proof}

\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndix}From the definition of variance, \begin {alignat}{2} &\mathbb {E} \norm {\vg _M }^2_2 \nonumber \\ &\;= \mathrm {tr}\,\V { \vg _M } + \norm {\mathbb {E} \vg }^2_2, \nonumber \shortintertext {following the definition in \cref {eq:def_gradient_M_est},} &\;= \mathrm {tr}\,\V { \frac {1}{M} \sum _{m=1}^M \vg _m } + \norm { \nabla F\left (\vlambda \right ) }^2_2, \nonumber \shortintertext {and then the definition in \cref {eq:def_gradient_m_est},} &\;= \mathrm {tr}\,\V { \frac {1}{M} \sum _{m=1}^M \nabla _{\vlambda } f\left (\vt _{\vlambda }\left (\rvvu _m\right )\right ) + \nabla h\left (\vlambda \right ) } + \norm { \nabla F\left (\vlambda \right ) }^2_2, \nonumber \shortintertext {by the linearity of variance,} &\;= \frac {1}{M} \mathrm {tr}\,\V { \nabla _{\vlambda } f\left (\vt _{\vlambda }\left (\rvvu \right )\right ) } + \norm { \nabla F\left (\vlambda \right ) }^2_2 \\ &\;= \frac {1}{M} \left ( \mathbb {E}{ \norm {\nabla _{\vlambda } f\left (\vt _{\vlambda }\left (\rvvu \right )\right )}_2^2 } - \norm { \mathbb {E}{ \nabla _{\vlambda } f\left (\vt _{\vlambda }\left (\rvvu \right )\right )} }_2^2 \right ) + \norm { \nabla F\left (\vlambda \right ) }^2_2 \nonumber \\ &\;\leq \frac {1}{M} \mathbb {E}{ \norm { \nabla _{\vlambda } f\left (\vt _{\vlambda }\left (\rvvu \right )\right ) }_2^2 } + \norm { \nabla F\left (\vlambda \right ) }^2_2. \nonumber \end {alignat} The results follow from applying \cref {thm:general_variational_gradient_norm_bound} accordingly. \par \todo [inline]{ I think it might be possible to do something about the \[ -\norm {\mathbb {E}{ \nabla _{\vlambda } f\left (\vt _{\vlambda }\left (\rvvu \right )\right )}}_2^2 \] term instead of just upper bounding it by 0. In fact, it is possible to generalize \cref {thm:general_variational_gradient_norm_identity} such that \begin {align*} &\inner { \nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) }{ \nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vv \right ) \right ) } \\ &\;= \left (1 + \inner {\vu }{\vv }\right ) \inner {\vg _{f,\vu }}{\vg _{f,\vv }} + \mathrm {tr}\left ( \vg _{f,\vu } \vg _{f,\vv }^{\top }\, \vv \vu ^{\top } \left ( \Phi ^2 - \mI \right ) \right ), \end {align*} where \(\vg _{f,\vu } = \nabla f\left (\vt _{\vlambda }\left (\vu \right )\right )\). }\end{proof}


==> main-pratendupperboundkeylemmagradientnormbound.tex <==


\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndiii}The proof continues from the result of \cref {thm:general_variational_gradient_norm_identity}. \par \paragraph {Proof for Cholesky} \cref {thm:general_variational_gradient_norm_identity} shows that \begin {alignat*}{2} \norm { \nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) }_2^2 = {\lVert \vg _{f} \rVert }_2^2 + \vg _{f}^{\top } \mSigma \vg _{f} + \vg _{f}^{\top } \mU \left ( \mPhi - \boldupright {I} \right ) \vg _{f}, \end {alignat*} where \(\vg _f = \nabla f\left (\vt _{\vlambda }\left (\vu \right )\right ) \). \par By the 1-Lipschitz assumption, the entries of the diagonal matrix \(\Phi \) satisfy \begin {align*} \Phi _{ii} = {\phi ^{\prime }\left (d_i\right )}^2 \leq 1, \end {align*} which means \begin {alignat*}{2} \mPhi \preceq \boldupright {I} \;\Rightarrow \; \mU \left ( \mPhi - \boldupright {I} \right ) \preceq 0 \;\Rightarrow \; {\vg _{f}}^{\top } \mU \left ( \mPhi - \boldupright {I} \right ) \vg _{f} \leq 0. \end {alignat*} Therefore, for the full-rank Cholesky parameterization and a 1-Lipschitz conditioner \(\phi \), \begin {alignat*}{2} &\norm {\nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vu \right ) \right )}_2^2 \\ &\;= {\lVert \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \rVert }_2^2 + {\vg _{f}}^{\top } \mSigma \vg _{f} + {\vg _{f}}^{\top } \mU \left ( \mPhi - \boldupright {I} \right ) \vg _{f} \\ &\;\leq {\lVert \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \rVert }_2^2 + {\vg _{f}}^{\top } \mSigma \vg _{f} \\ &\;\leq {\lVert \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \rVert }_2^2 + \norm { \mSigma }_{2,2} {\lVert \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \rVert }_2^2 \\ &\;= {\lVert \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \rVert }_2^2 + \left ( \sum ^{d}_{i=1} u_{i}^2 \right ) {\lVert \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \rVert }_2^2 \\ &\;= \left (1 + \norm {\vu }^2_2\right ) {\lVert \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \rVert }_2^2, \end {alignat*} where \(\norm {\mU }_{2,2}\) is the \(L_2\) operator norm of \(\mU \). This upper bound coincides with that of the matrix square root parameteration. Thus, unforunately, this bound fails to acknowledge the lower variance of the Cholesky parameterization, coinciding with that of the matrix square root parameterization. \par \paragraph {Proof for Mean-field (\cref {def:meanfield})} For the mean-field parameterization,~\cref {thm:general_variational_gradient_norm_identity} shows that \begin {alignat*}{2} \norm { \nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) }_2^2 = {\lVert \vg _{f} \rVert }_2^2 + \vg _{f}^{\top } \mU \mPhi \vg _{f}. \end {alignat*} \par For the second term, \begin {alignat*}{2} \vg _{f}^{\top } \mU \mPhi \vg _{f} \leq {\lVert \mU \rVert }_{2,2} {\lVert \mPhi \rVert }_{2,2} {\lVert \vg _{f} \rVert }^2_2. \end {alignat*} By the \(1\)-Lipschitzness of \(\phi \), \[ {\lVert \mPhi \rVert }_{2,2} = \sigma _{\mathrm {max}}\left ( \mPhi \right ) = \max _{i = 1, \ldots , d} {\phi ^{\prime }\left ( s_i \right )}^2 \leq 1. \] Then, \begin {alignat}{2} \vg _{f}^{\top } \left ( \mU \mPhi \right ) \vg _{f} &\leq {\lVert \mU \rVert }_{2,2} \, {\lVert \vg _{f} \rVert }^2_2 \label {eq:variational_gradient_norm_identity_mf_eq1} \\ &\leq {\lVert \mU \rVert }_{\mathrm {F}} \, {\lVert \vg _{f} \rVert }^2_2, \label {eq:variational_gradient_norm_identity_mf_eq2} \end {alignat} which gives the result. Here, unlike the bounds on \(\mPhi \), the bounds in \cref {eq:variational_gradient_norm_identity_mf_eq1,eq:variational_gradient_norm_identity_mf_eq2} are quite loose, and become looser as the dimensionality increases. \par \end{proof}


==> main-pratendupperboundkeylemmagradientnormidentity.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndii}The proof starts by applying the Chain Rule and then computing the quadratic norm of the gradient as \begin {alignat}{2} &\norm {\nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) }_2^2 \nonumber \\ &\;= {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \nonumber \\ &\;= {\nabla f^{\top }\left ( \vt _{\vlambda }\left (\vu \right ) \right )} {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \nabla f\left ( \vt _{\vlambda }\left (\vu \right ) \right ) \nonumber \\ &\;= {\vg _{f}^{\top }} {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \vg _{f}.\label {eq:variational_gradient_norm_identity_eq1} \end {alignat} Naturally, the derivative of the reparameterization function will depend on the specific parameterization used. \par \paragraph {Proof for Cholesky} \par Let \(p\) denote the number of scalar variational parameters such that \(\vlambda = (\lambda _1, \ldots , \lambda _p)\). Then, \begin {alignat*}{2} &{\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \\ &\;= \sum ^{d}_{i=1} \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial m_i } {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial m_i } \right )}^{\top } + \sum ^{d}_{i=1} \sum ^{d}_{j \leq i} \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } \right )}^{\top }, \end {alignat*} where \(\lambda _{C_{ij}}\) denote the parameter responsible for the \(ij\)-th entry of \(\mC \), \(C_{ij}\). Notice that, unlike for the matrix square root parameterization~\citep {domke_provable_2019}, the sum for \(C_{ij}\) is only over the lower triangular section. \par For the derivatives with respect to \(m_i\) and \(C_{ij}\), \citet {domke_provable_2020, domke_provable_2019} show that \begin {alignat}{2} \frac {\partial \vt _{\vlambda }\left (\vu \right ) }{ \partial m_i } &= \boldupright {e}_i \quad \frac {\partial \vt _{\vlambda }\left (\vu \right ) }{ \partial C_{ij} } &= \boldupright {e}_i u_j,\label {eq:covariance_derivative} \end {alignat} where \(\boldupright {e}_i\) is the unit basis of the \(i\)th component. \par Therefore, \begin {alignat}{2} &{\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \nonumber \\ &\;= \sum ^{d}_{i=1} \boldupright {e}_i \boldupright {e}_i^{\top } + \sum ^{d}_{i=1} \sum _{j \leq i} \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } \right )}^{\top } \nonumber \\ &\;= \boldupright {I} + \underbrace { \sum ^{d}_{i=1} \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ii}} } {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ii}} } \right )}^{\top } }_{\text {diagonal of \(\mC \)}} \nonumber \\ &\qquad + \underbrace { \sum ^{d}_{i=1} \sum _{j < i} \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } \right )}^{\top }}_{\text {off-diagonal of \(\mC \)}}, \label {eq:thm:variational_gradient_norm_identity_eq2} \end {alignat} leaving us with the derivatives of the scale term. \par The gradient with respect to \(\lambda _{C_{ij}}\), however, depends on the parameterization. That is, \begin {alignat}{2} \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \lambda _{C_{ij}} } &= \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial C_{ij} } \frac { \partial C_{ij} }{ \partial \lambda _{C_{ij}} } &= \boldupright {e}_i u_j \frac { \partial C_{ij} }{ \partial \lambda _{C_{ij}} }. \label {eq:thm:variational_gradient_norm_identity_covderivative} \end {alignat} \par For the diagonal elements, \(\lambda _{C_{ii}} = s_i\). Thus, \begin {align} \frac { \partial C_{ii} }{ \partial s_i } = \frac { \partial \phi \left (s_i\right ) }{ \partial s_i } = \phi ^{\prime }\left (s_i\right ). \label {eq:thm:variational_gradient_norm_identity_diag} \end {align} And for the off-diagonal elements, \(\lambda _{L_{ij}} = L_{ij}\), and \begin {align} \frac { \partial C_{ij} }{ \partial L_{ij} } = 1. \label {eq:thm:variational_gradient_norm_identity_offdiag} \end {align} \par Plugging \cref {eq:thm:variational_gradient_norm_identity_diag,eq:thm:variational_gradient_norm_identity_offdiag,eq:thm:variational_gradient_norm_identity_covderivative} into \cref {eq:thm:variational_gradient_norm_identity_eq2}, \begin {alignat}{2} &{\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \nonumber \\ &\;= \boldupright {I} + \underbrace { \sum ^{d}_{i=1} {\left ( u_i \phi ^{\prime }\left (s_i\right ) \right )}^2 \boldupright {e}_i \boldupright {e}_i^{\top } }_{\text {diagonal of \(\mC \)}} + \underbrace { \sum ^{d}_{i=1} \sum _{j=1, j < i} u_j^2 \, \boldupright {e}_i \boldupright {e}_i^{\top } }_{\text {off-diagonal of \(\mC \)}} \nonumber \\ &\;= \boldupright {I} + \underbrace { \sum ^{d}_{i=1} u_i^2 {\left (\phi ^{\prime }\left (s_i\right ) \right )}^2 \boldupright {e}_i \boldupright {e}_i^{\top } }_{\text {diagonal of \(\mC \)}} + \underbrace { \sum ^{d}_{i=1} \sum _{j \leq i} u_j^2 \, \boldupright {e}_i \boldupright {e}_i^{\top } - \sum ^{d}_{i=1} u_i^2 \, \boldupright {e}_i \boldupright {e}_i^{\top } }_{\text {off-diagonal of \(\mC \)}} \nonumber \\ &\;= \boldupright {I} + \underbrace { \mU \, \mPhi }_{\text {diagonal of \(\mC \)}} + \underbrace { \mSigma - \mU }_{\text {off-diagonal of \(\mC \)}} \nonumber \\ &\;= \left ( \boldupright {I} + \mSigma \right ) + \mU \left ( \mPhi - \boldupright {I} \right ), \label {eq:variational_gradient_norm_identity_jacinner} \end {alignat} where \(\mU ,\mPhi ,\mSigma \) are diagonal matrices defined as \begin {alignat*}{2} & \mPhi &&= \mathrm {diag}\left ( \left [ {\phi ^{\prime }\left (s_1\right )}^2, \ldots , {\phi ^{\prime }\left (s_d\right )}^2 \right ] \right ) \\ &\mU &&= \mathrm {diag}\left ( \left [ u_1^2, \ldots , u_d^2 \right ] \right ) \\ &\mSigma &&= \mathrm {diag}\left ( \left [ u_1^2, u_1^2 + u_2^2,\, \ldots \,, {\textstyle \sum ^{d}_{i=1} u_i^2} \right ] \right ). \end {alignat*} The major difference with the proof of \citet [Lemma 8]{domke_provable_2019} for the matrix square root case is that we only sum the \(u_j^2 \boldupright {e}_i \boldupright {e}_i^{\top }\) terms over the \textit {lower diagonal elements}. This is the variance reduction effect we get from using the Cholesky parameterization. \par Coming back to \cref {eq:variational_gradient_norm_identity_eq1}, \begin {alignat}{2} &\norm {\nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vu \right ) \right )}_2^2 \nonumber \\ \;&= \vg _f^{\top } {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \vg \nonumber \\ &= \vg _{f}^{\top } \Big ( \left ( \boldupright {I} + \mSigma \right ) + \mU \left ( \mPhi - \boldupright {I} \right ) \Big ) \vg _{f} \nonumber \\ &= {\lVert \vg _{f} \rVert }_2^2 + \vg _{f}^{\top } \mSigma \vg _{f} + \vg _{f}^{\top } \mU \left ( \mPhi - \boldupright {I} \right ) \vg _{f}. \label {eq:variational_gradient_norm_identity_conclusion} \end {alignat} \par \paragraph {Proof for Mean-field} For the mean-field variational family, the covariance has only diagonal elements. Therefore, \cref {eq:variational_gradient_norm_identity_jacinner} becomes \begin {alignat}{2} {\left ( \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \vt _{\vlambda }\left (\vu \right ) }{ \partial \vlambda } &= \boldupright {I} + \mU \mPhi , \nonumber \end {alignat} and \cref {eq:variational_gradient_norm_identity_conclusion} becomes \begin {alignat}{2} \norm {\nabla _{\vlambda } f\left ( \vt _{\vlambda }\left (\vu \right ) \right )}_2^2 = \vg _{f}^{\top } \left ( \boldupright {I} + \mU \mPhi \right ) \vg _{f} = {\lVert \vg _{f} \rVert }_2^2 + \vg _{f}^{\top } \mU \mPhi \vg _{f}. \nonumber \end {alignat}\end{proof}


==> main-pratendupperboundkeylemmameanfield.tex <==


\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndiv}The key idea is to prove a similar result as \cref {thm:reparam_u_identity}, but with better constants to reflect that the mean-field parameterization has a lower variance. \par First, \begin {align} &\mathbb {E}\norm {\vt _{\vlambda }\left (\rvvu \right ) - \vz }_2^2 \, \left ( 1 + \norm {\mathbfsfit {U}}_{\mathrm {F}} \right ) \nonumber \\ &\;= \mathbb {E}\norm {\vt _{\vlambda }\left (\rvvu \right ) - \vz }_2^2 + \mathbb {E} \norm {\mathbfsfit {U}}_{\mathrm {F}} \, \norm {\vt _{\vlambda }\left (\rvvu \right ) - \vz }_2^2, \nonumber \shortintertext {applying \cref {thm:reparam_quadratic},} &\;= \norm { \vm - \vz }_2^2 + \norm {\mC }_{\mathrm {F}} + \mathbb {E} \norm {\mathbfsfit {U}}_{\mathrm {F}} \, \norm {\vt _{\vlambda }\left (\rvvu \right ) - \vz }_2^2. \label {thm:meanfield_eq0} \end {align} \par The last term decomposes as \begin {alignat}{2} \mathbb {E} \norm {\mathbfsfit {U}}_{\mathrm {F}} \norm {\vt _{\vlambda }\left (\rvvu \right ) - \vz }_2^2 \nonumber &= \underbrace { \mathbb {E} \norm {\mathbfsfit {U}}_{\mathrm {F}} \, \rvvu ^{\top } \mC ^{\top } \mC \rvvu }_{\text {Term \ding {182}}} \nonumber \\ &\quad + 2\, \underbrace { \mathbb {E} \norm {\mathbfsfit {U}}_{\mathrm {F}} \, \rvvu ^{\top } \mC ^{\top } \left ( \vm - \vz \right ) }_{\text {Term \ding {183}}} \nonumber \\ &\quad + \underbrace {\mathbb {E} \norm {\mathbfsfit {U}}_{\mathrm {F}}}_{\text {Term \ding {184}}} \, \norm { \vm - \vz }_2^2. \label {thm:meanfield_eq1} \end {alignat} We will now focus on the stochastic terms \ding {182}-\ding {184} one by one. \par First, for Term \ding {182}, notice that the mean-field parameterization implies that \(\mC = \mathrm {diag}\left ( c_1, \ldots , c_d \right )\). Thus, \begin {alignat}{2} \mathbb {E} \norm {\mathbfsfit {U}}_{\mathrm {F}} \, \rvvu ^{\top } \mC ^{\top } \mC \rvvu &= \mathbb {E} \left ( \sqrt { \sum _{i=1}^d \rvu _i^4 } \right ) \left ( \sum _{i=1}^d c_i^2 \, u_i^2 \right ) \nonumber \\ &= \sum _{i=1}^d c_i^2 \, \mathbb {E} \left ( \sqrt { \sum _{j=1}^d \rvu _j^4 } \right ) \rvu _i^2, \nonumber \shortintertext {applying Cauchy-Schwarz inequality for expectations,} &\leq \sum _{i=1}^d c_i^2 \sqrt { \left ( \mathbb {E} \sum _{j=1}^d \rvu _j^4 \right ) \left ( \mathbb {E} \rvu _i^4 \right ) } \nonumber \shortintertext {and given \cref {assumption:symmetric_standard},} &\;= \sum _{i=1}^d c_i^2 \, \sqrt { d \kappa ^2 } \nonumber \\ &\;= \kappa \sqrt {d} \, \norm { \mC }_{\mathrm {F}}^2. \label {thm:meanfield_eq5} \end {alignat} \par Term \ding {183} can be bounded as \begin {alignat}{2} &\mathbb {E} \norm {\mathbfsfit {U}}_{\mathrm {F}} \, \rvvu ^{\top } \mC ^{\top } \left ( \vm - \vz \right ) \nonumber \shortintertext {using the Cauchy-Schwarz inequality for vectors as} &\;\leq \mathbb {E} \norm {\mathbfsfit {U}}_{\mathrm {F}} \, \norm {\mC \rvvu }_2 \norm { \vm - \vz }_2, \nonumber \shortintertext {again, applying the inequality for expectations,} &\;= \sqrt { \mathbb {E} \norm {\mathbfsfit {U}}_{\mathrm {F}}^2 \, \mathbb {E} \norm {\mC \rvvu }_2^2 } \, \norm { \vm - \vz }_2 \nonumber \\ &\;= \sqrt { \mathbb {E} \left ( \sum ^d_{i=1} \rvu _i^4 \right ) \, \mathrm {tr}\left (\mC ^{\top } \mC \, \mathbb {E} \rvvu \rvvu ^{\top } \right ) } \, \norm { \vm - \vz }_2, \nonumber \shortintertext {from \cref {assumption:symmetric_standard},} &\;= \sqrt { d \kappa \, \mathrm {tr}\left (\mC ^{\top } \mC \right ) } \, \norm { \vm - \vz }_2 \nonumber \\ &\;= \sqrt {d \kappa } \, \norm {\mC }_{\mathrm {F}} \, \norm { \vm - \vz }_2 \nonumber \\ &\;= \sqrt {d \kappa } \, \sqrt { \norm {\mC }_{\mathrm {F}}^2 \, \norm { \vm - \vz }_2^2 }, \nonumber \shortintertext {and by the arithmetic mean-geometric mean inequality,} &\;= \frac {\sqrt {d \kappa }}{2} \left ( \norm {\mC }_{\mathrm {F}}^2 + \norm { \vm - \vz }_2^2 \right ). \label {thm:meanfield_eq3} \end {alignat} \par Finally, Term \ding {184} follows as \begin {alignat}{2} \mathbb {E} \norm {\mathbfsfit {U}}_{\mathrm {F}} &= \mathbb {E} \sqrt { \sum _{i=1}^d \rvu _i^4 }, \nonumber \shortintertext {using Jensen's inequality,} &\leq \sqrt { \mathbb {E} \sum _{i=1}^d \rvu _i^4 } \nonumber \\ &= \sqrt { d \kappa }. \label {thm:meanfield_eq2} \end {alignat} \par Combining all the results, \cref {thm:meanfield_eq0} becomes \begin {alignat*}{2} &\mathbb {E}\norm {\vt _{\vlambda }\left (\rvvu \right ) - \vz }_2^2 \, \left ( 1 + \norm {\mathbfsfit {U}}_{\mathrm {F}} \right ) \\ &\;\leq \norm { \vm - \vz }_2^2 + \norm {\mC }_{\mathrm {F}}^2 \\ &\;\quad + \mathbb {E} \norm {\mathbfsfit {U}}_{\mathrm {F}} \, \rvvu ^{\top } \mC ^{\top } \mC \rvvu \\ &\;\quad + 2\,\mathbb {E} \norm {\mathbfsfit {U}}_{\mathrm {F}} \, \rvvu ^{\top } \mC ^{\top } \norm { \vm - \vz }_2^2 \\ &\;\quad + \mathbb {E} \norm {\mathbfsfit {U}}_{\mathrm {F}} \, \norm { \vm - \vz }_2^2 \shortintertext {and applying \cref {thm:meanfield_eq2,thm:meanfield_eq3,thm:meanfield_eq5},} &\;\leq \norm { \vm - \vz }_2^2 + \norm {\mC }_{\mathrm {F}}^2 \\ &\;\quad + \kappa \sqrt {d} \norm {\mC }_{\mathrm {F}} \\ &\;\quad + \kappa \sqrt {d} \left ( \norm {\mC }_{\mathrm {F}}^2 + \norm {\vm - \vz }_2^2 \right ) \\ &\;\quad + \sqrt {d \kappa } \, \norm { \vm - \vz }_2^2 \\ &\;= \left (\sqrt {d \kappa } + \kappa \sqrt {d} + 1\right ) \, \norm { \vm - \vz }_2^2 + \left (2 \kappa \sqrt {d} + 1\right ) \norm {\mC }_{\mathrm {F}}^2. \end {alignat*} \par \end{proof}


==> main-pratendupperboundkeylemmavariancegeneral.tex <==


\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndv}From the definition of variance, \begin {alignat}{2} &\mathbb {E} \norm {\vg _M }^2_2 \nonumber \\ &\;= \mathrm {tr}\,\V { \vg _M } + \norm {\mathbb {E} \vg _M }^2_2, \nonumber \shortintertext {following the definition in \cref {eq:def_gradient_M_est},} &\;= \mathrm {tr}\,\V { \frac {1}{M} \sum _{m=1}^M \vg _m } + \norm { \nabla F\left (\vlambda \right ) }^2_2, \nonumber \shortintertext {and then the definition in \cref {eq:def_gradient_m_est},} &\;= \mathrm {tr}\,\V { \frac {1}{M} \sum _{m=1}^M \nabla _{\vlambda } f\left (\vt _{\vlambda }\left (\rvvu _m\right )\right ) + \nabla h\left (\vlambda \right ) } + \norm { \nabla F\left (\vlambda \right ) }^2_2, \nonumber \shortintertext {by the linearity of variance,} &\;= \frac {1}{M} \mathrm {tr}\,\V { \nabla _{\vlambda } f\left (\vt _{\vlambda }\left (\rvvu \right )\right ) } + \norm { \nabla F\left (\vlambda \right ) }^2_2 \nonumber \\ &\;= \frac {1}{M} \left ( \mathbb {E}{ \norm {\nabla _{\vlambda } f\left (\vt _{\vlambda }\left (\rvvu \right )\right )}_2^2 } - \norm { \mathbb {E}{ \nabla _{\vlambda } f\left (\vt _{\vlambda }\left (\rvvu \right )\right )} }_2^2 \right ) \nonumber \\ &\qquad + \norm { \nabla F\left (\vlambda \right ) }^2_2 \label {eq:thm_gradient_variance_general_definition} \\ &\;\leq \frac {1}{M} \mathbb {E}{ \norm { \nabla _{\vlambda } f\left (\vt _{\vlambda }\left (\rvvu \right )\right ) }_2^2 } + \norm { \nabla F\left (\vlambda \right ) }^2_2. \nonumber \end {alignat}\end{proof}


==> main-pratendupperboundlemma.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevi}\label{thm:prAtEndvi}\label {thm:reparam_quadratic} Let \(\vt _{\vlambda }: \mathbb {R}^d \rightarrow \mathbb {R}^d\) be a location-scale reparameterizaiton function (\cref {def:reparam}). Also, let \(\vz \in \mathbb {R}^d\) be some vector, and let \(\rvvu \sim \varphi \) satisfy~\cref {assumption:symmetric_standard}. Then, \begin {alignat*}{2} \mathbb {E}\norm {\vt _{\vlambda }\left (\rvvu \right ) - \vz }_2^2 &= \norm {\vm - \vz }^2_2 + \norm {\mC }_{\mathrm {F}}^2. \end {alignat*}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndvi}\begin {alignat}{2} \mathbb {E}\norm { \vt _{\vlambda }\left (\rvvu \right ) - \vz }_2^2 &= \mathbb {E}\norm { \mC \rvvu + \vm - \vz }_2^2 \nonumber \\ &= \mathbb {E} \rvvu ^{\top } \mC ^{\top } \mC \rvvu + 2\,\mathbb {E} \rvvu ^{\top } \mC ^{\top } \vm - 2\,\mathbb {E} \rvvu ^{\top } \mC ^{\top } \vz \nonumber \\ &\;\quad + \vm ^{\top } \vm - 2\,\vm ^{\top } \vz + \vz ^{\top } \vz . \label {eq:reparam_quadratic_eq1} \end {alignat} The first three terms follow as \begin {alignat*}{2} &\mathbb {E} \rvvu ^{\top } \mC ^{\top } \mC \rvvu + 2\,\mathbb {E} \rvvu ^{\top } \mC ^{\top } \vm - 2\,\mathbb {E} \rvvu ^{\top } \mC ^{\top } \vz \\ &\;= \mathbb {E} \mathrm {tr}\left (\rvvu ^{\top } \mC ^{\top } \mC \rvvu \right ) + 2\,\mathbb {E} \rvvu ^{\top } \mC ^{\top } \vm - 2\,\mathbb {E} \rvvu ^{\top } \mC ^{\top } \vz \\ &\;= \mathrm {tr}\left ( \mC ^{\top } \mC \mathbb {E} \rvvu \rvvu ^{\top }\right ) + 2\,\mathbb {E} \rvvu ^{\top } \mC ^{\top } \vm - 2\,\mathbb {E} \rvvu ^{\top } \mC ^{\top } \vz , \shortintertext {applying \cref {thm:u_identities},} &\;= \mathrm {tr}\left ( \mC ^{\top } \mC \right ) \\ &\;= \norm { \mC }_{\mathrm {F}}^2. \end {alignat*} Applying this to \cref {eq:reparam_quadratic_eq1}, \begin {alignat*}{2} \mathbb {E}\norm {\vt _{\vlambda }\left (\rvvu \right ) - \vz }_2^2 &= \vm ^{\top } \vm - 2\,\vm ^{\top } \vz + \vz ^{\top } \vz + \norm {\mC }_{\mathrm {F}}^2 \\ &= \norm {\vm - \vz }^2_2 + \norm {\mC }_{\mathrm {F}}^2. \end {alignat*}\end{proof}


==> main-pratendupperboundtheorem.tex <==


\prAtEndRestatevii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndvii}The proof uses the \(L_{\mathrm {H}}\)-smoothness of \(f_{\mathrm {H}}\) such that \begin {align} \mathbb {E} \norm { \nabla f_{\mathrm {H}}\left (\vt _{\vlambda }\left (\rvvu \right )\right ) }_2^2 &= \mathbb {E} {\lVert \nabla f_{\mathrm {H}}\left (\vt _{\vlambda }\left (\rvvu \right )\right ) - \nabla f_{\mathrm {H}}\left (\bar {\vzeta }_{\mathrm {H}}\right ) \rVert }_2^2 \nonumber \\ &\leq L^2_{\mathrm {H}} \mathbb {E} {\lVert \vt _{\vlambda }\left (\rvvu \right ) - \bar {\vzeta }_{\mathrm {H}} \rVert }_2^2, \label {eq:thm_upper_bound_smoothness} \end {align} where \(\bar {\vzeta }_{\mathrm {H}}\) is a stationary point of \(f_{\mathrm {H}}\) such that \(\nabla f_{\mathrm {H}}\left (\bar {\vzeta }_{\mathrm {H}}\right ) = \mathbf {0}\). These steps have been previously used by \citet [Theorem 3]{domke_provable_2019} to prove the special case for the matrix square root parameterization. \par For the mean-field parameterization, we start from \cref {thm:general_variational_gradient_norm_bound} and apply~\cref {eq:thm_upper_bound_smoothness} as \begin {align} &\mathbb {E} \norm { \nabla _{\vlambda } f_{\mathrm {H}}\left (\vt _{\vlambda }\left (\rvvu \right )\right ) }_2^2 \nonumber \\ &\;\leq \mathbb {E} \norm { \nabla f_{\mathrm {H}}\left (\vt _{\vlambda }\left (\rvvu \right )\right ) }_2^2 \left (1 + \norm {\mathbfsfit {U}}_{\mathrm {F}}\right ) \nonumber \\ &\;\leq L^2_{\mathrm {H}} \, \mathbb {E} {\lVert \vt _{\vlambda }\left (\rvvu \right ) + \bar {\vzeta }_{\mathrm {H}} \rVert }_2^2 \left (1 + \norm {\mathbfsfit {U}}_{\mathrm {F}}\right ), \nonumber \shortintertext {applying \cref {thm:meanfield_u_identity},} &\;\leq L^2_{\mathrm {H}} \left ( \kappa \sqrt {d} + \sqrt {\kappa d} + 1 \right ) {\lVert \vm - \bar {\vzeta }_{\mathrm {H}} \rVert }_2^2 \nonumber \\ &\;\;\quad + L^2_{\mathrm {H}} \left (2 \kappa \sqrt {d} + 1\right ) \norm {\mC }_{\mathrm {F}}^2, \nonumber \shortintertext {and since the kurtosis satisfies \(\kappa \geq 1\) and thus \(\kappa \geq \sqrt {\kappa }\),} &\;\leq L^2_{\mathrm {H}} \left ( 2 \kappa \sqrt {d} + 1 \right ) \left ( {\lVert \vm - \bar {\vzeta }_{\mathrm {H}} \rVert }_2^2 + \norm {\mC }_{\mathrm {F}}^2 \right ). \label {eq:thm1_meanfield} \end {align} \par Similarly, for the full-rank parameterizations, we start from \cref {thm:general_variational_gradient_norm_bound} and apply~\cref {eq:thm_upper_bound_smoothness} as \begin {alignat}{2} &\mathbb {E} \norm { \nabla _{\vlambda } f_{\mathrm {H}}\left (\vt _{\vlambda }\left (\rvvu \right )\right ) }_2^2 \\ &\;\leq \mathbb {E}\norm {\nabla f_{\mathrm {H}}\left (\vt _{\vlambda }\left (\rvvu \right )\right )}_2^2 \left (1 + \norm {\rvvu }_2^2 \right ), \nonumber \\ &\;\leq L^2_{\mathrm {H}}\,\mathbb {E}{\lVert \vt _{\vlambda }\left (\rvvu \right ) - \bar {\vzeta }_{\mathrm {H}} \rVert }_2^2 \left (1 + \norm {\rvvu }_2^2 \right ), \nonumber \shortintertext {applying \cref {thm:reparam_u_identity},} &\;= L^2_{\mathrm {H}}\left (\left (d + 1\right ) {\lVert \vm - \bar {\vzeta }_{\mathrm {H}} \rVert }_2^2 + \left (d + \kappa \right ) \norm {\mC }_{\mathrm {F}}^2 \right ), \nonumber \shortintertext {and since the kurtosis satisfies \(\kappa \geq 1\),} &\;\leq L^2_{\mathrm {H}}\left (d + \kappa \right ) \left ( {\lVert \vm - \bar {\vzeta }_{\mathrm {H}} \rVert }_2^2 + \norm {\mC }_{\mathrm {F}}^2 \right ). \label {eq:thm1_fullrank} \end {alignat} \par Both \cref {eq:thm1_meanfield,eq:thm1_fullrank} can now be denoted as \begin {alignat}{2} \mathbb {E}\norm {\nabla _{\vlambda } f_{\mathrm {H}}\left (\vt _{\vlambda }\left (\rvvu \right )\right )}_2^2 &\leq L^2_{\mathrm {H}}\, C\left (d, \kappa \right ) \left ( {\lVert \vm - \bar {\vzeta }_{\mathrm {H}} \rVert }_2^2 + \norm {\mC }_{\mathrm {F}}^2 \right ), \nonumber \shortintertext {where by \cref {thm:reparam_quadratic},} &= L^2_{\mathrm {H}}\, C\left (d, \kappa \right ) \mathbb {E} {\Vert \vt _{\vlambda }\left (\rvvu \right ) - \bar {\vzeta }_{\mathrm {H}} \rVert }_2^2, \label {eq:thm1_parameter_suboptimality_unified} \end {alignat} and the constants are \(C\left (d, \kappa \right ) = \kappa \sqrt {d} + 1\) for mean-field and \(C\left (d, \kappa \right ) = d + \kappa \) for the full-rank parameterizations. \par As mentioned in the sketch, it is necessary to convert the entropy-regularized form into the KL-regularized form through the following inequality: {\setlength {\belowdisplayskip }{1ex} \setlength {\belowdisplayshortskip }{1ex}\setlength {\abovedisplayskip }{1ex} \setlength {\abovedisplayshortskip }{1ex}\begin {alignat*}{2} \hspace {-0.5em} \mathbb {E} {\Vert \vt _{\vlambda }\left (\rvvu \right ) - \bar {\vzeta }_{\mathrm {H}} \rVert }_2^2 &\leq 2\,\mathbb {E} {\lVert \vt _{\vlambda }\left (\rvvu \right ) - \bar {\vzeta }_{\text {KL}} \rVert }_2^2 + 2 \, {\lVert \bar {\vzeta }_{\text {KL}} - \bar {\vzeta }_{\mathrm {H}} \rVert }_2^2. \end {alignat*} }where \(\bar {\vzeta }_{\mathrm {KL}} = \Pi _{f_{\mathrm {KL}}}\left (\bar {\vzeta }_{\mathrm {H}}\right )\) is a projection of \(\bar {\vzeta }_{\mathrm {H}}\) to the set of minimizers of \(f_{\mathrm {KL}}\). Note that the KL-regularized form does not need to be tractable; only its existence suffices. We can now apply the quadratic growth assumption as {\setlength {\belowdisplayskip }{1ex} \setlength {\belowdisplayshortskip }{1ex}\setlength {\abovedisplayskip }{1ex} \setlength {\abovedisplayshortskip }{1ex}\begin {alignat}{2} \hspace {-1em} \mathbb {E} {\lVert \vt _{\vlambda }\left (\rvvu \right ) - \bar {\vzeta }_{\text {KL}} \rVert }_2^2 \nonumber &\leq \frac {2}{\mu _{\mathrm {KL}}} \left ( \mathbb {E} f_{\text {KL}}\left (\vt _{\vlambda }\left (\rvvu \right )\right ) - f^*_{\text {KL}} \right ) \nonumber \\ &= \frac {2}{\mu _{\mathrm {KL}}} \left ( F\left (\vlambda \right ) - h_{\mathrm {KL}}\left (\vlambda \right ) - f^*_{\text {KL}} \right ), \nonumber \shortintertext {and since \(-h_{\mathrm {KL}}\left (\vlambda \right ) = -\DKL {q_{\vlambda }}{p} \leq 0\) by definition,} &\leq \frac {2}{\mu _{\mathrm {KL}}} \left ( F\left (\vlambda \right ) - f^*_{\text {KL}} \right ) \label {eq:thm_upper_bound_kl_upper_bound} \\ &= \frac {2}{\mu _{\mathrm {KL}}} \left ( \left ( F\left (\vlambda \right ) - F^* \right ) + \left ( F^* - f^*_{\text {KL}} \right ) \right ). \label {eq:thm_upper_bound_f_quadratic} \end {alignat} }Combining \cref {eq:thm1_parameter_suboptimality_unified} with \cref {eq:thm_upper_bound_parallel}, {\begin {align*} &\mathbb {E}\norm {\nabla _{\vlambda } f_{\mathrm {H}}\left (\vt _{\vlambda }\left (\rvvu \right )\right )}_2^2 \\ &\;\leq 2 \, L^2_{\mathrm {H}}\, C\left (d, \kappa \right ) \mathbb {E} {\Vert \vt _{\vlambda }\left (\rvvu \right ) - \bar {\vzeta }_{\mathrm {H}} \rVert }_2^2 + 2 \, L^2_{\mathrm {H}}\, C\left (d, \kappa \right ) {\lVert \bar {\vzeta }_{\text {KL}} - \bar {\vzeta }_{\mathrm {H}} \rVert }_2^2, \shortintertext {and applying \cref {eq:thm_upper_bound_f_quadratic},} &\;\leq \frac {4 \, L^2_{\mathrm {H}}}{\mu _{\mathrm {KL}}} C\left (d, \kappa \right ) \left ( \left ( F\left (\vlambda \right ) - F^* \right ) + \left ( F^* - f^*_{\text {KL}} \right ) \right ) \\ &\;\quad + 2 \, L^2_{\mathrm {H}}\, C\left (d, \kappa \right ) {\lVert \bar {\vzeta }_{\text {KL}} - \bar {\vzeta }_{\mathrm {H}} \rVert }_2^2 \end {align*} }Plugging this into \cref {thm:gradient_variance_general_upper_bound} yields the result.\end{proof}


==> main-pratendupperboundtheoremboundedentropy.tex <==


\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndix}The proof is similar to that of \cref {thm:gradient_upper_bound}. As mentioned in the \textit {proof sketch}, we use the fact that the entropic regularizer is bounded such that \[ -h_{\mathrm {H}}\left (\vlambda \right ) < -h_{\mathrm {H}}^*. \] By applying the quadratic growth assumption directly to \(f_{\mathrm {H}}\), \begin {alignat}{2} \mathbb {E} {\lVert \vt _{\vlambda }\left (\rvvu \right ) - \bar {\vzeta }_{\text {H}} \rVert }_2^2 &\leq \frac {2}{\mu _{\mathrm {H}}} \left ( \mathbb {E} f_{\text {H}}\left (\vt _{\vlambda }\left (\rvvu \right )\right ) - f^*_{\text {H}} \right ) \nonumber \\ &= \frac {2}{\mu _{\mathrm {H}}} \left ( F\left (\vlambda \right ) - h_{\mathrm {H}}\left (\vlambda \right ) - f^*_{\text {H}} \right ), \nonumber \shortintertext {and by \cref {assumption:bounded_entropy},} &\leq \frac {2}{\mu _{\mathrm {H}}} \left ( F\left (\vlambda \right ) - F^* \right ) + \frac {2}{\mu _{\mathrm {H}}} \left ( F^* - f^*_{\text {H}} - h_{\mathrm {H}}^*\right ). \label {eq:thm_upper_bound_f_H_quadratic} \end {alignat} \par The proof resumes from \cref {eq:thm1_parameter_suboptimality_unified} as {\setlength {\belowdisplayskip }{1.ex} \setlength {\belowdisplayshortskip }{1.ex}\setlength {\abovedisplayskip }{1.ex} \setlength {\abovedisplayshortskip }{1.ex}\begin {alignat}{2} &\mathbb {E}\norm {\nabla _{\vlambda } f_{\mathrm {H}}\left (\vt _{\vlambda }\left (\rvvu \right )\right )}_2^2 \nonumber \\ &\;\leq L^2_{\mathrm {H}} C\left (d, \kappa \right ) \mathbb {E} {\Vert \vt _{\vlambda }\left (\rvvu \right ) - \bar {\vzeta }_{\mathrm {H}} \rVert }_2^2, \nonumber \shortintertext {and by applying \cref {eq:thm_upper_bound_f_H_quadratic},} &\;= \frac {2 L^2_{\mathrm {H}} }{\mu _{\mathrm {H}}} C\left (d, \kappa \right ) \left ( F\left (\vlambda \right ) - F^* \right ) + \frac {2 L^2_{\mathrm {H}} }{\mu _{\mathrm {H}}} C\left (d, \kappa \right ) \left ( F^* - f^*_{\mathrm {H}} - h_{\mathrm {H}}^* \right ). \nonumber \end {alignat} }Plugging this to \cref {thm:gradient_variance_general_upper_bound} proves the result.\end{proof}


==> main-pratendupperboundtheoremklform.tex <==


\prAtEndRestateviii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndviii}This proof uses the smoothness of \(f_{\mathrm {KL}}\) instead of \(f_{\mathrm {H}}\). That is, \begin {align} \mathbb {E} \norm { \nabla f_{\mathrm {KL}}\left (\vt _{\vlambda }\left (\rvvu \right )\right ) }_2^2 &= \mathbb {E} {\lVert \nabla f_{\mathrm {KL}}\left (\vt _{\vlambda }\left (\rvvu \right )\right ) - \nabla f_{\mathrm {KL}}\left ( \bar {\vzeta }_{\mathrm {KL}} \right ) \rVert }_2^2 \nonumber \shortintertext {applying \cref {eq:thm_upper_bound_smoothness},} &\leq L^2_{\mathrm {KL}} \, \mathbb {E} {\lVert \vt _{\vlambda }\left (\rvvu \right ) - \bar {\vzeta }_{\mathrm {KL}} \rVert }_2^2, \label {eq:thm3_kl_smoothness} \end {align} where \(\bar {\vzeta }_{\mathrm {KL}}\) is a stationary point of \(f_{\mathrm {KL}}\). \par Substituting \cref {eq:thm3_kl_smoothness} in \cref {eq:thm1_parameter_suboptimality_unified}, \begin {alignat}{2} &\mathbb {E}\norm {\nabla _{\vlambda } f_{\mathrm {KL}}\left (\vt _{\vlambda }\left (\rvvu \right )\right )}_2^2 \nonumber \\ &\;\leq L^2_{\mathrm {KL}} C\left (d, \kappa \right ) \mathbb {E} {\Vert \vt _{\vlambda }\left (\rvvu \right ) - \bar {\vzeta }_{\mathrm {KL}} \rVert }_2^2, \nonumber \shortintertext {and by applying \cref {eq:thm_upper_bound_f_quadratic} for \(f_{\mathrm {KL}}\),} &\;= \frac {2 L^2_{\mathrm {KL}} }{\mu _{\mathrm {KL}}} C\left (d, \kappa \right ) \left ( F\left (\vlambda \right ) - F^* \right ) + \frac {2 L^2_{\mathrm {KL}} }{\mu _{\mathrm {KL}}} C\left (d, \kappa \right ) \left ( F^* - f^*_{\text {KL}} \right ). \nonumber \end {alignat} Plugging this to \cref {thm:gradient_variance_general_upper_bound} proves the result.\end{proof}


==> section_gradient_variance_conditions.tex <==

\section{Assumptions on the Gradient Variance}

\begin{definition}[\textbf{Expected Strong Growth; ESG}]
  \(\rvvg\) is said to satisfy the expected strong growth condition if 
  \begin{align*}
    \mathbb{E} \norm{\rvvg\left(\vlambda\right)}^2_2 \leq B \, \norm{ \nabla F\left(\vlambda\right) }^2
  \end{align*}
  for some finite \(B > 0\).
\end{definition}
This is a weaker version of the maximal strong growth condition~\citep{tseng_incremental_1998, schmidt_fast_2013}, where the bound is assumed to hold uniformly instead of in expectation.
Under ESG, for \(L\)-smooth non-convex objectives, \citet{vaswani_fast_2019} prove that SGD with a fixed stepsize of \(\gamma = \nicefrac{1}{B L}\) converges as \(\mathcal{O}\left(2 B L / T\right)\).

Arguably, the most widely recognized gradient condition is the relaxed strong growth by \citet{bottou_optimization_2018}.
\begin{definition}[\textbf{Relaxed Strong Growth; RSG}]
  \(\rvvg\) is said to satisfy the expected strong growth condition if 
  \begin{align*}
    \mathbb{E} \norm{\rvvg\left(\vlambda\right)}^2_2 \leq B \, \norm{ \nabla F\left(\vlambda\right) }^2_2 + C
  \end{align*}
  for some finite \(B, C > 0\).
\end{definition}
\citeauthor{bottou_optimization_2018} prove that, for \(L\)-smooth non-convex objectives and some additional regularity conditions, SGD with a fixed stepsize in \(\mathcal{O}\left(\nicefrac{1}{L B}\right)\) converges to a \(\mathcal{O}\left(\alpha L C\right)\) neighborhood in a rate of \(\mathcal{O}\left(\nicefrac{1}{T \alpha}\right) \).

\begin{definition}[\textbf{Convex Expected Smoothness; C-ES}]
  \(\rvvg\) is said to satisfy the expected strong growth condition if 
  \begin{align*}
    \mathbb{E} \norm{\rvvg\left(\vlambda\right) - \rvvg\left(\vlambda^*\right)}^2_2 \leq 2 A \left( F\left(\vlambda\right) - F\left(\vlambda^*\right) \right)
  \end{align*}
  for some finite \(A > 0\), where \(\vlambda^*\) is the global minimizer.
\end{definition}
This condition was first used by~\cite{gower_stochastic_2021} for studying the JacSketch algorithm  for strongly convex problems.

%%% Local Variables:
%%% TeX-master: "main"
%%% End:

==> section_smoothness.tex <==

\subsection{Non-Smoothness of the ADVI Family}

For the bijection function \(\psi^{-1}: \mathbb{R} \mapsto \mathbb{R}_+\), we provide the following assumptions to verify establish the smoothness of some univariate constrained support distributions.
\begin{assumption}\label{assumption:smooth_bijector}
  \(\psi^{-1}\) is \(L_{\psi}\)-smooth.
\end{assumption}

\begin{assumption}\label{assumption:gamma1}
  \(
  \gamma_1\left(x\right) = \nicefrac{ {\left( \psi^{-1} \right)}^{\prime} \left(x\right) }{ \psi^{-1}\left(x\right) } 
  \)
  is \(L_1\)-Lipschitz.
\end{assumption}

\begin{assumption}\label{assumption:gamma2}
  \(
  \gamma_2\left(x\right) = \nicefrac{ {\left( \psi^{-1} \right)}^{\prime}\left(x\right) }{ {\left(\psi^{-1}\left(x\right)\right)}^2 } 
  \)
  is \(L_2\)-Lipschitz.
\end{assumption}

\begin{assumption}\label{assumption:gamma3}
  \(
  \gamma_3\left(x\right) = {\left(\psi^{-1} \right)}^{\prime}\left(x\right) \, \psi^{-1}\left(x\right) 
  \)
  is \(L_3\)-Lipschitz.
\end{assumption}

\begin{theoremEnd}[category=smoothness]{proposition}
  Let \(\psi^{-1} : \mathbb{R} \mapsto \mathbb{R}_+ \) be the exponential bijector \(\psi^{-1}\left(x\right) = e^x\). 
  Then, \(\psi^{-1}\) 
  \begin{enumerate}[label=(\roman*)]
    \item does not satisfy \cref{assumption:smooth_bijector},
    \item satisfies \cref{assumption:gamma1} for any \(L_1 > 0\),
    \item does not satisfy \cref{assumption:gamma2},
    \item does not satisfy \cref{assumption:gamma3}.
  \end{enumerate}
\end{theoremEnd}
\begin{proofEnd}
  Notice that
  \begin{align*}
    \gamma_1\left(x\right) &= \frac{ e^x }{ e^x } = 1 \\
    \gamma_2\left(x\right) &= \frac{ e^x }{ e^{2x} } = e^{-x} \\
    \gamma_3\left(x\right) &= e^x e^x = e^{2x}.
    \nonumber
  \end{align*}
  Therefore, 
  \begin{enumerate}[label=(\roman*)]
    \item holds trivially.
    \item holds trivially.
    \item The Lipschitzness of \(\gamma_2\left(x\right)\) is equivalent to whether \(e^x\) is Lipschitness, which it is not.
    \item The Lipschitzness of \(\gamma_3\left(x\right)\) is equivalent to whether \(e^{2x}\) is Lipschitness, which it is not.
  \end{enumerate}
\end{proofEnd}

\input{thm_gamma_smoothness}

\input{thm_inverse_gamma_smoothness}

\input{thm_half_normal_smoothness}

%\input{thm_beta_smoothness}

%%% Local Variables:
%%% TeX-master: "main"
%%% End:


==> thm_gamma_smoothness.tex <==

\begin{theoremEnd}[category=smoothness]{proposition}[\textbf{Smoothness of Gamma}]
  Let \(f\left(x; \alpha, \beta\right)\) be the probability density function of the Gamma distribution with parameters \(\alpha, \beta\).
  Also, let \(\psi^{-1} : \mathbb{R} \mapsto \mathbb{R}_+\) be a bijection function.
  \(f \circ \psi^{-1}\) is \(L\)-smooth if and only if \cref{assumption:gamma1,assumption:smooth_bijector} hold, where the the smoothnes constant is \(L = \left(\alpha - 1\right) L_1 + \beta L_{\psi} \).
\end{theoremEnd}
\begin{proofEnd}
  First, the log probability density of the half-normal distribution is given as
  \begin{align}
    \log f\left(x; \sigma\right)
    =
    \left(\alpha - 1\right) \log x - \beta x
    \nonumber
  \end{align}
  where \(\log Z\) is a constant normalizer.
  The derivatives of the inverse gamma distribution with a bijection \(\psi^{-1}\) is given as
  \begin{align*}
    &\frac{d \log f\left(\psi^{-1}\left(x\right); \sigma\right)}{dx}
    \\
    &\;=
    \frac{d \log f\left(\psi^{-1}\left(x\right); \sigma\right)}{d\psi}
    \frac{d \psi^{-1}}{dx}
    \\
    &\;=
    \frac{d \psi^{-1}}{dx}
    \left(
    \left(\alpha - 1\right) \frac{1}{\psi^{-1}\left(x\right)} - \beta 
    \right)
    \\
    &\;=
    \left(\alpha - 1 \right) \frac{ {\left( \psi^{-1} \right)}^{\prime} \left(x\right) }{\psi^{-1}\left(x\right)} + \beta \psi^{-1}\left(x\right).
    \\
    &\;=
    \left(\alpha - 1 \right) \gamma_1\left(x\right)
    +
    \beta {\left( \psi^{-1} \right)}^{\prime} \left(x\right)
  \end{align*}
  Thus, the smoothness is euquivalent to the Lipschitzness of \(\gamma_3\left(x\right)\).

  By the triangle inequlity, the two-way inequality
  \begin{alignat*}{2}
    &\abs{
      \left(\alpha - 1 \right)
    \abs{
      \gamma_1\left(x\right) - \gamma_1\left(y\right)
    }
    -
    \beta
    \abs{
      {\left( \psi^{-1} \right)}^{\prime} \left(x\right)
      -
      {\left( \psi^{-1} \right)}^{\prime} \left(y\right)
    }
    }
    \\
    &\quad\leq
    \abs{
    \frac{d \log f\left(\psi^{-1}\left(x\right); \alpha, \beta\right)}{dx}
    -
    \frac{d \log f\left(\psi^{-1}\left(y\right); \alpha, \beta\right)}{dy}
    }
    \\
    &\quad\quad\leq
    \left( \alpha - 1 \right)
    \abs{
      \gamma_1\left(x\right) - \gamma_1\left(y\right)
    }
    +
    \beta 
    \abs{
      {\left( \psi^{-1} \right)}^{\prime} \left(x\right)
      -
      {\left( \psi^{-1} \right)}^{\prime} \left(y\right)
    }
  \end{alignat*}
  holds.
  The upper bound proves the implication (\(\Rightarrow\)), while the lower bounds (\(\Leftarrow\)) proves the converse by contraposition.
\end{proofEnd}

%%% Local Variables:
%%% TeX-master: "main"
%%% End:


==> thm_strong_convexity.tex <==

\begin{theoremEnd}[category=convexity]{theorem}[\textbf{Strong Convexity}]
  For the location-scale family (\cref{def:family}) with the full-rank (\cref{def:fullrank}) parameterization with a 1-Lipschitz strictly positive function \(\phi\), if \(f\) is \(\mu\)-strongly convex, then \(F\) is also \(\mu\)-strongly convex.
\end{theoremEnd}
\begin{proofsketch}
  For the matrix square root parameterization \citet{domke_provable_2020} have shown that, if \(f\) is \(\mu\)-strongly convex, \(\vlambda \mapsto \mathbb{E} f \circ \vt_{\vlambda}\left(\rvvu\right)\) is also \(\mu\)-strongly convex.
  We simply extrapolate this result by showing that the diagonal elements \(\vs\) preserve strong convexity.
\end{proofsketch}
\begin{proofEnd}
  Recall that
  \begin{align}
    F\left(\vlambda\right)
    =
    \underbrace{\mathbb{E} f\left(\vt_{\vlambda}\left(\rvvu\right)\right)}_{\text{likelihood term}} + \underbrace{h\left(\vlambda\right)}_{\text{regularization term}}.
  \end{align}
  We first establish the strong convexity of the likelihood term and then the convexity of the regularization term.

  \paragraph{Strong Convexity of likelihood term}
  For the matrix square root parameterization (\cref{def:squareroot}), 
  if \(f\) is \(\mu\)-strongly convex, then the likelihood term is also \(\mu\)-strongly convex \citep{domke_provable_2020}.
  This means that, 
  \begin{align}
      & \mathbb{E} f\left(\vt_{\vlambda}\left(\rvvu\right)\right)  - 
 \mathbb{E} f\left(\vt_{\vlambda^{\prime}}\left(\rvvu\right)\right)
      \nonumber
      \\
      &\;=
      \inner{\nabla_{\vlambda^{\prime}} \mathbb{E} f\left( \vt_{\vlambda^{\prime}}\left(\rvvu\right) \right) }{
        \vlambda - \vlambda^{\prime}
      }
      +
      \frac{\mu}{2} \mathbb{E}\norm{\vt_{\vlambda}\left(\rvvu\right) - \vt_{\vlambda^{\prime}}\left(\rvvu\right)}_2^2
      \nonumber
      \\
      &=
      \inner{ 
        \mathbb{E} 
        \frac{
          \partial \vt_{\vlambda^{\prime}}\left(\rvvu\right)
        }{
          \partial \vlambda^{\prime}
        }
        \nabla f \left( \vt_{\vlambda^{\prime}}\left(\rvvu\right) \right)
      }{
        \vlambda - \vlambda^{\prime}
      }
      +
      \frac{\mu}{2} \mathbb{E}\norm{\vt_{\vlambda}\left(\rvvu\right) - \vt_{\vlambda^{\prime}}\left(\rvvu\right)}_2^2.
      \label{eq:thm_convexity_inequality}
  \end{align}
  Focusing on the inner product term,
  \begin{align*}
    &\inner{ 
      \mathbb{E} 
      \frac{
        \partial \vt_{\vlambda^{\prime}}\left(\rvvu\right)
      }{
        \partial \vlambda^{\prime}
      }
      \nabla f \left( \vt_{\vlambda^{\prime}}\left(\rvvu\right) \right)
    }{
      \vlambda - \vlambda^{\prime}
    }
    \\
    &\;= 
    \inner{ 
      \mathbb{E} 
      \frac{
        \partial \vt_{\vlambda^{\prime}}\left(\rvvu\right)
      }{
        \partial \vm^{\prime}
      }
      \nabla f \left( \vt_{\vlambda^{\prime}}\left(\rvvu\right) \right)
    }{
      \vm - \vm^{\prime}
    }
    \\
    &\;\quad+
    \sum^d_{j=1} \sum^d_{i=1} 
    \left(
    \mathbb{E} 
    \frac{
      \partial \vt_{\vlambda^{\prime}}\left(\rvvu\right)
    }{
      \partial C_{ij}^{\prime}
    }
    \nabla f \left( \vt_{\vlambda^{\prime}}\left(\rvvu\right) \right)
    \right)
    \left(C_{ij} - C_{ij}^{\prime}\right)
    \\
    &\;= 
    \inner{ 
      \mathbb{E} 
      \frac{
        \partial \vt_{\vlambda}\left(\rvvu\right)
      }{
        \partial \vm^{\prime}
      }
      \nabla f \left( \vt_{\vlambda^{\prime}}\left(\rvvu\right) \right)
    }{
      \vm - \vm^{\prime}
    }
    \\
    &\;\quad+
    \underbrace{
    \sum^d_{j=1} \sum^d_{i=1,\,i \neq j} 
    \left(
    \mathbb{E} 
    \frac{
      \partial \vt_{\vlambda^{\prime}}\left(\rvvu\right)
    }{
      \partial C_{ij}^{\prime}
    }
    \nabla f \left( \vt_{\vlambda^{\prime}}\left(\rvvu\right) \right)
    \right)
    \left(C_{ij} - C_{ij}^{\prime}\right)
    }_{\text{off-diagonal of \(\mC\)}}
    \\
    &\;\quad+
    \underbrace{
    \sum^d_{i=1} 
    \left(
    \mathbb{E}
    \frac{
      \partial \vt_{\vlambda^{\prime}}\left(\rvvu\right)
    }{
      \partial C_{ii}^{\prime}
    }
    \nabla f \left( \vt_{\vlambda^{\prime}}\left(\rvvu\right) \right)
    \right)
    \left(C_{ii} - C_{ii}^{\prime}\right)
    }_{\text{diagonal of \(\mC\)}}.
  \end{align*}
  Furthermore, the  diagonal terms can be shown to satisfy
  \begin{align}
    &\sum^d_{i=1} 
    \left(
    \mathbb{E}
    \frac{
      \partial \vt_{\vlambda^{\prime}}\left(\rvvu\right)
    }{
      \partial C_{ii}^{\prime}
    }
    \nabla f \left( \vt_{\vlambda^{\prime}}\left(\rvvu\right) \right)
    \right)
    \left(C_{ii} - C_{ii}^{\prime}\right)
    \nonumber
    \\
    &\;=
    \sum^d_{i=1} 
    \mathbb{E}
    u_i \ve_i^{\top} \nabla f \left( \vt_{\vlambda^{\prime}}\left(\rvvu\right) \right)
    \left(C_{ii} - C_{ii}^{\prime}\right).\label{eq:thm_convexity_diagonal_squareroot}
  \end{align}
  For the parameterizations in \cref{def:meanfield} and \cref{def:fullrank}, the derivatives only differ for the diagonal of \(\mC\).
  Specifically, since the diagonals are \(C_{\mathrm{FR},ii} = \phi\left(s_i\right)\), the inner product term of the diagonal entries of the full rank parameterization (\cref{def:fullrank}) is now
  \begin{align*}
    &\sum^d_{i=1} 
    \left(
    \mathbb{E}
    \frac{
      \partial \vt_{\vlambda^{\prime}}\left(\rvvu\right)
    }{
      \partial C_{\mathrm{FR},ii}^{\prime}
    }
    \nabla f \left( \vt_{\vlambda^{\prime}}\left(\rvvu\right) \right)
    \right)
    \left(C_{\mathrm{FR},ii} - C_{\mathrm{FR},ii}^{\prime}\right)
    \\
    &\;=
    \sum^d_{i=1} 
    \mathbb{E}
    \phi^{\prime}\left(s_i^{\prime}\right) u_i \ve_i^{\top} \nabla f \left( \vt_{\vlambda^{\prime}}\left(\rvvu\right) \right)
    \left(C_{\mathrm{FR},ii} - C_{\mathrm{FR},ii}^{\prime}\right)
    \\
    &\;\leq
    \sum^d_{i=1} 
    \mathbb{E}
    u_i \ve_i^{\top} \nabla f \left( \vt_{\vlambda^{\prime}}\left(\rvvu\right) \right)
    \left(C_{\mathrm{FR},ii} - C_{\mathrm{FR},ii}^{\prime}\right),
  \end{align*}
  which is equal to~\cref{eq:thm_convexity_diagonal_squareroot}.
  Therefore, the bound in \cref{eq:thm_convexity_inequality} is preserved, where the strong convexity term 

  \paragraph{Convexity of regularization term}
  For the full-rank Cholesky parameterization \cref{def:fullrank}, the regularization term is 
  \begin{align*}
    h\left(\vlambda\right) 
    &= - \mathrm{H}\left(q_{\vlambda}\right)
    \\
    &= - \mathrm{H}\left(\varphi\right) - \log \abs{ \mC }
    \\
    &= - \mathrm{H}\left(\varphi\right) - \sum_{i=1}^{d} \log \phi\left(s_i\right).
  \end{align*}
  Showing that \(-\log \phi\) is convex shows that \(h\) is convex since the sum of convex functions is convex.
  Now, since
  \begin{align*}
    -\frac{d^2 \log \phi}{ds^2} 
    =
    \frac{
      {\phi^{\prime}\left(s\right)}^{2} - \phi^{\prime\prime}\left(x\right)
    }{
      {\phi\left(s\right)}^{2}
    }
  \end{align*}
  and \(\phi\left(s\right) > 0\) for all \(s\), any \(\phi\) satisfying results in \(h\) being convex.
\end{proofEnd}

%%% Local Variables:
%%% TeX-master: "main"
%%% End:

